Constraining the Parameter Space of the Dark Energy Equation of State Using Alternative Cosmic Tracers

We propose to use HII galaxies (HIIG) to trace the redshift-distance relation, by means of their $L(\mathrm{H}\beta) - \sigma$ correlation, in an attempt to constrain the dark energy equation of state parameter solution space, as an alternative to the cosmological use of type Ia supernovae. For a sample of 128 local compact HIIG with high equivalent widths of their Balmer emission lines we obtained ionised gas velocity dispersion from high S/N, high-dispersion spectroscopy (Subaru-HDS and ESO VLT-UVES) and integrated H$\beta$ fluxes from low dispersion wide aperture spectrophotometry. We find that the $L(\mathrm{H}\beta) - \sigma$ relation is strong and stable against restrictions in the sample. The size of the starforming region is an important second parameter, while adding the emission line equivalent width or the continuum colour and metallicity, produces the solution with the smallest rms scatter. We have used the $L(\mathrm{H}\beta) - \sigma$ relation from a local sample of HIIG and a local calibration or `anchor', given by giant HII regions in nearby galaxies which have accurate distance measurements determined via primary indicators, to obtain a value of $H_0$. Using our best sample of 69 HIIG and 23 Giant HII regions in 9 galaxies we obtain $H_{0}=74.3 \pm 3.1$ (statistical)$\pm$ 2.9 (systematic) km s$^{-1}$ Mpc$^{-1}$, in excellent agreement with, and independently confirming, the most recent SNa Ia based results. Using a local sample (107 sources) and a sample of 21 high redshift HIIG, 6 of them with medium-dispersion spectroscopy (ESO VLT-XShooter) and 17 taken from the literature, we have obtained constraints on the planes $H_0 - \Omega_m$, $\Omega_m - w_0$ and $w_0 - w_1$ (CPL model).

==> ch04/tab/tab05_old.tex <==
%Table  5 --- Derived data for the H II galaxies sample

\onecolumn
%\begin{landscape}
\scriptsize
\begin{center}
\begin{longtable}{@{} l l c c c c c c c c c @{}}
 
\caption{ Derived data for the \hii\ galaxies sample. } 
\label{tab:tab5} \\


%This is the header for the first page of the table...
\hline \hline \\[-2ex]
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} & 
\multicolumn{1}{c}{(8)} & 
\multicolumn{1}{c}{(9)} & 
\multicolumn{1}{c}{(10)} & 
\multicolumn{1}{c}{(11)} \\

\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{\bf{Flag}} &
\multicolumn{1}{c}{$\mathbf{z_c}$} &
\multicolumn{1}{c}{$\mathbf{A_v}$} &
\multicolumn{1}{c}{$\mathbf{100 \times Q}$} &
\multicolumn{1}{c}{$\mathbf{C_{\hb}}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma ([\Oiii])}$} &
\multicolumn{1}{c}{$\mathbf{\logd L (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\mathrm{O/H} + 12}$} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ (mag)} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{erg\ s^{-1}}$)} & 
\multicolumn{1}{c}{}  \\[0.5ex] \hline \\[-1.8ex]


\endfirsthead

%This is the header for the remaining page(s) of the table...
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} & 
\multicolumn{1}{c}{(8)} & 
\multicolumn{1}{c}{(9)} & 
\multicolumn{1}{c}{(10)} & 
\multicolumn{1}{c}{(11)} \\

\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{\bf{Flag}} &
\multicolumn{1}{c}{$\mathbf{z_c}$} &
\multicolumn{1}{c}{$\mathbf{A_v}$} &
\multicolumn{1}{c}{$\mathbf{100 \times Q}$} &
\multicolumn{1}{c}{$\mathbf{C_{\hb}}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma ([\Oiii])}$} &
\multicolumn{1}{c}{$\mathbf{\logd L (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\mathrm{O/H} + 12}$} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ (mag)} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{erg\ s^{-1}}$)} & 
\multicolumn{1}{c}{}  \\[0.5ex] \hline \\[-1.8ex]
\endhead

\multicolumn{2}{l}{{Continued on Next Page\ldots}} \\
\endfoot


\\[-1.8ex] \hline 
%\insertTableNotes
\endlastfoot
001	&	J000657+005125	&	G	&	0.073	$\pm$	0.000006	&	0.67	$\pm$	0.152	&	0.08	&	0.30	$\pm$	0.069	&	1.624	$\pm$	0.032	&	1.551	$\pm$	0.027	&	41.19	$\pm$	0.127	&	8.06	$\pm$	0.142	\\
002	&	J001647-104742	&	NG	&	0.022	$\pm$	0.000005	&	1.42	$\pm$	0.271	&	0.83	&	0.64	$\pm$	0.123	&	1.301	$\pm$	0.047	&	1.324	$\pm$	0.026	&	41.01	$\pm$	0.197	&	8.07	$\pm$	0.134	\\
003	&	J002339-094848	&	NG	&	0.052	$\pm$	0.000035	&	1.07	$\pm$	0.206	&	0.00	&	0.48	$\pm$	0.094	&	0.788	$\pm$	0.450	&	1.507	$\pm$	0.024	&	41.43	$\pm$	0.162	&	8.15	$\pm$	0.184	\\
004	&	J002425+140410	&	NG	&	0.013	$\pm$	0.000006	&	0.37	$\pm$	0.096	&	6.35	&	0.17	$\pm$	0.044	&	1.581	$\pm$	0.036	&	1.497	$\pm$	0.026	&	40.31	$\pm$	0.080	&	8.19	$\pm$	0.117	\\
005	&	J003218+150014	&	NG	&	0.016	$\pm$	0.000979	&	0.05	$\pm$	0.052	&	4.62	&	0.02	$\pm$	0.024	&	1.601	$\pm$	0.032	&	1.615	$\pm$	0.023	&	40.43	$\pm$	0.116	&	8.02	$\pm$	0.060	\\
006	&	J005147+000940	&	NG	&	0.036	$\pm$	0.000879	&	0.02	$\pm$	0.018	&	0.41	&	0.01	$\pm$	0.008	&	1.430	$\pm$	0.037	&	1.325	$\pm$	0.024	&	40.51	$\pm$	0.084	&	7.80	$\pm$	0.015	\\
007	&	J005602-101009	&	G	&	0.057	$\pm$	0.000006	&	0.59	$\pm$	0.149	&	0.99	&	0.27	$\pm$	0.068	&	1.508	$\pm$	0.034	&	1.467	$\pm$	0.024	&	40.95	$\pm$	0.122	&	7.88	$\pm$	0.169	\\
008	&	J013258-085337	&	G	&	0.094	$\pm$	0.000691	&	0.00	$\pm$	0.009	&	3.88	&	0.00	$\pm$	0.004	&	1.552	$\pm$	0.032	&	1.475	$\pm$	0.024	&	41.19	$\pm$	0.081	&	8.30	$\pm$	0.075	\\
009	&	J013344+005711	&	NG	&	0.018	$\pm$	0.000006	&	0.20	$\pm$	0.108	&	3.14	&	0.09	$\pm$	0.049	&	1.314	$\pm$	0.046	&	1.178	$\pm$	0.027	&	39.68	$\pm$	0.295	&	8.02	$\pm$	0.104	\\
010	&	J014137-091435	&	G	&	0.017	$\pm$	0.000004	&	0.83	$\pm$	0.194	&	1.65	&	0.38	$\pm$	0.088	&	1.377	$\pm$	0.042	&	1.327	$\pm$	0.026	&	40.52	$\pm$	0.146	&	8.03	$\pm$	0.182	\\
011	&	J014707+135629	&	G	&	0.056	$\pm$	0.000835	&	0.53	$\pm$	0.122	&	0.99	&	0.24	$\pm$	0.055	&	1.620	$\pm$	0.031	&	1.583	$\pm$	0.023	&	41.26	$\pm$	0.114	&	7.94	$\pm$	0.096	\\
012	&	J021852-091218	&	NG	&	0.012	$\pm$	0.000004	&	0.86	$\pm$	0.193	&	0.00	&	0.39	$\pm$	0.088	&	1.229	$\pm$	0.054	&	1.176	$\pm$	0.028	&	39.80	$\pm$	0.148	&	7.94	$\pm$	0.230	\\
013	&	J022037-092907	&	G	&	0.112	$\pm$	0.000007	&	0.37	$\pm$	0.098	&	0.08	&	0.17	$\pm$	0.044	&	1.662	$\pm$	0.030	&	1.601	$\pm$	0.023	&	41.83	$\pm$	0.102	&	8.07	$\pm$	0.133	\\
014	&	J024052-082827	&	G	&	0.082	$\pm$	0.000908	&	0.47	$\pm$	0.113	&	0.00	&	0.21	$\pm$	0.051	&	1.565	$\pm$	0.032	&	1.595	$\pm$	0.023	&	41.66	$\pm$	0.108	&	7.99	$\pm$	0.061	\\
015	&	J024453-082137	&	NG	&	0.077	$\pm$	0.000005	&	0.33	$\pm$	0.125	&	4.79	&	0.15	$\pm$	0.057	&	1.600	$\pm$	0.031	&	1.563	$\pm$	0.023	&	41.32	$\pm$	0.107	&	7.99	$\pm$	0.099	\\
016	&	J025426-004122	&	G	&	0.014	$\pm$	0.000005	&	0.23	$\pm$	0.085	&	9.32	&	0.11	$\pm$	0.038	&	1.388	$\pm$	0.041	&	1.400	$\pm$	0.024	&	40.05	$\pm$	0.093	&	7.84	$\pm$	0.097	\\
017	&	J030321-075923	&	NG	&	0.164	$\pm$	0.000012	&	0.00	$\pm$	0.007	&	7.76	&	0.00	$\pm$	0.003	&	1.737	$\pm$	0.028	&	1.708	$\pm$	0.023	&	41.51	$\pm$	0.084	&	7.91	$\pm$	0.033	\\
018	&	J031023-083432	&	G	&	0.051	$\pm$	0.000006	&	0.21	$\pm$	0.125	&	6.52	&	0.10	$\pm$	0.057	&	1.513	$\pm$	0.035	&	1.472	$\pm$	0.024	&	40.48	$\pm$	0.115	&	8.17	$\pm$	0.067	\\
019	&	J033526-003811	&	G	&	0.023	$\pm$	0.000004	&	0.54	$\pm$	0.163	&	4.04	&	0.25	$\pm$	0.074	&	1.373	$\pm$	0.043	&	1.248	$\pm$	0.032	&	40.34	$\pm$	0.127	&	7.87	$\pm$	0.163	\\
020	&	J040937-051805	&	G	&	0.074	$\pm$	0.000740	&	0.47	$\pm$	0.128	&	2.06	&	0.21	$\pm$	0.058	&	1.570	$\pm$	0.033	&	1.494	$\pm$	0.023	&	41.52	$\pm$	0.112	&	8.15	$\pm$	0.117	\\
021	&	J051519-391741	&	NG	&	0.050	$\pm$	0.000335	&	0.68	$\pm$	0.383	&	0.00	&	0.31	$\pm$	0.174	&	1.423	$\pm$	0.017	&	1.395	$\pm$	0.006	&	41.21	$\pm$	0.214	&	---	$\pm$	---	\\
022	&	J064650-374322	&	G	&	0.027	$\pm$	0.000174	&	1.37	$\pm$	0.525	&	0.66	&	0.62	$\pm$	0.238	&	---	$\pm$	---	&	---	$\pm$	---	&	41.01	$\pm$	0.290	&	---	$\pm$	---	\\
023	&	J074806+193146	&	G	&	0.063	$\pm$	0.000844	&	0.88	$\pm$	0.183	&	0.00	&	0.40	$\pm$	0.083	&	1.563	$\pm$	0.017	&	1.525	$\pm$	0.008	&	41.32	$\pm$	0.152	&	8.27	$\pm$	0.186	\\
024	&	J074947+154013	&	G	&	0.075	$\pm$	0.000006	&	0.55	$\pm$	0.141	&	0.00	&	0.25	$\pm$	0.064	&	1.559	$\pm$	0.015	&	1.527	$\pm$	0.004	&	41.11	$\pm$	0.117	&	8.17	$\pm$	0.146	\\
025	&	J080000+274642	&	G	&	0.040	$\pm$	0.000008	&	0.57	$\pm$	0.142	&	7.26	&	0.26	$\pm$	0.065	&	1.473	$\pm$	0.018	&	1.402	$\pm$	0.007	&	40.78	$\pm$	0.256	&	8.18	$\pm$	0.155	\\
026	&	J080619+194927	&	G	&	0.071	$\pm$	0.000775	&	0.50	$\pm$	0.116	&	3.80	&	0.23	$\pm$	0.053	&	1.721	$\pm$	0.029	&	1.714	$\pm$	0.023	&	41.88	$\pm$	0.112	&	8.23	$\pm$	0.110	\\
027	&	J081334+313252	&	NG	&	0.020	$\pm$	0.000005	&	0.32	$\pm$	0.082	&	2.64	&	0.14	$\pm$	0.037	&	1.444	$\pm$	0.038	&	1.498	$\pm$	0.024	&	40.61	$\pm$	0.116	&	8.10	$\pm$	0.114	\\
028	&	J081403+235328	&	NG	&	0.021	$\pm$	0.000005	&	0.40	$\pm$	0.171	&	7.26	&	0.18	$\pm$	0.078	&	1.483	$\pm$	0.017	&	1.492	$\pm$	0.005	&	40.22	$\pm$	0.123	&	8.22	$\pm$	0.241	\\
029	&	J081420+575008	&	NG	&	0.055	$\pm$	0.000005	&	0.32	$\pm$	0.110	&	7.84	&	0.14	$\pm$	0.050	&	1.584	$\pm$	0.034	&	1.545	$\pm$	0.024	&	41.04	$\pm$	0.103	&	8.18	$\pm$	0.123	\\
030	&	J081737+520236	&	G	&	0.024	$\pm$	0.000033	&	0.74	$\pm$	0.158	&	6.35	&	0.33	$\pm$	0.072	&	1.576	$\pm$	0.032	&	1.609	$\pm$	0.024	&	40.88	$\pm$	0.176	&	8.29	$\pm$	0.263	\\
031	&	J082520+082723	&	G	&	0.088	$\pm$	0.000008	&	0.65	$\pm$	0.179	&	2.31	&	0.29	$\pm$	0.081	&	1.548	$\pm$	0.019	&	1.547	$\pm$	0.002	&	41.17	$\pm$	0.132	&	8.12	$\pm$	0.177	\\
032	&	J082530+504804	&	G	&	0.097	$\pm$	0.000008	&	0.37	$\pm$	0.111	&	5.61	&	0.17	$\pm$	0.050	&	1.647	$\pm$	0.030	&	1.641	$\pm$	0.023	&	41.66	$\pm$	0.105	&	8.10	$\pm$	0.123	\\
033	&	J082722+202612	&	G	&	0.109	$\pm$	0.000006	&	0.94	$\pm$	0.191	&	0.00	&	0.43	$\pm$	0.087	&	1.706	$\pm$	0.014	&	1.705	$\pm$	0.006	&	41.97	$\pm$	0.152	&	8.07	$\pm$	0.195	\\
034	&	J083946+140033	&	G	&	0.112	$\pm$	0.000007	&	0.54	$\pm$	0.150	&	5.12	&	0.25	$\pm$	0.068	&	1.702	$\pm$	0.010	&	1.700	$\pm$	0.005	&	41.65	$\pm$	0.122	&	8.17	$\pm$	0.170	\\
035	&	J084000+180531	&	G	&	0.073	$\pm$	0.000007	&	0.35	$\pm$	0.101	&	1.65	&	0.16	$\pm$	0.046	&	1.655	$\pm$	0.021	&	1.629	$\pm$	0.009	&	41.32	$\pm$	0.101	&	7.95	$\pm$	0.151	\\
036	&	J084029+470710	&	G	&	0.043	$\pm$	0.001019	&	0.76	$\pm$	0.172	&	4.95	&	0.34	$\pm$	0.078	&	1.561	$\pm$	0.033	&	1.479	$\pm$	0.024	&	41.49	$\pm$	0.137	&	7.72	$\pm$	0.270	\\
037	&	J084056+022030	&	NG	&	0.052	$\pm$	0.000796	&	0.65	$\pm$	0.138	&	0.00	&	0.29	$\pm$	0.063	&	---	$\pm$	---	&	---	$\pm$	---	&	40.68	$\pm$	0.122	&	8.09	$\pm$	0.155	\\
038	&	J084219+300703	&	G	&	0.085	$\pm$	0.000009	&	0.74	$\pm$	0.166	&	6.52	&	0.33	$\pm$	0.075	&	1.646	$\pm$	0.016	&	1.607	$\pm$	0.007	&	41.67	$\pm$	0.136	&	8.04	$\pm$	0.141	\\
039	&	J084220+115000	&	NG	&	0.031	$\pm$	0.000030	&	1.05	$\pm$	0.217	&	0.00	&	0.48	$\pm$	0.098	&	1.484	$\pm$	0.035	&	1.440	$\pm$	0.024	&	41.07	$\pm$	0.178	&	8.04	$\pm$	0.205	\\
040	&	J084414+022621	&	G	&	0.092	$\pm$	0.000741	&	1.07	$\pm$	0.209	&	0.41	&	0.48	$\pm$	0.095	&	1.726	$\pm$	0.007	&	1.709	$\pm$	0.005	&	42.08	$\pm$	0.148	&	8.20	$\pm$	0.195	\\
041	&	J084527+530852	&	NG	&	0.031	$\pm$	0.000031	&	0.60	$\pm$	0.121	&	0.00	&	0.27	$\pm$	0.055	&	1.433	$\pm$	0.037	&	1.440	$\pm$	0.024	&	40.90	$\pm$	0.116	&	---	$\pm$	---	\\
042	&	J084634+362620	&	NG	&	0.011	$\pm$	0.000010	&	0.84	$\pm$	0.163	&	0.00	&	0.38	$\pm$	0.074	&	0.946	$\pm$	0.258	&	1.368	$\pm$	0.029	&	40.28	$\pm$	0.157	&	8.07	$\pm$	0.150	\\
043	&	J085221+121651	&	NG	&	0.077	$\pm$	0.000796	&	0.55	$\pm$	0.113	&	0.00	&	0.25	$\pm$	0.052	&	1.785	$\pm$	0.027	&	1.565	$\pm$	0.027	&	42.01	$\pm$	0.112	&	8.12	$\pm$	0.106	\\
044	&	J090418+260106	&	NG	&	0.099	$\pm$	0.000006	&	0.80	$\pm$	0.181	&	6.02	&	0.36	$\pm$	0.082	&	1.772	$\pm$	0.015	&	1.747	$\pm$	0.007	&	41.69	$\pm$	0.154	&	8.19	$\pm$	0.159	\\
045	&	J090506+223833	&	G	&	0.126	$\pm$	0.000009	&	0.29	$\pm$	0.093	&	2.15	&	0.13	$\pm$	0.042	&	1.647	$\pm$	0.014	&	1.632	$\pm$	0.004	&	41.71	$\pm$	0.098	&	8.14	$\pm$	0.084	\\
046	&	J090531+033530	&	G	&	0.040	$\pm$	0.000918	&	0.01	$\pm$	0.044	&	3.38	&	0.00	$\pm$	0.020	&	1.558	$\pm$	0.014	&	1.550	$\pm$	0.004	&	40.77	$\pm$	0.086	&	7.86	$\pm$	0.039	\\
047	&	J091434+470207	&	G	&	0.028	$\pm$	0.000030	&	0.32	$\pm$	0.081	&	3.22	&	0.15	$\pm$	0.037	&	1.529	$\pm$	0.034	&	1.486	$\pm$	0.024	&	41.06	$\pm$	0.072	&	8.12	$\pm$	0.072	\\
048	&	J091640+182807	&	NG	&	0.023	$\pm$	0.000006	&	0.50	$\pm$	0.108	&	0.00	&	0.23	$\pm$	0.049	&	1.495	$\pm$	0.037	&	1.451	$\pm$	0.023	&	40.42	$\pm$	0.109	&	8.03	$\pm$	0.096	\\
049	&	J091652+003113	&	G	&	0.058	$\pm$	0.000004	&	0.47	$\pm$	0.124	&	0.58	&	0.21	$\pm$	0.056	&	1.598	$\pm$	0.009	&	1.586	$\pm$	0.004	&	40.97	$\pm$	0.112	&	8.32	$\pm$	0.140	\\
050	&	J092540+063116	&	G	&	0.076	$\pm$	0.000005	&	0.59	$\pm$	0.141	&	0.83	&	0.27	$\pm$	0.064	&	1.658	$\pm$	0.017	&	1.636	$\pm$	0.013	&	41.36	$\pm$	0.121	&	8.06	$\pm$	0.143	\\
051	&	J092749+084037	&	G	&	0.108	$\pm$	0.000007	&	0.95	$\pm$	0.207	&	1.24	&	0.43	$\pm$	0.094	&	1.732	$\pm$	0.015	&	1.695	$\pm$	0.006	&	41.85	$\pm$	0.157	&	7.88	$\pm$	0.216	\\
052	&	J092918+002813	&	G	&	0.095	$\pm$	0.000005	&	0.35	$\pm$	0.118	&	0.41	&	0.16	$\pm$	0.054	&	1.560	$\pm$	0.012	&	1.556	$\pm$	0.003	&	41.49	$\pm$	0.107	&	8.06	$\pm$	0.108	\\
053	&	J093006+602653	&	G	&	0.014	$\pm$	0.000009	&	0.25	$\pm$	0.071	&	2.72	&	0.11	$\pm$	0.032	&	1.449	$\pm$	0.038	&	1.403	$\pm$	0.024	&	40.40	$\pm$	0.091	&	7.99	$\pm$	0.056	\\
054	&	J093424+222522	&	G	&	0.085	$\pm$	0.000753	&	0.50	$\pm$	0.118	&	0.58	&	0.22	$\pm$	0.054	&	1.696	$\pm$	0.013	&	1.681	$\pm$	0.004	&	41.32	$\pm$	0.125	&	8.06	$\pm$	0.131	\\
055	&	J093813+542825	&	NG	&	0.103	$\pm$	0.000712	&	0.48	$\pm$	0.113	&	6.11	&	0.22	$\pm$	0.051	&	1.785	$\pm$	0.027	&	1.756	$\pm$	0.022	&	42.09	$\pm$	0.109	&	8.10	$\pm$	0.213	\\
056	&	J094000+203122	&	NG	&	0.046	$\pm$	0.000007	&	0.00	$\pm$	0.000	&	0.00	&	0.00	$\pm$	0.000	&	1.596	$\pm$	0.019	&	1.581	$\pm$	0.007	&	40.64	$\pm$	0.080	&	---	$\pm$	---	\\
057	&	J094252+354725	&	NG	&	0.016	$\pm$	0.000010	&	0.23	$\pm$	0.051	&	0.00	&	0.11	$\pm$	0.023	&	1.498	$\pm$	0.035	&	1.501	$\pm$	0.025	&	40.03	$\pm$	0.109	&	7.98	$\pm$	0.043	\\
058	&	J094254+340411	&	NG	&	0.023	$\pm$	0.000004	&	0.01	$\pm$	0.045	&	1.65	&	0.00	$\pm$	0.020	&	1.680	$\pm$	0.101	&	1.332	$\pm$	0.026	&	39.95	$\pm$	0.084	&	7.77	$\pm$	0.062	\\
059	&	J094809+425713	&	NG	&	0.018	$\pm$	0.000006	&	0.35	$\pm$	0.079	&	0.00	&	0.16	$\pm$	0.036	&	1.443	$\pm$	0.038	&	1.396	$\pm$	0.025	&	40.09	$\pm$	0.115	&	8.17	$\pm$	0.043	\\
060	&	J095000+300341	&	NG	&	0.018	$\pm$	0.000004	&	0.44	$\pm$	0.098	&	0.17	&	0.20	$\pm$	0.044	&	1.446	$\pm$	0.038	&	1.453	$\pm$	0.024	&	40.31	$\pm$	0.103	&	---	$\pm$	---	\\
061	&	J095023+004229	&	NG	&	0.099	$\pm$	0.000719	&	0.62	$\pm$	0.131	&	0.00	&	0.28	$\pm$	0.059	&	1.753	$\pm$	0.016	&	1.706	$\pm$	0.006	&	41.75	$\pm$	0.119	&	8.08	$\pm$	0.155	\\
062	&	J095131+525936	&	NG	&	0.047	$\pm$	0.000817	&	0.54	$\pm$	0.144	&	3.80	&	0.25	$\pm$	0.065	&	1.716	$\pm$	0.031	&	1.682	$\pm$	0.024	&	41.41	$\pm$	0.120	&	8.05	$\pm$	0.124	\\
063	&	J095226+021759	&	G	&	0.120	$\pm$	0.000685	&	0.71	$\pm$	0.159	&	1.82	&	0.32	$\pm$	0.072	&	1.718	$\pm$	0.017	&	1.691	$\pm$	0.008	&	41.76	$\pm$	0.143	&	8.21	$\pm$	0.268	\\
064	&	J095227+322809	&	G	&	0.016	$\pm$	0.000004	&	0.35	$\pm$	0.086	&	0.66	&	0.16	$\pm$	0.039	&	1.297	$\pm$	0.049	&	1.241	$\pm$	0.029	&	40.21	$\pm$	0.099	&	7.91	$\pm$	0.075	\\
065	&	J095545+413429	&	G	&	0.016	$\pm$	0.000005	&	0.95	$\pm$	0.202	&	2.23	&	0.43	$\pm$	0.092	&	1.445	$\pm$	0.038	&	1.399	$\pm$	0.025	&	40.39	$\pm$	0.168	&	8.06	$\pm$	0.221	\\
066	&	J100720+193349	&	G	&	0.033	$\pm$	0.000005	&	0.35	$\pm$	0.111	&	0.00	&	0.16	$\pm$	0.051	&	1.321	$\pm$	0.029	&	1.270	$\pm$	0.000	&	40.19	$\pm$	0.105	&	7.81	$\pm$	0.095	\\
067	&	J100746+025228	&	NG	&	0.025	$\pm$	0.000926	&	0.66	$\pm$	0.134	&	0.00	&	0.30	$\pm$	0.061	&	1.536	$\pm$	0.034	&	1.447	$\pm$	0.024	&	40.79	$\pm$	0.127	&	7.90	$\pm$	0.026	\\
068	&	J101036+641242	&	NG	&	0.040	$\pm$	0.000810	&	0.92	$\pm$	0.182	&	5.20	&	0.42	$\pm$	0.082	&	1.816	$\pm$	0.027	&	1.807	$\pm$	0.023	&	41.44	$\pm$	0.146	&	8.24	$\pm$	0.184	\\
069	&	J101042+125516	&	G	&	0.062	$\pm$	0.000933	&	0.20	$\pm$	0.043	&	0.00	&	0.09	$\pm$	0.020	&	1.635	$\pm$	0.024	&	1.578	$\pm$	0.012	&	41.67	$\pm$	0.088	&	8.03	$\pm$	0.072	\\
070	&	J101136+263027	&	G	&	0.056	$\pm$	0.000775	&	0.66	$\pm$	0.140	&	0.83	&	0.30	$\pm$	0.064	&	1.612	$\pm$	0.017	&	1.573	$\pm$	0.007	&	41.21	$\pm$	0.124	&	8.11	$\pm$	0.125	\\
071	&	J101157+130822	&	NG	&	0.145	$\pm$	0.000005	&	0.09	$\pm$	0.064	&	0.74	&	0.04	$\pm$	0.029	&	0.998	$\pm$	0.079	&	1.656	$\pm$	0.023	&	41.57	$\pm$	0.102	&	8.04	$\pm$	0.137	\\
072	&	J101430+004755	&	NG	&	0.148	$\pm$	0.000003	&	0.47	$\pm$	0.147	&	10.07	&	0.21	$\pm$	0.067	&	1.788	$\pm$	0.010	&	1.763	$\pm$	0.001	&	41.71	$\pm$	0.127	&	8.03	$\pm$	0.147	\\
073	&	J101458+193219	&	NG	&	0.014	$\pm$	0.000004	&	0.42	$\pm$	0.111	&	0.00	&	0.19	$\pm$	0.051	&	1.325	$\pm$	0.046	&	1.191	$\pm$	0.026	&	39.39	$\pm$	0.117	&	7.77	$\pm$	0.136	\\
074	&	J102429+052451	&	G	&	0.035	$\pm$	0.000889	&	0.28	$\pm$	0.070	&	1.07	&	0.13	$\pm$	0.032	&	1.567	$\pm$	0.033	&	1.485	$\pm$	0.024	&	41.24	$\pm$	0.095	&	7.87	$\pm$	0.059	\\
075	&	J102732-284201	&	NG	&	0.034	$\pm$	0.000215	&	1.17	$\pm$	0.510	&	3.71	&	0.53	$\pm$	0.231	&	1.525	$\pm$	0.014	&	1.540	$\pm$	0.005	&	41.05	$\pm$	0.279	&	---	$\pm$	---	\\
076	&	J103226+271755	&	NG	&	0.193	$\pm$	0.000009	&	0.47	$\pm$	0.129	&	0.66	&	0.21	$\pm$	0.059	&	---	$\pm$	---	&	---	$\pm$	---	&	41.93	$\pm$	0.115	&	8.20	$\pm$	0.170	\\
077	&	J103328+070801	&	G	&	0.046	$\pm$	0.000879	&	1.01	$\pm$	0.213	&	3.05	&	0.46	$\pm$	0.097	&	1.743	$\pm$	0.028	&	1.759	$\pm$	0.023	&	41.85	$\pm$	0.162	&	8.15	$\pm$	0.189	\\
078	&	J103412+014249	&	G	&	0.070	$\pm$	0.000004	&	0.64	$\pm$	0.156	&	0.74	&	0.29	$\pm$	0.071	&	1.615	$\pm$	0.013	&	1.574	$\pm$	0.001	&	40.81	$\pm$	0.135	&	7.84	$\pm$	0.145	\\
079	&	J103509+094516	&	NG	&	0.051	$\pm$	0.000006	&	0.15	$\pm$	0.109	&	6.35	&	0.07	$\pm$	0.050	&	1.626	$\pm$	0.032	&	1.554	$\pm$	0.024	&	40.72	$\pm$	0.099	&	7.98	$\pm$	0.096	\\
080	&	J103726+270759	&	G	&	0.078	$\pm$	0.000005	&	0.62	$\pm$	0.163	&	3.47	&	0.28	$\pm$	0.074	&	1.598	$\pm$	0.016	&	1.601	$\pm$	0.007	&	41.06	$\pm$	0.138	&	8.10	$\pm$	0.193	\\
081	&	J104457+035313	&	NG	&	0.015	$\pm$	0.000027	&	0.17	$\pm$	0.043	&	0.00	&	0.07	$\pm$	0.019	&	1.392	$\pm$	0.040	&	1.404	$\pm$	0.024	&	40.27	$\pm$	0.085	&	7.62	$\pm$	0.045	\\
082	&	J104554+010405	&	G	&	0.028	$\pm$	0.000030	&	0.47	$\pm$	0.095	&	0.00	&	0.21	$\pm$	0.043	&	1.488	$\pm$	0.037	&	1.572	$\pm$	0.024	&	41.20	$\pm$	0.105	&	8.18	$\pm$	0.077	\\
083	&	J104653+134645	&	NG	&	0.012	$\pm$	0.000988	&	0.38	$\pm$	0.080	&	0.00	&	0.17	$\pm$	0.036	&	0.947	$\pm$	0.187	&	1.344	$\pm$	0.025	&	40.24	$\pm$	0.121	&	7.99	$\pm$	0.071	\\
084	&	J104723+302144	&	G	&	0.030	$\pm$	0.000033	&	1.00	$\pm$	0.202	&	0.66	&	0.45	$\pm$	0.092	&	1.606	$\pm$	0.031	&	1.603	$\pm$	0.024	&	41.69	$\pm$	0.160	&	8.17	$\pm$	0.178	\\
085	&	J104755+073951	&	NG	&	0.169	$\pm$	0.000019	&	1.58	$\pm$	0.347	&	10.97	&	0.72	$\pm$	0.158	&	---	$\pm$	---	&	---	$\pm$	---	&	42.40	$\pm$	0.236	&	8.02	$\pm$	0.369	\\
086	&	J104829+111520	&	G	&	0.094	$\pm$	0.000006	&	0.32	$\pm$	0.135	&	3.80	&	0.15	$\pm$	0.061	&	1.529	$\pm$	0.017	&	1.475	$\pm$	0.004	&	41.35	$\pm$	0.110	&	8.11	$\pm$	0.100	\\
087	&	J105032+153806	&	NG	&	0.086	$\pm$	0.000825	&	0.44	$\pm$	0.091	&	0.00	&	0.20	$\pm$	0.041	&	1.596	$\pm$	0.031	&	1.560	$\pm$	0.023	&	41.93	$\pm$	0.103	&	7.98	$\pm$	0.130	\\
088	&	J105040+342947	&	G	&	0.053	$\pm$	0.000855	&	0.37	$\pm$	0.082	&	0.17	&	0.17	$\pm$	0.037	&	1.548	$\pm$	0.018	&	1.520	$\pm$	0.005	&	41.25	$\pm$	0.099	&	8.06	$\pm$	0.067	\\
089	&	J105108+131927	&	G	&	0.047	$\pm$	0.000036	&	0.34	$\pm$	0.113	&	2.48	&	0.15	$\pm$	0.052	&	1.422	$\pm$	0.042	&	1.377	$\pm$	0.025	&	40.77	$\pm$	0.105	&	8.04	$\pm$	0.115	\\
090	&	J105210+032713	&	G	&	0.151	$\pm$	0.000008	&	0.17	$\pm$	0.149	&	14.27	&	0.08	$\pm$	0.068	&	1.593	$\pm$	0.028	&	1.582	$\pm$	0.000	&	41.31	$\pm$	0.119	&	8.18	$\pm$	0.168	\\
091	&	J105326+043014	&	NG	&	0.021	$\pm$	0.000005	&	0.58	$\pm$	0.151	&	3.96	&	0.26	$\pm$	0.068	&	1.246	$\pm$	0.066	&	1.275	$\pm$	0.033	&	40.29	$\pm$	0.123	&	8.02	$\pm$	0.169	\\
092	&	J105331+011740	&	G	&	0.125	$\pm$	0.000006	&	0.28	$\pm$	0.122	&	7.84	&	0.13	$\pm$	0.055	&	1.649	$\pm$	0.014	&	1.630	$\pm$	0.008	&	41.61	$\pm$	0.104	&	8.04	$\pm$	0.136	\\
093	&	J105741+653539	&	G	&	0.011	$\pm$	0.000010	&	0.60	$\pm$	0.120	&	0.00	&	0.27	$\pm$	0.054	&	1.383	$\pm$	0.043	&	1.396	$\pm$	0.026	&	40.06	$\pm$	0.117	&	8.17	$\pm$	0.099	\\
094	&	J105940+080056	&	NG	&	0.029	$\pm$	0.000004	&	1.04	$\pm$	0.207	&	1.73	&	0.47	$\pm$	0.094	&	1.694	$\pm$	0.031	&	1.715	$\pm$	0.025	&	40.95	$\pm$	0.160	&	8.24	$\pm$	0.211	\\
095	&	J110838+223809	&	G	&	0.025	$\pm$	0.000005	&	0.44	$\pm$	0.098	&	0.00	&	0.20	$\pm$	0.044	&	1.419	$\pm$	0.018	&	1.399	$\pm$	0.004	&	40.38	$\pm$	0.104	&	8.06	$\pm$	0.087	\\
096	&	J114212+002003	&	NG	&	0.021	$\pm$	0.002160	&	1.22	$\pm$	0.246	&	0.00	&	0.55	$\pm$	0.112	&	1.905	$\pm$	0.009	&	1.893	$\pm$	0.008	&	41.99	$\pm$	0.202	&	7.76	$\pm$	0.211	\\
097	&	J115023-003141	&	NG	&	0.014	$\pm$	0.000081	&	0.00	$\pm$	0.000	&	0.00	&	0.00	$\pm$	0.000	&	1.272	$\pm$	0.021	&	1.195	$\pm$	0.004	&	39.80	$\pm$	0.081	&	---	$\pm$	---	\\
098	&	J121329+114056	&	G	&	0.022	$\pm$	0.000007	&	0.65	$\pm$	0.135	&	0.00	&	0.30	$\pm$	0.061	&	1.467	$\pm$	0.012	&	1.434	$\pm$	0.004	&	40.67	$\pm$	0.120	&	8.29	$\pm$	0.132	\\
099	&	J121717-280233	&	NG	&	0.028	$\pm$	0.000174	&	0.76	$\pm$	0.394	&	0.00	&	0.34	$\pm$	0.179	&	1.393	$\pm$	0.021	&	1.366	$\pm$	0.001	&	40.85	$\pm$	0.227	&	---	$\pm$	---	\\
100	&	J125305-031258	&	NG	&	0.024	$\pm$	0.001478	&	0.00	$\pm$	0.000	&	33.00	&	0.00	$\pm$	0.000	&	1.775	$\pm$	0.010	&	1.778	$\pm$	0.005	&	41.78	$\pm$	0.083	&	---	$\pm$	---	\\
101	&	J130119+123959	&	NG	&	0.070	$\pm$	0.000766	&	1.54	$\pm$	0.315	&	0.00	&	0.70	$\pm$	0.143	&	1.854	$\pm$	0.008	&	1.842	$\pm$	0.003	&	42.26	$\pm$	0.210	&	8.20	$\pm$	0.256	\\
102	&	J131235+125743	&	G	&	0.027	$\pm$	0.000005	&	0.65	$\pm$	0.149	&	2.89	&	0.30	$\pm$	0.068	&	1.434	$\pm$	0.016	&	1.396	$\pm$	0.001	&	40.78	$\pm$	0.145	&	8.16	$\pm$	0.127	\\
103	&	J132347-013252	&	NG	&	0.024	$\pm$	0.000031	&	0.41	$\pm$	0.112	&	0.91	&	0.18	$\pm$	0.051	&	1.335	$\pm$	0.019	&	1.300	$\pm$	0.003	&	40.53	$\pm$	0.087	&	7.88	$\pm$	0.106	\\
104	&	J132549+330354	&	G	&	0.015	$\pm$	0.000113	&	0.25	$\pm$	0.072	&	2.64	&	0.11	$\pm$	0.033	&	1.419	$\pm$	0.017	&	1.402	$\pm$	0.003	&	40.27	$\pm$	0.092	&	8.22	$\pm$	0.057	\\
105	&	J133708-325528	&	NG	&	0.014	$\pm$	0.000081	&	0.11	$\pm$	0.109	&	0.00	&	0.05	$\pm$	0.049	&	1.223	$\pm$	0.025	&	1.162	$\pm$	0.002	&	40.00	$\pm$	0.120	&	---	$\pm$	---	\\
106	&	J134531+044232	&	G	&	0.031	$\pm$	0.000824	&	0.59	$\pm$	0.124	&	0.58	&	0.27	$\pm$	0.056	&	1.552	$\pm$	0.018	&	1.480	$\pm$	0.009	&	41.11	$\pm$	0.098	&	8.10	$\pm$	0.102	\\
107	&	J142342+225728	&	NG	&	0.033	$\pm$	0.000018	&	0.38	$\pm$	0.077	&	0.00	&	0.17	$\pm$	0.035	&	1.689	$\pm$	0.014	&	1.709	$\pm$	0.012	&	40.92	$\pm$	0.130	&	7.71	$\pm$	0.074	\\
108	&	J144805-011057	&	G	&	0.028	$\pm$	0.000047	&	0.63	$\pm$	0.125	&	0.00	&	0.29	$\pm$	0.057	&	1.690	$\pm$	0.014	&	1.689	$\pm$	0.008	&	41.35	$\pm$	0.093	&	8.12	$\pm$	0.118	\\
109	&	J162152+151855	&	NG	&	0.034	$\pm$	0.000032	&	0.00	$\pm$	0.000	&	8.58	&	0.00	$\pm$	0.000	&	1.734	$\pm$	0.011	&	1.727	$\pm$	0.005	&	41.12	$\pm$	0.054	&	8.18	$\pm$	0.058	\\
110	&	J171236+321633	&	G	&	0.011	$\pm$	0.000004	&	0.24	$\pm$	0.072	&	0.91	&	0.11	$\pm$	0.033	&	1.367	$\pm$	0.017	&	1.363	$\pm$	0.002	&	39.79	$\pm$	0.086	&	7.80	$\pm$	0.066	\\
111	&	J192758-413432	&	NG	&	0.009	$\pm$	0.000060	&	0.00	$\pm$	0.058	&	0.00	&	0.00	$\pm$	0.026	&	1.385	$\pm$	0.020	&	1.346	$\pm$	0.008	&	40.79	$\pm$	0.135	&	---	$\pm$	---	\\
112	&	J210114-055510	&	NG	&	0.195	$\pm$	0.000006	&	0.77	$\pm$	0.162	&	0.00	&	0.35	$\pm$	0.074	&	---	$\pm$	---	&	---	$\pm$	---	&	42.13	$\pm$	0.136	&	8.16	$\pm$	0.159	\\
113	&	J210501-062238	&	G	&	0.142	$\pm$	0.000010	&	0.83	$\pm$	0.203	&	3.14	&	0.37	$\pm$	0.092	&	1.639	$\pm$	0.036	&	1.658	$\pm$	0.024	&	42.16	$\pm$	0.151	&	7.91	$\pm$	0.193	\\
114	&	J211527-075951	&	G	&	0.027	$\pm$	0.000007	&	0.60	$\pm$	0.151	&	5.36	&	0.27	$\pm$	0.069	&	1.397	$\pm$	0.017	&	1.313	$\pm$	0.002	&	40.48	$\pm$	0.139	&	8.22	$\pm$	0.151	\\
115	&	J211902-074226	&	NG	&	0.089	$\pm$	0.000008	&	0.79	$\pm$	0.190	&	13.20	&	0.36	$\pm$	0.086	&	1.432	$\pm$	0.089	&	1.480	$\pm$	0.024	&	41.58	$\pm$	0.143	&	7.91	$\pm$	0.207	\\
116	&	J212043+010006	&	NG	&	0.113	$\pm$	0.000790	&	1.02	$\pm$	0.224	&	2.81	&	0.46	$\pm$	0.102	&	1.853	$\pm$	0.019	&	1.821	$\pm$	0.029	&	41.63	$\pm$	0.175	&	8.00	$\pm$	0.240	\\
117	&	J212332-074831	&	G	&	0.027	$\pm$	0.000008	&	0.71	$\pm$	0.203	&	10.40	&	0.32	$\pm$	0.092	&	1.379	$\pm$	0.049	&	1.332	$\pm$	0.026	&	40.35	$\pm$	0.141	&	8.19	$\pm$	0.230	\\
118	&	J214350-072003	&	NG	&	0.109	$\pm$	0.000010	&	0.30	$\pm$	0.125	&	2.23	&	0.14	$\pm$	0.057	&	1.157	$\pm$	0.235	&	1.707	$\pm$	0.025	&	41.08	$\pm$	0.115	&	7.97	$\pm$	0.128	\\
119	&	J220802+131334	&	NG	&	0.115	$\pm$	0.000007	&	0.79	$\pm$	0.166	&	0.00	&	0.36	$\pm$	0.076	&	1.795	$\pm$	0.029	&	1.785	$\pm$	0.023	&	41.77	$\pm$	0.138	&	7.83	$\pm$	0.163	\\
120	&	J221823+003918	&	G	&	0.107	$\pm$	0.000005	&	1.10	$\pm$	0.241	&	1.90	&	0.50	$\pm$	0.110	&	1.741	$\pm$	0.026	&	1.726	$\pm$	0.008	&	41.32	$\pm$	0.178	&	7.98	$\pm$	0.248	\\
121	&	J222510-001152	&	G	&	0.066	$\pm$	0.000005	&	0.41	$\pm$	0.111	&	3.22	&	0.18	$\pm$	0.051	&	1.616	$\pm$	0.019	&	1.603	$\pm$	0.006	&	41.34	$\pm$	0.105	&	8.00	$\pm$	0.114	\\
122	&	J224556+125022	&	G	&	0.079	$\pm$	0.000008	&	0.74	$\pm$	0.155	&	0.91	&	0.34	$\pm$	0.070	&	1.688	$\pm$	0.029	&	1.626	$\pm$	0.023	&	41.70	$\pm$	0.131	&	8.17	$\pm$	0.170	\\
123	&	J225140+132713	&	G	&	0.061	$\pm$	0.000006	&	0.69	$\pm$	0.151	&	3.63	&	0.31	$\pm$	0.069	&	1.676	$\pm$	0.029	&	1.696	$\pm$	0.023	&	41.83	$\pm$	0.128	&	8.08	$\pm$	0.133	\\
124	&	J230117+135230	&	G	&	0.023	$\pm$	0.000005	&	0.80	$\pm$	0.167	&	0.58	&	0.36	$\pm$	0.076	&	1.382	$\pm$	0.040	&	1.395	$\pm$	0.024	&	40.56	$\pm$	0.139	&	8.08	$\pm$	0.142	\\
125	&	J230123+133314	&	G	&	0.029	$\pm$	0.000894	&	0.81	$\pm$	0.177	&	4.70	&	0.37	$\pm$	0.081	&	1.573	$\pm$	0.032	&	1.571	$\pm$	0.023	&	41.14	$\pm$	0.142	&	8.00	$\pm$	0.146	\\
126	&	J230703+011311	&	NG	&	0.125	$\pm$	0.000010	&	0.40	$\pm$	0.113	&	9.98	&	0.18	$\pm$	0.051	&	1.787	$\pm$	0.027	&	1.758	$\pm$	0.022	&	41.84	$\pm$	0.106	&	8.00	$\pm$	0.210	\\
127	&	J231442+010621	&	G	&	0.033	$\pm$	0.000005	&	0.32	$\pm$	0.178	&	7.26	&	0.14	$\pm$	0.081	&	1.481	$\pm$	0.039	&	1.438	$\pm$	0.024	&	40.27	$\pm$	0.124	&	7.96	$\pm$	0.200	\\
128	&	J232936-011056	&	G	&	0.065	$\pm$	0.000006	&	0.68	$\pm$	0.140	&	0.00	&	0.31	$\pm$	0.064	&	1.578	$\pm$	0.032	&	1.575	$\pm$	0.023	&	41.27	$\pm$	0.126	&	8.13	$\pm$	0.119	\\

\end{longtable}
%\end{ThreePartTable}
\end{center}
\normalsize 
%\end{landscape}
\twocolumn


==> ch04/tab/tab05_old2.tex <==
%Table  5 --- Derived data for the H II galaxies sample
\onecolumn
\begin{landscape}
\scriptsize
\begin{center}
\setlength{\tabcolsep}{4pt}
\begin{longtable}{@{} l c l c c c c c c c c c c c c@{}}
 
\caption{ Derived data for the \hii\ galaxies sample. } 
\label{tab:tab05} \\


%This is the header for the first page of the table...
\hline \hline \\[-2ex]
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} &
\multicolumn{1}{c}{(8)} &
\multicolumn{1}{c}{(9)} &
\multicolumn{1}{c}{(10)} &
\multicolumn{1}{c}{(11)} &
\multicolumn{1}{c}{(12)} & 
\multicolumn{1}{c}{(13)} &
\multicolumn{1}{c}{(14)} &
\multicolumn{1}{c}{(15)} \\

\multicolumn{1}{c}{\bf{Index}} &
%\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{\bf{Flag}} &
\multicolumn{1}{c}{$\mathbf{z_c^{*}}$} &
\multicolumn{1}{c}{$\mathbf{A_v}$} &
\multicolumn{1}{c}{$\mathbf{100 \times Q}$} &
\multicolumn{1}{c}{$\mathbf{C_{\hb}}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma ([\Oiii])}$} &
\multicolumn{1}{c}{$\mathbf{\logd L (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{12 + \logd \mathrm{O/H}}$} &
\multicolumn{1}{c}{$\mathbf{T_{e}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{dyn}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{cl}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{ion}}$} &
\multicolumn{1}{c}{$\mathbf{\logd SFR}$} \\

\multicolumn{1}{c}{} &
%\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ (mag)} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{erg\ s^{-1}}$)} & 
\multicolumn{1}{c}{}& 
\multicolumn{1}{c}{($\mathrm{10^4\ K}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} &
\multicolumn{1}{c}{($\mathrm{M_{\odot}\ yr^{-1}}$)} \\[0.5ex] \hline \\[-1.8ex]


\endfirsthead

%This is the header for the remaining page(s) of the table...
%\multicolumn{7}{c}{{\tablename} \thetable{} -- Continued} \\[0.5ex]
%\hline \hline \\[-2ex]

\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} &
\multicolumn{1}{c}{(8)} &
\multicolumn{1}{c}{(9)} &
\multicolumn{1}{c}{(10)} &
\multicolumn{1}{c}{(11)} &
\multicolumn{1}{c}{(12)} & 
\multicolumn{1}{c}{(13)} &
\multicolumn{1}{c}{(14)} &
\multicolumn{1}{c}{(15)} \\

\multicolumn{1}{c}{\bf{Index}} &
%\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{\bf{Flag}} &
\multicolumn{1}{c}{$\mathbf{z_c^{*}}$} &
\multicolumn{1}{c}{$\mathbf{A_v}$} &
\multicolumn{1}{c}{$\mathbf{100 \times Q}$} &
\multicolumn{1}{c}{$\mathbf{C_{\hb}}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{\logd \sigma ([\Oiii])}$} &
\multicolumn{1}{c}{$\mathbf{\logd L (\hb)}$} &
\multicolumn{1}{c}{$\mathbf{12 + \logd \mathrm{O/H}}$} &
\multicolumn{1}{c}{$\mathbf{T_{e}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{dyn}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{cl}}$} &
\multicolumn{1}{c}{$\mathbf{\logd M_{ion}}$} &
\multicolumn{1}{c}{$\mathbf{\logd SFR}$} \\

\multicolumn{1}{c}{} &
%\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ (mag)} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{km\ s^{-1}}$)} & 
\multicolumn{1}{c}{($\mathrm{erg\ s^{-1}}$)} & 
\multicolumn{1}{c}{}& 
\multicolumn{1}{c}{($\mathrm{10^4\ K}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} & 
\multicolumn{1}{c}{($\mathrm{M_{\odot}}$)} &
\multicolumn{1}{c}{($\mathrm{M_{\odot}\ yr^{-1}}$)} \\[0.5ex] \hline \\[-1.8ex]

\endhead



\multicolumn{8}{l}{{Continued on Next Page\ldots}} \\
\endfoot


\\[-1.8ex] \hline 
\multicolumn{8}{l}{$^*$ The errors in redshift are expressed as multiples of $10^{-5}$.}\\ 
\endlastfoot
001	&	G	&	0.07252	(0.6)	&	0.66	$\pm$	0.20	&	0.00	&	0.30	$\pm$	0.07	&	---	&	1.551	$\pm$	0.027	&	41.31	$\pm$	0.10	&	8.06	$\pm$	0.16	&	1.33	$\pm$	0.16	&	9.30	$\pm$	0.03	&	8.05	$\pm$	0.13	&	6.86	$\pm$	0.08	&	0.38	$\pm$	0.13	\\
002	&	NG	&	0.02203	(0.5)	&	1.41	$\pm$	0.28	&	0.01	&	0.64	$\pm$	0.12	&	1.377	$\pm$	0.039	&	1.324	$\pm$	0.026	&	40.88	$\pm$	0.15	&	8.06	$\pm$	0.19	&	1.27	$\pm$	0.21	&	8.64	$\pm$	0.03	&	7.86	$\pm$	0.20	&	6.49	$\pm$	0.08	&	0.20	$\pm$	0.20	\\
003	&	NG	&	0.05191	(3.5)	&	1.06	$\pm$	0.24	&	0.00	&	0.48	$\pm$	0.09	&	1.463	$\pm$	0.036	&	1.507	$\pm$	0.024	&	41.31	$\pm$	0.13	&	8.15	$\pm$	0.18	&	1.26	$\pm$	0.17	&	7.92	$\pm$	0.10	&	8.28	$\pm$	0.16	&	7.16	$\pm$	0.10	&	0.62	$\pm$	0.16	\\
004	&	NG	&	0.01257	(0.6)	&	0.36	$\pm$	0.10	&	0.06	&	0.17	$\pm$	0.04	&	1.538	$\pm$	0.034	&	1.497	$\pm$	0.026	&	40.26	$\pm$	0.06	&	8.20	$\pm$	0.08	&	1.03	$\pm$	0.05	&	8.74	$\pm$	0.03	&	7.16	$\pm$	0.08	&	6.12	$\pm$	0.07	&	-0.50	$\pm$	0.08	\\
005	&	NG	&	0.01636	(97.9)	&	0.04	$\pm$	0.06	&	0.05	&	0.02	$\pm$	0.02	&	1.577	$\pm$	0.034	&	1.615	$\pm$	0.023	&	40.41	$\pm$	0.11	&	8.02	$\pm$	0.05	&	1.23	$\pm$	0.05	&	8.76	$\pm$	0.04	&	7.28	$\pm$	0.12	&	6.63	$\pm$	0.07	&	-0.38	$\pm$	0.12	\\
006	&	NG	&	0.03637	(87.9)	&	0.01	$\pm$	0.06	&	0.00	&	0.01	$\pm$	0.01	&	1.454	$\pm$	0.036	&	1.325	$\pm$	0.024	&	40.48	$\pm$	0.06	&	7.80	$\pm$	0.05	&	1.57	$\pm$	0.07	&	8.77	$\pm$	0.04	&	7.36	$\pm$	0.08	&	6.27	$\pm$	0.04	&	-0.30	$\pm$	0.08	\\
007	&	G	&	0.05712	(0.6)	&	0.59	$\pm$	0.18	&	0.01	&	0.27	$\pm$	0.07	&	1.529	$\pm$	0.034	&	1.467	$\pm$	0.024	&	40.85	$\pm$	0.10	&	7.89	$\pm$	0.14	&	1.46	$\pm$	0.25	&	9.08	$\pm$	0.03	&	7.81	$\pm$	0.12	&	6.46	$\pm$	0.08	&	0.14	$\pm$	0.12	\\
008	&	G	&	0.09424	(69.1)	&	0.00	$\pm$	0.10	&	0.04	&	0.00	$\pm$	0.00	&	1.527	$\pm$	0.033	&	1.475	$\pm$	0.024	&	41.12	$\pm$	0.07	&	8.31	$\pm$	0.08	&	1.00	$\pm$	0.07	&	8.79	$\pm$	0.16	&	8.04	$\pm$	0.08	&	7.51	$\pm$	0.04	&	0.38	$\pm$	0.08	\\
009	&	NG	&	0.01812	(0.6)	&	0.20	$\pm$	0.13	&	0.03	&	0.09	$\pm$	0.05	&	1.283	$\pm$	0.042	&	1.178	$\pm$	0.027	&	39.82	$\pm$	0.08	&	8.03	$\pm$	0.11	&	1.34	$\pm$	0.11	&	8.26	$\pm$	0.06	&	6.53	$\pm$	0.29	&	5.75	$\pm$	0.06	&	-1.13	$\pm$	0.29	\\
010	&	G	&	0.01718	(0.4)	&	0.83	$\pm$	0.22	&	0.02	&	0.38	$\pm$	0.09	&	1.369	$\pm$	0.040	&	1.327	$\pm$	0.026	&	40.15	$\pm$	0.11	&	8.03	$\pm$	0.19	&	1.28	$\pm$	0.17	&	8.45	$\pm$	0.08	&	7.37	$\pm$	0.15	&	6.10	$\pm$	0.09	&	-0.29	$\pm$	0.15	\\
011	&	G	&	0.05574	(83.5)	&	0.54	$\pm$	0.13	&	0.01	&	0.24	$\pm$	0.06	&	1.625	$\pm$	0.033	&	1.583	$\pm$	0.023	&	41.18	$\pm$	0.08	&	7.94	$\pm$	0.10	&	1.44	$\pm$	0.12	&	9.29	$\pm$	0.04	&	8.11	$\pm$	0.11	&	6.70	$\pm$	0.06	&	0.45	$\pm$	0.11	\\
012	&	NG	&	0.01207	(0.4)	&	0.86	$\pm$	0.27	&	0.00	&	0.39	$\pm$	0.09	&	1.144	$\pm$	0.060	&	1.176	$\pm$	0.028	&	39.73	$\pm$	0.13	&	7.94	$\pm$	0.25	&	1.50	$\pm$	0.29	&	7.89	$\pm$	0.05	&	6.65	$\pm$	0.15	&	5.82	$\pm$	0.11	&	-1.01	$\pm$	0.15	\\
013	&	G	&	0.11235	(0.7)	&	0.36	$\pm$	0.14	&	0.00	&	0.17	$\pm$	0.04	&	1.706	$\pm$	0.033	&	1.601	$\pm$	0.023	&	41.72	$\pm$	0.08	&	8.07	$\pm$	0.12	&	1.25	$\pm$	0.11	&	9.25	$\pm$	0.04	&	8.69	$\pm$	0.10	&	7.30	$\pm$	0.07	&	1.02	$\pm$	0.10	\\
014	&	G	&	0.08164	(90.8)	&	0.45	$\pm$	0.16	&	0.00	&	0.21	$\pm$	0.05	&	1.651	$\pm$	0.034	&	1.595	$\pm$	0.023	&	41.56	$\pm$	0.09	&	7.95	$\pm$	0.13	&	1.49	$\pm$	0.16	&	---	&	8.51	$\pm$	0.11	&	6.71	$\pm$	0.05	&	0.85	$\pm$	0.11	\\
015	&	NG	&	0.07687	(0.5)	&	0.33	$\pm$	0.13	&	0.05	&	0.15	$\pm$	0.06	&	1.590	$\pm$	0.034	&	1.563	$\pm$	0.023	&	41.24	$\pm$	0.08	&	7.99	$\pm$	0.10	&	1.31	$\pm$	0.10	&	9.20	$\pm$	0.04	&	8.17	$\pm$	0.11	&	7.62	$\pm$	0.07	&	0.51	$\pm$	0.11	\\
016	&	G	&	0.01420	(0.5)	&	0.23	$\pm$	0.09	&	0.09	&	0.11	$\pm$	0.04	&	1.390	$\pm$	0.038	&	1.400	$\pm$	0.024	&	40.02	$\pm$	0.07	&	7.85	$\pm$	0.07	&	1.40	$\pm$	0.09	&	8.32	$\pm$	0.03	&	6.91	$\pm$	0.09	&	6.15	$\pm$	0.06	&	-0.76	$\pm$	0.09	\\
017	&	NG	&	0.16417	(1.2)	&	0.00	$\pm$	0.12	&	0.08	&	0.00	$\pm$	0.00	&	1.782	$\pm$	0.032	&	1.708	$\pm$	0.023	&	41.68	$\pm$	0.06	&	7.89	$\pm$	0.10	&	1.45	$\pm$	0.11	&	9.73	$\pm$	0.04	&	8.36	$\pm$	0.08	&	6.39	$\pm$	0.04	&	0.70	$\pm$	0.08	\\
018	&	G	&	0.05097	(0.6)	&	0.21	$\pm$	0.13	&	0.06	&	0.10	$\pm$	0.06	&	1.419	$\pm$	0.039	&	1.472	$\pm$	0.024	&	40.68	$\pm$	0.07	&	8.17	$\pm$	0.11	&	1.13	$\pm$	0.09	&	8.66	$\pm$	0.06	&	7.33	$\pm$	0.11	&	6.92	$\pm$	0.04	&	-0.33	$\pm$	0.11	\\
019	&	G	&	0.02282	(0.4)	&	0.54	$\pm$	0.17	&	0.04	&	0.25	$\pm$	0.07	&	1.350	$\pm$	0.041	&	1.248	$\pm$	0.032	&	40.25	$\pm$	0.09	&	7.88	$\pm$	0.14	&	1.47	$\pm$	0.17	&	8.56	$\pm$	0.06	&	7.20	$\pm$	0.13	&	6.63	$\pm$	0.09	&	-0.47	$\pm$	0.13	\\
020	&	G	&	0.07443	(74.0)	&	0.47	$\pm$	0.13	&	0.02	&	0.21	$\pm$	0.06	&	1.548	$\pm$	0.034	&	1.494	$\pm$	0.023	&	41.10	$\pm$	0.08	&	8.15	$\pm$	0.11	&	1.21	$\pm$	0.09	&	9.00	$\pm$	0.07	&	8.37	$\pm$	0.11	&	6.93	$\pm$	0.07	&	0.71	$\pm$	0.11	\\
021	&	NG	&	0.05041	(33.5)	&	0.68	$\pm$	0.65	&	0.00	&	0.31	$\pm$	0.17	&	1.446	$\pm$	0.026	&	1.395	$\pm$	0.006	&	41.19	$\pm$	0.26	&	---	&	---	&	---	&	8.07	$\pm$	0.21	&	---	&	0.40	$\pm$	0.21	\\
022	&	G	&	0.02725	(17.4)	&	1.38	$\pm$	0.77	&	0.01	&	0.62	$\pm$	0.24	&	---	&	---	&	40.94	$\pm$	0.32	&	---	&	---	&	---	&	7.86	$\pm$	0.29	&	---	&	0.20	$\pm$	0.29	\\
023	&	G	&	0.06347	(84.4)	&	0.88	$\pm$	0.25	&	0.00	&	0.40	$\pm$	0.08	&	1.576	$\pm$	0.025	&	1.525	$\pm$	0.008	&	41.26	$\pm$	0.11	&	8.27	$\pm$	0.19	&	1.03	$\pm$	0.13	&	9.06	$\pm$	0.05	&	8.17	$\pm$	0.15	&	7.05	$\pm$	0.10	&	0.51	$\pm$	0.15	\\
024	&	G	&	0.07485	(0.6)	&	0.55	$\pm$	0.21	&	0.00	&	0.25	$\pm$	0.06	&	1.567	$\pm$	0.022	&	1.527	$\pm$	0.004	&	41.03	$\pm$	0.10	&	8.16	$\pm$	0.18	&	1.15	$\pm$	0.15	&	8.88	$\pm$	0.06	&	7.96	$\pm$	0.12	&	6.89	$\pm$	0.07	&	0.30	$\pm$	0.12	\\
025	&	G	&	0.03993	(0.8)	&	0.57	$\pm$	0.14	&	0.07	&	0.26	$\pm$	0.06	&	1.484	$\pm$	0.026	&	1.402	$\pm$	0.007	&	40.84	$\pm$	0.09	&	8.18	$\pm$	0.11	&	1.18	$\pm$	0.10	&	8.84	$\pm$	0.03	&	7.63	$\pm$	0.26	&	6.51	$\pm$	0.09	&	-0.03	$\pm$	0.26	\\
026	&	G	&	0.07051	(77.5)	&	0.50	$\pm$	0.11	&	0.04	&	0.23	$\pm$	0.05	&	1.791	$\pm$	0.032	&	1.714	$\pm$	0.023	&	41.80	$\pm$	0.08	&	8.23	$\pm$	0.08	&	1.06	$\pm$	0.06	&	9.35	$\pm$	0.03	&	8.73	$\pm$	0.11	&	7.54	$\pm$	0.07	&	1.07	$\pm$	0.11	\\
027	&	NG	&	0.02021	(0.5)	&	0.31	$\pm$	0.09	&	0.03	&	0.14	$\pm$	0.04	&	1.463	$\pm$	0.035	&	1.498	$\pm$	0.024	&	40.57	$\pm$	0.11	&	8.10	$\pm$	0.07	&	1.28	$\pm$	0.06	&	8.68	$\pm$	0.03	&	7.46	$\pm$	0.12	&	6.42	$\pm$	0.07	&	-0.20	$\pm$	0.12	\\
028	&	NG	&	0.02077	(0.5)	&	0.39	$\pm$	0.16	&	0.07	&	0.18	$\pm$	0.08	&	1.480	$\pm$	0.026	&	1.492	$\pm$	0.005	&	40.17	$\pm$	0.09	&	8.22	$\pm$	0.17	&	1.08	$\pm$	0.13	&	8.56	$\pm$	0.04	&	7.07	$\pm$	0.12	&	6.51	$\pm$	0.09	&	-0.59	$\pm$	0.12	\\
029	&	NG	&	0.05547	(0.5)	&	0.31	$\pm$	0.11	&	0.08	&	0.14	$\pm$	0.05	&	1.565	$\pm$	0.033	&	1.545	$\pm$	0.024	&	40.97	$\pm$	0.07	&	8.19	$\pm$	0.09	&	1.09	$\pm$	0.08	&	9.24	$\pm$	0.03	&	7.89	$\pm$	0.10	&	7.02	$\pm$	0.06	&	0.23	$\pm$	0.10	\\
030	&	G	&	0.02370	(3.3)	&	0.74	$\pm$	0.16	&	0.06	&	0.33	$\pm$	0.07	&	1.588	$\pm$	0.033	&	1.609	$\pm$	0.024	&	40.81	$\pm$	0.15	&	8.31	$\pm$	0.12	&	0.98	$\pm$	0.08	&	8.88	$\pm$	0.03	&	7.74	$\pm$	0.18	&	7.33	$\pm$	0.14	&	0.07	$\pm$	0.18	\\
031	&	G	&	0.08769	(0.8)	&	0.63	$\pm$	0.22	&	0.03	&	0.29	$\pm$	0.08	&	1.532	$\pm$	0.035	&	1.547	$\pm$	0.002	&	41.06	$\pm$	0.11	&	8.13	$\pm$	0.19	&	1.26	$\pm$	0.18	&	9.22	$\pm$	0.04	&	8.02	$\pm$	0.13	&	6.74	$\pm$	0.09	&	0.36	$\pm$	0.13	\\
032	&	G	&	0.09729	(0.8)	&	0.36	$\pm$	0.11	&	0.06	&	0.17	$\pm$	0.05	&	1.649	$\pm$	0.033	&	1.641	$\pm$	0.023	&	41.53	$\pm$	0.08	&	8.10	$\pm$	0.08	&	1.21	$\pm$	0.08	&	9.01	$\pm$	0.07	&	8.51	$\pm$	0.10	&	7.42	$\pm$	0.08	&	0.85	$\pm$	0.10	\\
033	&	G	&	0.10937	(0.6)	&	0.94	$\pm$	0.26	&	0.00	&	0.43	$\pm$	0.09	&	1.688	$\pm$	0.025	&	1.705	$\pm$	0.006	&	41.83	$\pm$	0.13	&	8.07	$\pm$	0.20	&	1.28	$\pm$	0.21	&	9.31	$\pm$	0.03	&	8.83	$\pm$	0.15	&	7.86	$\pm$	0.10	&	1.16	$\pm$	0.15	\\
034	&	G	&	0.11245	(0.7)	&	0.55	$\pm$	0.16	&	0.05	&	0.25	$\pm$	0.07	&	1.707	$\pm$	0.024	&	1.700	$\pm$	0.005	&	41.54	$\pm$	0.09	&	8.17	$\pm$	0.14	&	1.10	$\pm$	0.13	&	9.55	$\pm$	0.03	&	8.50	$\pm$	0.12	&	7.40	$\pm$	0.08	&	0.84	$\pm$	0.12	\\
035	&	G	&	0.07302	(0.7)	&	0.38	$\pm$	0.13	&	0.01	&	0.16	$\pm$	0.05	&	1.664	$\pm$	0.019	&	1.629	$\pm$	0.009	&	41.25	$\pm$	0.08	&	7.93	$\pm$	0.11	&	1.42	$\pm$	0.12	&	8.92	$\pm$	0.03	&	8.17	$\pm$	0.10	&	7.16	$\pm$	0.08	&	0.51	$\pm$	0.10	\\
036	&	G	&	0.04258	(101.9)	&	0.67	$\pm$	0.15	&	0.06	&	0.34	$\pm$	0.08	&	1.637	$\pm$	0.034	&	1.479	$\pm$	0.024	&	41.38	$\pm$	0.09	&	7.68	$\pm$	0.14	&	1.71	$\pm$	0.20	&	8.77	$\pm$	0.03	&	8.35	$\pm$	0.14	&	6.47	$\pm$	0.12	&	0.68	$\pm$	0.14	\\
037	&	NG	&	0.05156	(79.6)	&	0.64	$\pm$	0.18	&	0.00	&	0.29	$\pm$	0.06	&	---	&	---	&	40.92	$\pm$	0.09	&	8.10	$\pm$	0.14	&	1.05	$\pm$	0.12	&	---	&	7.54	$\pm$	0.12	&	6.31	$\pm$	0.08	&	-0.13	$\pm$	0.12	\\
038	&	G	&	0.08479	(0.9)	&	0.74	$\pm$	0.16	&	0.06	&	0.33	$\pm$	0.08	&	1.652	$\pm$	0.024	&	1.607	$\pm$	0.007	&	41.56	$\pm$	0.10	&	8.04	$\pm$	0.12	&	1.24	$\pm$	0.13	&	9.42	$\pm$	0.03	&	8.52	$\pm$	0.14	&	7.91	$\pm$	0.08	&	0.86	$\pm$	0.14	\\
039	&	NG	&	0.03065	(3.0)	&	1.05	$\pm$	0.23	&	0.00	&	0.48	$\pm$	0.10	&	1.490	$\pm$	0.035	&	1.440	$\pm$	0.024	&	41.15	$\pm$	0.12	&	8.04	$\pm$	0.17	&	1.30	$\pm$	0.18	&	9.15	$\pm$	0.03	&	7.92	$\pm$	0.18	&	7.45	$\pm$	0.11	&	0.26	$\pm$	0.18	\\
040	&	G	&	0.09209	(74.1)	&	1.07	$\pm$	0.22	&	0.00	&	0.48	$\pm$	0.10	&	1.747	$\pm$	0.024	&	1.709	$\pm$	0.005	&	41.93	$\pm$	0.12	&	8.19	$\pm$	0.18	&	1.16	$\pm$	0.14	&	9.43	$\pm$	0.03	&	8.93	$\pm$	0.15	&	7.66	$\pm$	0.10	&	1.27	$\pm$	0.15	\\
041	&	NG	&	0.03127	(3.1)	&	0.60	$\pm$	0.17	&	0.00	&	0.27	$\pm$	0.05	&	1.449	$\pm$	0.035	&	1.440	$\pm$	0.024	&	40.83	$\pm$	0.10	&	---	&	---	&	8.72	$\pm$	0.03	&	7.75	$\pm$	0.12	&	7.16	$\pm$	0.07	&	0.09	$\pm$	0.12	\\
042	&	NG	&	0.01125	(1.0)	&	0.84	$\pm$	0.18	&	0.00	&	0.38	$\pm$	0.07	&	1.406	$\pm$	0.040	&	1.368	$\pm$	0.029	&	40.37	$\pm$	0.10	&	8.06	$\pm$	0.15	&	1.17	$\pm$	0.11	&	7.72	$\pm$	0.05	&	7.13	$\pm$	0.16	&	6.17	$\pm$	0.08	&	-0.53	$\pm$	0.16	\\
043	&	NG	&	0.07687	(79.6)	&	0.55	$\pm$	0.13	&	0.00	&	0.25	$\pm$	0.05	&	1.725	$\pm$	0.032	&	1.565	$\pm$	0.027	&	41.91	$\pm$	0.08	&	8.11	$\pm$	0.10	&	1.26	$\pm$	0.09	&	9.57	$\pm$	0.03	&	8.86	$\pm$	0.11	&	7.71	$\pm$	0.07	&	1.20	$\pm$	0.11	\\
044	&	NG	&	0.09922	(0.6)	&	0.79	$\pm$	0.18	&	0.06	&	0.36	$\pm$	0.08	&	1.766	$\pm$	0.024	&	1.747	$\pm$	0.007	&	41.77	$\pm$	0.10	&	8.19	$\pm$	0.13	&	1.18	$\pm$	0.12	&	9.48	$\pm$	0.03	&	8.54	$\pm$	0.15	&	7.43	$\pm$	0.09	&	0.88	$\pm$	0.15	\\
045	&	G	&	0.12641	(0.9)	&	0.24	$\pm$	0.09	&	0.03	&	0.13	$\pm$	0.04	&	1.646	$\pm$	0.025	&	1.632	$\pm$	0.004	&	41.60	$\pm$	0.07	&	8.13	$\pm$	0.08	&	1.20	$\pm$	0.07	&	9.33	$\pm$	0.04	&	8.56	$\pm$	0.10	&	7.28	$\pm$	0.06	&	0.90	$\pm$	0.10	\\
046	&	G	&	0.04038	(91.8)	&	0.01	$\pm$	0.08	&	0.03	&	0.00	$\pm$	0.02	&	1.566	$\pm$	0.025	&	1.550	$\pm$	0.004	&	40.74	$\pm$	0.07	&	7.87	$\pm$	0.06	&	1.48	$\pm$	0.08	&	9.06	$\pm$	0.05	&	7.62	$\pm$	0.09	&	7.09	$\pm$	0.05	&	-0.04	$\pm$	0.09	\\
047	&	G	&	0.02771	(3.0)	&	0.32	$\pm$	0.08	&	0.03	&	0.15	$\pm$	0.04	&	1.535	$\pm$	0.035	&	1.486	$\pm$	0.024	&	41.02	$\pm$	0.05	&	8.11	$\pm$	0.06	&	1.23	$\pm$	0.05	&	8.88	$\pm$	0.03	&	7.92	$\pm$	0.07	&	6.91	$\pm$	0.05	&	0.25	$\pm$	0.07	\\
048	&	NG	&	0.02293	(0.6)	&	0.50	$\pm$	0.15	&	0.00	&	0.23	$\pm$	0.05	&	1.477	$\pm$	0.035	&	1.451	$\pm$	0.023	&	40.36	$\pm$	0.09	&	8.03	$\pm$	0.12	&	1.32	$\pm$	0.12	&	8.51	$\pm$	0.03	&	7.27	$\pm$	0.11	&	6.17	$\pm$	0.06	&	-0.39	$\pm$	0.11	\\
049	&	G	&	0.05815	(0.4)	&	0.47	$\pm$	0.17	&	0.01	&	0.21	$\pm$	0.06	&	1.614	$\pm$	0.024	&	1.586	$\pm$	0.004	&	40.90	$\pm$	0.09	&	8.32	$\pm$	0.15	&	1.00	$\pm$	0.10	&	8.99	$\pm$	0.04	&	7.82	$\pm$	0.11	&	6.88	$\pm$	0.06	&	0.16	$\pm$	0.11	\\
050	&	G	&	0.07590	(0.5)	&	0.57	$\pm$	0.16	&	0.01	&	0.27	$\pm$	0.06	&	---	&	1.636	$\pm$	0.013	&	41.26	$\pm$	0.09	&	8.06	$\pm$	0.12	&	1.29	$\pm$	0.13	&	9.39	$\pm$	0.04	&	8.21	$\pm$	0.12	&	7.47	$\pm$	0.08	&	0.55	$\pm$	0.12	\\
051	&	G	&	0.10809	(0.7)	&	0.96	$\pm$	0.26	&	0.01	&	0.43	$\pm$	0.09	&	1.737	$\pm$	0.023	&	1.695	$\pm$	0.006	&	41.69	$\pm$	0.13	&	7.88	$\pm$	0.20	&	1.31	$\pm$	0.25	&	9.45	$\pm$	0.05	&	8.70	$\pm$	0.16	&	7.38	$\pm$	0.11	&	1.04	$\pm$	0.16	\\
052	&	G	&	0.09494	(0.5)	&	0.33	$\pm$	0.19	&	0.00	&	0.16	$\pm$	0.05	&	1.561	$\pm$	0.025	&	1.556	$\pm$	0.003	&	41.33	$\pm$	0.10	&	8.06	$\pm$	0.17	&	1.29	$\pm$	0.15	&	9.12	$\pm$	0.05	&	8.34	$\pm$	0.11	&	7.27	$\pm$	0.06	&	0.68	$\pm$	0.11	\\
053	&	G	&	0.01352	(0.9)	&	0.25	$\pm$	0.08	&	0.03	&	0.11	$\pm$	0.03	&	1.441	$\pm$	0.036	&	1.403	$\pm$	0.024	&	40.32	$\pm$	0.06	&	7.98	$\pm$	0.06	&	1.29	$\pm$	0.06	&	8.36	$\pm$	0.04	&	7.25	$\pm$	0.09	&	6.55	$\pm$	0.05	&	-0.41	$\pm$	0.09	\\
054	&	G	&	0.08536	(75.3)	&	0.51	$\pm$	0.15	&	0.00	&	0.22	$\pm$	0.05	&	1.700	$\pm$	0.024	&	1.681	$\pm$	0.004	&	41.46	$\pm$	0.08	&	8.06	$\pm$	0.11	&	1.28	$\pm$	0.12	&	9.40	$\pm$	0.03	&	8.17	$\pm$	0.12	&	7.79	$\pm$	0.08	&	0.51	$\pm$	0.12	\\
055	&	NG	&	0.10263	(71.2)	&	0.44	$\pm$	0.10	&	0.07	&	0.22	$\pm$	0.05	&	1.787	$\pm$	0.031	&	1.756	$\pm$	0.022	&	41.97	$\pm$	0.07	&	8.00	$\pm$	0.08	&	1.17	$\pm$	0.07	&	9.65	$\pm$	0.03	&	8.94	$\pm$	0.11	&	7.94	$\pm$	0.11	&	1.28	$\pm$	0.11	\\
056	&	NG	&	0.04587	(0.7)	&	0.00	$\pm$	0.00	&	0.00	&	0.00	$\pm$	0.00	&	1.602	$\pm$	0.025	&	1.581	$\pm$	0.007	&	40.61	$\pm$	0.05	&	---	&	---	&	8.88	$\pm$	0.03	&	7.49	$\pm$	0.08	&	6.49	$\pm$	0.04	&	-0.17	$\pm$	0.08	\\
057	&	NG	&	0.01558	(1.0)	&	0.24	$\pm$	0.10	&	0.00	&	0.11	$\pm$	0.02	&	1.536	$\pm$	0.034	&	1.501	$\pm$	0.025	&	40.19	$\pm$	0.06	&	7.97	$\pm$	0.08	&	1.31	$\pm$	0.07	&	8.41	$\pm$	0.03	&	6.88	$\pm$	0.11	&	6.16	$\pm$	0.04	&	-0.78	$\pm$	0.11	\\
058	&	NG	&	0.02329	(0.4)	&	0.01	$\pm$	0.18	&	0.02	&	0.00	$\pm$	0.02	&	1.496	$\pm$	0.036	&	1.332	$\pm$	0.026	&	39.93	$\pm$	0.09	&	7.78	$\pm$	0.16	&	1.64	$\pm$	0.23	&	8.89	$\pm$	0.06	&	6.80	$\pm$	0.08	&	5.18	$\pm$	0.05	&	-0.86	$\pm$	0.08	\\
059	&	NG	&	0.01765	(0.6)	&	0.35	$\pm$	0.11	&	0.00	&	0.16	$\pm$	0.04	&	1.434	$\pm$	0.036	&	1.396	$\pm$	0.025	&	40.25	$\pm$	0.07	&	8.14	$\pm$	0.09	&	1.08	$\pm$	0.07	&	8.47	$\pm$	0.03	&	6.94	$\pm$	0.11	&	6.14	$\pm$	0.04	&	-0.72	$\pm$	0.11	\\
060	&	NG	&	0.01822	(0.4)	&	0.44	$\pm$	0.13	&	0.00	&	0.20	$\pm$	0.04	&	1.440	$\pm$	0.035	&	1.453	$\pm$	0.024	&	40.27	$\pm$	0.08	&	---	&	---	&	8.43	$\pm$	0.03	&	7.16	$\pm$	0.10	&	6.53	$\pm$	0.08	&	-0.50	$\pm$	0.10	\\
061	&	NG	&	0.09883	(71.9)	&	0.60	$\pm$	0.16	&	0.00	&	0.28	$\pm$	0.06	&	1.750	$\pm$	0.025	&	1.706	$\pm$	0.006	&	41.64	$\pm$	0.09	&	8.04	$\pm$	0.13	&	1.29	$\pm$	0.12	&	9.19	$\pm$	0.03	&	8.60	$\pm$	0.12	&	7.34	$\pm$	0.08	&	0.94	$\pm$	0.12	\\
062	&	NG	&	0.04662	(81.7)	&	0.53	$\pm$	0.15	&	0.04	&	0.25	$\pm$	0.07	&	1.808	$\pm$	0.032	&	1.682	$\pm$	0.024	&	41.33	$\pm$	0.09	&	8.05	$\pm$	0.12	&	1.29	$\pm$	0.11	&	9.27	$\pm$	0.03	&	8.26	$\pm$	0.12	&	7.27	$\pm$	0.07	&	0.60	$\pm$	0.12	\\
063	&	G	&	0.12029	(68.5)	&	0.72	$\pm$	0.18	&	0.02	&	0.32	$\pm$	0.07	&	1.746	$\pm$	0.025	&	1.691	$\pm$	0.008	&	41.86	$\pm$	0.10	&	8.20	$\pm$	0.15	&	1.07	$\pm$	0.12	&	9.58	$\pm$	0.04	&	8.61	$\pm$	0.14	&	7.55	$\pm$	0.13	&	0.95	$\pm$	0.14	\\
064	&	G	&	0.01578	(0.4)	&	0.35	$\pm$	0.11	&	0.01	&	0.16	$\pm$	0.04	&	1.296	$\pm$	0.044	&	1.241	$\pm$	0.029	&	40.17	$\pm$	0.07	&	7.91	$\pm$	0.09	&	1.42	$\pm$	0.10	&	8.47	$\pm$	0.03	&	7.07	$\pm$	0.10	&	5.81	$\pm$	0.05	&	-0.60	$\pm$	0.10	\\
065	&	G	&	0.01621	(0.5)	&	0.94	$\pm$	0.21	&	0.02	&	0.43	$\pm$	0.09	&	1.425	$\pm$	0.042	&	1.399	$\pm$	0.025	&	40.49	$\pm$	0.11	&	8.06	$\pm$	0.18	&	1.09	$\pm$	0.13	&	8.65	$\pm$	0.03	&	7.24	$\pm$	0.17	&	6.34	$\pm$	0.11	&	-0.42	$\pm$	0.17	\\
066	&	G	&	0.03259	(0.5)	&	0.34	$\pm$	0.20	&	0.00	&	0.16	$\pm$	0.05	&	1.297	$\pm$	0.035	&	1.270	$\pm$	0.000	&	40.14	$\pm$	0.10	&	7.82	$\pm$	0.16	&	1.56	$\pm$	0.22	&	8.26	$\pm$	0.07	&	7.04	$\pm$	0.10	&	6.44	$\pm$	0.06	&	-0.62	$\pm$	0.10	\\
067	&	NG	&	0.02518	(92.6)	&	0.66	$\pm$	0.16	&	0.00	&	0.30	$\pm$	0.06	&	1.532	$\pm$	0.034	&	1.447	$\pm$	0.024	&	40.72	$\pm$	0.10	&	7.86	$\pm$	0.12	&	1.31	$\pm$	0.12	&	8.56	$\pm$	0.03	&	7.64	$\pm$	0.13	&	6.61	$\pm$	0.05	&	-0.02	$\pm$	0.13	\\
068	&	NG	&	0.03964	(81.0)	&	0.91	$\pm$	0.19	&	0.05	&	0.42	$\pm$	0.08	&	1.839	$\pm$	0.032	&	1.807	$\pm$	0.023	&	41.34	$\pm$	0.11	&	8.23	$\pm$	0.14	&	1.04	$\pm$	0.10	&	9.26	$\pm$	0.03	&	8.29	$\pm$	0.15	&	6.87	$\pm$	0.10	&	0.63	$\pm$	0.15	\\
069	&	G	&	0.06244	(93.3)	&	0.22	$\pm$	0.08	&	0.00	&	0.09	$\pm$	0.02	&	1.681	$\pm$	0.042	&	1.578	$\pm$	0.012	&	41.62	$\pm$	0.07	&	7.99	$\pm$	0.07	&	1.31	$\pm$	0.08	&	8.86	$\pm$	0.03	&	8.52	$\pm$	0.09	&	7.26	$\pm$	0.05	&	0.86	$\pm$	0.09	\\
070	&	G	&	0.05564	(77.5)	&	0.68	$\pm$	0.17	&	0.00	&	0.30	$\pm$	0.06	&	1.612	$\pm$	0.025	&	1.573	$\pm$	0.007	&	41.12	$\pm$	0.10	&	8.11	$\pm$	0.12	&	1.20	$\pm$	0.12	&	9.24	$\pm$	0.03	&	8.06	$\pm$	0.12	&	6.96	$\pm$	0.08	&	0.40	$\pm$	0.12	\\
071	&	NG	&	0.14486	(0.5)	&	0.06	$\pm$	0.15	&	0.01	&	0.04	$\pm$	0.03	&	1.709	$\pm$	0.032	&	1.656	$\pm$	0.023	&	41.69	$\pm$	0.08	&	8.03	$\pm$	0.14	&	1.38	$\pm$	0.13	&	---	&	8.42	$\pm$	0.10	&	7.04	$\pm$	0.08	&	0.76	$\pm$	0.10	\\
072	&	NG	&	0.14807	(0.3)	&	0.46	$\pm$	0.14	&	0.10	&	0.21	$\pm$	0.07	&	1.774	$\pm$	0.024	&	1.763	$\pm$	0.001	&	41.82	$\pm$	0.08	&	8.03	$\pm$	0.11	&	1.29	$\pm$	0.12	&	9.69	$\pm$	0.03	&	8.56	$\pm$	0.13	&	8.21	$\pm$	0.08	&	0.90	$\pm$	0.13	\\
073	&	NG	&	0.01390	(0.4)	&	0.42	$\pm$	0.18	&	0.00	&	0.19	$\pm$	0.05	&	1.279	$\pm$	0.044	&	1.191	$\pm$	0.026	&	39.59	$\pm$	0.09	&	7.73	$\pm$	0.14	&	1.60	$\pm$	0.20	&	8.04	$\pm$	0.05	&	6.24	$\pm$	0.12	&	5.34	$\pm$	0.08	&	-1.42	$\pm$	0.12	\\
074	&	G	&	0.03476	(88.9)	&	0.28	$\pm$	0.08	&	0.01	&	0.13	$\pm$	0.03	&	1.560	$\pm$	0.037	&	1.485	$\pm$	0.024	&	41.20	$\pm$	0.07	&	7.87	$\pm$	0.06	&	1.46	$\pm$	0.08	&	9.02	$\pm$	0.03	&	8.09	$\pm$	0.09	&	7.00	$\pm$	0.05	&	0.43	$\pm$	0.10	\\
075	&	NG	&	0.03375	(21.5)	&	1.17	$\pm$	0.71	&	0.04	&	0.53	$\pm$	0.23	&	1.540	$\pm$	0.034	&	1.540	$\pm$	0.005	&	41.00	$\pm$	0.30	&	---	&	---	&	---	&	7.90	$\pm$	0.28	&	---	&	0.24	$\pm$	0.28	\\
076	&	NG	&	0.19347	(0.9)	&	0.47	$\pm$	0.16	&	0.01	&	0.21	$\pm$	0.06	&	---	&	---	&	41.77	$\pm$	0.09	&	8.20	$\pm$	0.13	&	1.13	$\pm$	0.11	&	---	&	8.78	$\pm$	0.11	&	7.41	$\pm$	0.09	&	1.12	$\pm$	0.11	\\
077	&	G	&	0.04583	(87.9)	&	1.03	$\pm$	0.21	&	0.03	&	0.46	$\pm$	0.10	&	1.791	$\pm$	0.033	&	1.759	$\pm$	0.023	&	41.74	$\pm$	0.12	&	8.14	$\pm$	0.14	&	1.04	$\pm$	0.11	&	9.28	$\pm$	0.03	&	8.70	$\pm$	0.16	&	7.42	$\pm$	0.11	&	1.04	$\pm$	0.16	\\
078	&	G	&	0.06988	(0.4)	&	0.63	$\pm$	0.21	&	0.01	&	0.29	$\pm$	0.07	&	1.597	$\pm$	0.022	&	1.574	$\pm$	0.001	&	40.98	$\pm$	0.10	&	7.85	$\pm$	0.16	&	1.58	$\pm$	0.24	&	---	&	7.66	$\pm$	0.14	&	6.98	$\pm$	0.08	&	0.00	$\pm$	0.14	\\
079	&	NG	&	0.05050	(0.6)	&	0.15	$\pm$	0.11	&	0.06	&	0.07	$\pm$	0.05	&	1.630	$\pm$	0.034	&	1.554	$\pm$	0.024	&	40.67	$\pm$	0.07	&	7.98	$\pm$	0.09	&	1.32	$\pm$	0.11	&	8.84	$\pm$	0.04	&	7.57	$\pm$	0.10	&	6.45	$\pm$	0.06	&	-0.09	$\pm$	0.10	\\
080	&	G	&	0.07806	(0.5)	&	0.62	$\pm$	0.19	&	0.03	&	0.28	$\pm$	0.07	&	1.593	$\pm$	0.025	&	1.601	$\pm$	0.007	&	41.21	$\pm$	0.10	&	8.11	$\pm$	0.16	&	1.24	$\pm$	0.17	&	9.31	$\pm$	0.03	&	7.92	$\pm$	0.14	&	6.96	$\pm$	0.09	&	0.25	$\pm$	0.14	\\
081	&	NG	&	0.01453	(2.7)	&	0.16	$\pm$	0.07	&	0.00	&	0.07	$\pm$	0.02	&	1.410	$\pm$	0.038	&	1.404	$\pm$	0.024	&	40.25	$\pm$	0.06	&	7.61	$\pm$	0.05	&	1.80	$\pm$	0.11	&	8.01	$\pm$	0.03	&	7.13	$\pm$	0.09	&	5.81	$\pm$	0.05	&	-0.54	$\pm$	0.09	\\
082	&	G	&	0.02777	(3.0)	&	0.48	$\pm$	0.13	&	0.00	&	0.21	$\pm$	0.04	&	1.593	$\pm$	0.034	&	1.572	$\pm$	0.024	&	41.14	$\pm$	0.08	&	8.17	$\pm$	0.10	&	1.15	$\pm$	0.08	&	8.82	$\pm$	0.04	&	8.05	$\pm$	0.10	&	6.91	$\pm$	0.06	&	0.39	$\pm$	0.10	\\
083	&	NG	&	0.01216	(98.8)	&	0.39	$\pm$	0.12	&	0.00	&	0.17	$\pm$	0.04	&	1.446	$\pm$	0.036	&	1.344	$\pm$	0.025	&	40.20	$\pm$	0.10	&	7.99	$\pm$	0.09	&	1.35	$\pm$	0.09	&	7.43	$\pm$	0.06	&	7.09	$\pm$	0.12	&	6.08	$\pm$	0.08	&	-0.57	$\pm$	0.12	\\
084	&	G	&	0.03039	(3.3)	&	1.00	$\pm$	0.22	&	0.01	&	0.45	$\pm$	0.09	&	1.639	$\pm$	0.033	&	1.603	$\pm$	0.024	&	41.60	$\pm$	0.12	&	8.17	$\pm$	0.16	&	1.13	$\pm$	0.13	&	8.99	$\pm$	0.02	&	8.54	$\pm$	0.16	&	7.44	$\pm$	0.10	&	0.88	$\pm$	0.16	\\
085	&	NG	&	0.16945	(1.9)	&	1.82	$\pm$	0.39	&	0.09	&	0.72	$\pm$	0.16	&	---	&	---	&	42.49	$\pm$	0.19	&	7.84	$\pm$	0.32	&	1.42	$\pm$	0.39	&	---	&	9.26	$\pm$	0.24	&	7.37	$\pm$	0.20	&	1.59	$\pm$	0.24	\\
086	&	G	&	0.09384	(0.6)	&	0.32	$\pm$	0.14	&	0.04	&	0.15	$\pm$	0.06	&	---	&	1.475	$\pm$	0.004	&	41.25	$\pm$	0.08	&	8.12	$\pm$	0.11	&	1.25	$\pm$	0.10	&	9.18	$\pm$	0.04	&	8.20	$\pm$	0.11	&	7.45	$\pm$	0.06	&	0.54	$\pm$	0.11	\\
087	&	NG	&	0.08564	(82.5)	&	0.44	$\pm$	0.11	&	0.00	&	0.20	$\pm$	0.04	&	1.561	$\pm$	0.033	&	1.560	$\pm$	0.023	&	41.83	$\pm$	0.08	&	7.98	$\pm$	0.09	&	1.42	$\pm$	0.10	&	9.08	$\pm$	0.03	&	8.78	$\pm$	0.10	&	7.83	$\pm$	0.07	&	1.12	$\pm$	0.10	\\
088	&	G	&	0.05314	(85.5)	&	0.34	$\pm$	0.12	&	0.01	&	0.17	$\pm$	0.04	&	1.544	$\pm$	0.026	&	1.520	$\pm$	0.005	&	41.18	$\pm$	0.08	&	8.06	$\pm$	0.09	&	1.24	$\pm$	0.08	&	9.05	$\pm$	0.03	&	8.10	$\pm$	0.10	&	7.25	$\pm$	0.05	&	0.44	$\pm$	0.10	\\
089	&	G	&	0.04670	(3.6)	&	0.34	$\pm$	0.13	&	0.02	&	0.15	$\pm$	0.05	&	1.569	$\pm$	0.034	&	1.377	$\pm$	0.025	&	40.72	$\pm$	0.08	&	8.05	$\pm$	0.10	&	1.25	$\pm$	0.12	&	8.89	$\pm$	0.03	&	7.63	$\pm$	0.10	&	7.09	$\pm$	0.07	&	-0.04	$\pm$	0.10	\\
090	&	G	&	0.15134	(0.8)	&	0.18	$\pm$	0.17	&	0.14	&	0.08	$\pm$	0.07	&	1.587	$\pm$	0.032	&	1.582	$\pm$	0.000	&	41.47	$\pm$	0.08	&	8.19	$\pm$	0.17	&	1.11	$\pm$	0.14	&	9.20	$\pm$	0.06	&	8.16	$\pm$	0.12	&	7.04	$\pm$	0.08	&	0.50	$\pm$	0.12	\\
091	&	NG	&	0.02055	(0.5)	&	0.57	$\pm$	0.15	&	0.04	&	0.26	$\pm$	0.07	&	---	&	1.275	$\pm$	0.033	&	40.23	$\pm$	0.09	&	8.03	$\pm$	0.13	&	1.15	$\pm$	0.11	&	7.97	$\pm$	0.03	&	7.14	$\pm$	0.12	&	6.66	$\pm$	0.08	&	-0.52	$\pm$	0.12	\\
092	&	G	&	0.12499	(0.6)	&	0.26	$\pm$	0.12	&	0.08	&	0.13	$\pm$	0.06	&	1.660	$\pm$	0.024	&	1.630	$\pm$	0.008	&	41.51	$\pm$	0.08	&	8.04	$\pm$	0.10	&	1.30	$\pm$	0.11	&	9.37	$\pm$	0.03	&	8.46	$\pm$	0.10	&	7.25	$\pm$	0.08	&	0.80	$\pm$	0.10	\\
093	&	G	&	0.01111	(1.0)	&	0.60	$\pm$	0.16	&	0.00	&	0.27	$\pm$	0.05	&	1.396	$\pm$	0.038	&	1.396	$\pm$	0.026	&	40.01	$\pm$	0.09	&	8.16	$\pm$	0.14	&	1.18	$\pm$	0.10	&	8.53	$\pm$	0.03	&	6.91	$\pm$	0.12	&	5.72	$\pm$	0.06	&	-0.75	$\pm$	0.12	\\
094	&	NG	&	0.02893	(0.4)	&	1.03	$\pm$	0.22	&	0.02	&	0.47	$\pm$	0.09	&	---	&	1.715	$\pm$	0.025	&	40.84	$\pm$	0.12	&	8.24	$\pm$	0.17	&	1.06	$\pm$	0.13	&	9.03	$\pm$	0.03	&	7.80	$\pm$	0.16	&	6.48	$\pm$	0.11	&	0.14	$\pm$	0.16	\\
095	&	G	&	0.02492	(0.5)	&	0.44	$\pm$	0.14	&	0.00	&	0.20	$\pm$	0.04	&	1.434	$\pm$	0.027	&	1.399	$\pm$	0.004	&	40.62	$\pm$	0.08	&	8.06	$\pm$	0.11	&	1.27	$\pm$	0.10	&	8.34	$\pm$	0.03	&	7.23	$\pm$	0.10	&	6.06	$\pm$	0.06	&	-0.43	$\pm$	0.10	\\
096	&	NG	&	0.02141	(216.0)	&	1.21	$\pm$	0.28	&	0.00	&	0.55	$\pm$	0.11	&	1.880	$\pm$	0.023	&	1.893	$\pm$	0.008	&	41.44	$\pm$	0.17	&	7.75	$\pm$	0.21	&	1.26	$\pm$	0.22	&	10.06	$\pm$	0.05	&	8.84	$\pm$	0.20	&	7.71	$\pm$	0.13	&	1.18	$\pm$	0.20	\\
097	&	NG	&	0.01361	(8.1)	&	0.00	$\pm$	0.00	&	0.00	&	0.00	$\pm$	0.00	&	0.992	$\pm$	0.053	&	1.195	$\pm$	0.004	&	39.54	$\pm$	0.01	&	---	&	---	&	8.27	$\pm$	0.03	&	6.65	$\pm$	0.08	&	---	&	-1.01	$\pm$	0.08	\\
098	&	G	&	0.02187	(0.7)	&	0.66	$\pm$	0.15	&	0.00	&	0.30	$\pm$	0.06	&	1.465	$\pm$	0.016	&	1.434	$\pm$	0.004	&	40.61	$\pm$	0.09	&	8.29	$\pm$	0.11	&	1.11	$\pm$	0.08	&	8.57	$\pm$	0.03	&	7.52	$\pm$	0.12	&	6.33	$\pm$	0.08	&	-0.14	$\pm$	0.12	\\
099	&	NG	&	0.02765	(17.4)	&	0.76	$\pm$	0.72	&	0.00	&	0.34	$\pm$	0.18	&	1.407	$\pm$	0.020	&	1.366	$\pm$	0.001	&	40.81	$\pm$	0.28	&	---	&	---	&	---	&	7.70	$\pm$	0.23	&	---	&	0.04	$\pm$	0.23	\\
100	&	NG	&	0.02418	(147.8)	&	0.00	$\pm$	0.00	&	0.33	&	0.00	$\pm$	0.00	&	1.831	$\pm$	0.023	&	1.778	$\pm$	0.005	&	41.76	$\pm$	0.07	&	---	&	---	&	9.17	$\pm$	0.04	&	8.63	$\pm$	0.08	&	7.10	$\pm$	0.10	&	0.97	$\pm$	0.08	\\
101	&	NG	&	0.07027	(76.6)	&	1.53	$\pm$	0.34	&	0.00	&	0.70	$\pm$	0.14	&	1.868	$\pm$	0.023	&	1.842	$\pm$	0.003	&	42.09	$\pm$	0.16	&	8.20	$\pm$	0.25	&	1.04	$\pm$	0.19	&	9.68	$\pm$	0.03	&	9.11	$\pm$	0.21	&	7.69	$\pm$	0.14	&	1.45	$\pm$	0.21	\\
102	&	G	&	0.02671	(0.5)	&	0.65	$\pm$	0.14	&	0.03	&	0.30	$\pm$	0.07	&	1.431	$\pm$	0.022	&	1.396	$\pm$	0.001	&	40.71	$\pm$	0.13	&	8.17	$\pm$	0.10	&	1.18	$\pm$	0.09	&	---	&	7.64	$\pm$	0.14	&	6.69	$\pm$	0.08	&	-0.03	$\pm$	0.14	\\
103	&	NG	&	0.02362	(3.1)	&	0.37	$\pm$	0.14	&	0.02	&	0.18	$\pm$	0.05	&	1.309	$\pm$	0.032	&	1.300	$\pm$	0.003	&	40.47	$\pm$	0.07	&	7.88	$\pm$	0.12	&	1.64	$\pm$	0.17	&	7.72	$\pm$	0.06	&	7.38	$\pm$	0.09	&	5.27	$\pm$	0.06	&	-0.28	$\pm$	0.09	\\
104	&	G	&	0.01508	(11.3)	&	0.24	$\pm$	0.06	&	0.03	&	0.11	$\pm$	0.03	&	1.424	$\pm$	0.027	&	1.402	$\pm$	0.003	&	40.24	$\pm$	0.06	&	8.22	$\pm$	0.05	&	1.13	$\pm$	0.04	&	8.29	$\pm$	0.03	&	7.12	$\pm$	0.09	&	6.03	$\pm$	0.05	&	-0.54	$\pm$	0.09	\\
105	&	NG	&	0.01356	(8.1)	&	0.10	$\pm$	0.69	&	0.00	&	0.05	$\pm$	0.05	&	1.007	$\pm$	0.055	&	1.162	$\pm$	0.002	&	40.00	$\pm$	0.26	&	---	&	---	&	---	&	6.85	$\pm$	0.12	&	---	&	-0.81	$\pm$	0.12	\\
106	&	G	&	0.03138	(82.4)	&	0.59	$\pm$	0.13	&	0.00	&	0.27	$\pm$	0.06	&	1.609	$\pm$	0.024	&	1.480	$\pm$	0.009	&	41.05	$\pm$	0.08	&	8.11	$\pm$	0.10	&	1.23	$\pm$	0.09	&	8.60	$\pm$	0.04	&	7.97	$\pm$	0.10	&	7.40	$\pm$	0.07	&	0.30	$\pm$	0.10	\\
107	&	NG	&	0.03328	(1.8)	&	0.38	$\pm$	0.14	&	0.00	&	0.17	$\pm$	0.04	&	1.683	$\pm$	0.024	&	1.709	$\pm$	0.012	&	40.86	$\pm$	0.13	&	7.71	$\pm$	0.11	&	1.65	$\pm$	0.16	&	8.92	$\pm$	0.03	&	7.77	$\pm$	0.13	&	6.72	$\pm$	0.05	&	0.11	$\pm$	0.13	\\
108	&	G	&	0.02808	(4.7)	&	0.63	$\pm$	0.14	&	0.00	&	0.29	$\pm$	0.06	&	1.688	$\pm$	0.024	&	1.689	$\pm$	0.008	&	41.28	$\pm$	0.07	&	8.12	$\pm$	0.12	&	1.27	$\pm$	0.10	&	8.98	$\pm$	0.03	&	8.20	$\pm$	0.09	&	6.94	$\pm$	0.07	&	0.54	$\pm$	0.09	\\
109	&	NG	&	0.03437	(3.2)	&	0.00	$\pm$	0.06	&	0.08	&	0.00	$\pm$	0.00	&	1.739	$\pm$	0.023	&	1.727	$\pm$	0.005	&	41.10	$\pm$	0.04	&	8.18	$\pm$	0.07	&	1.06	$\pm$	0.05	&	9.26	$\pm$	0.03	&	7.97	$\pm$	0.05	&	6.84	$\pm$	0.04	&	0.31	$\pm$	0.05	\\
110	&	G	&	0.01094	(0.4)	&	0.22	$\pm$	0.08	&	0.01	&	0.11	$\pm$	0.03	&	1.340	$\pm$	0.021	&	1.363	$\pm$	0.002	&	39.76	$\pm$	0.07	&	7.80	$\pm$	0.06	&	1.57	$\pm$	0.08	&	8.22	$\pm$	0.04	&	6.64	$\pm$	0.09	&	6.09	$\pm$	0.08	&	-1.02	$\pm$	0.09	\\
111	&	NG	&	0.00880	(6.0)	&	0.00	$\pm$	0.62	&	0.00	&	0.00	$\pm$	0.03	&	1.494	$\pm$	0.025	&	1.346	$\pm$	0.008	&	40.60	$\pm$	0.24	&	---	&	---	&	---	&	7.64	$\pm$	0.13	&	---	&	-0.02	$\pm$	0.13	\\
112	&	NG	&	0.19521	(0.6)	&	0.78	$\pm$	0.26	&	0.00	&	0.35	$\pm$	0.07	&	---	&	---	&	41.96	$\pm$	0.13	&	8.16	$\pm$	0.20	&	1.19	$\pm$	0.18	&	---	&	8.98	$\pm$	0.14	&	7.82	$\pm$	0.09	&	1.32	$\pm$	0.14	\\
113	&	G	&	0.14186	(1.0)	&	0.83	$\pm$	0.20	&	0.03	&	0.37	$\pm$	0.09	&	---	&	1.658	$\pm$	0.024	&	41.67	$\pm$	0.11	&	7.91	$\pm$	0.15	&	1.37	$\pm$	0.21	&	9.60	$\pm$	0.05	&	9.01	$\pm$	0.15	&	7.19	$\pm$	0.10	&	1.35	$\pm$	0.15	\\
114	&	G	&	0.02711	(0.7)	&	0.59	$\pm$	0.14	&	0.06	&	0.27	$\pm$	0.07	&	1.397	$\pm$	0.017	&	1.313	$\pm$	0.002	&	40.62	$\pm$	0.08	&	8.23	$\pm$	0.11	&	1.07	$\pm$	0.07	&	8.53	$\pm$	0.07	&	7.33	$\pm$	0.14	&	6.73	$\pm$	0.09	&	-0.33	$\pm$	0.14	\\
115	&	NG	&	0.08855	(0.8)	&	0.79	$\pm$	0.20	&	0.13	&	0.36	$\pm$	0.09	&	---	&	1.480	$\pm$	0.024	&	41.47	$\pm$	0.11	&	7.90	$\pm$	0.16	&	1.40	$\pm$	0.19	&	9.24	$\pm$	0.07	&	8.43	$\pm$	0.14	&	7.90	$\pm$	0.11	&	0.77	$\pm$	0.14	\\
116	&	NG	&	0.11270	(79.0)	&	1.02	$\pm$	0.23	&	0.03	&	0.46	$\pm$	0.10	&	1.880	$\pm$	0.025	&	1.821	$\pm$	0.029	&	41.72	$\pm$	0.12	&	8.01	$\pm$	0.17	&	1.29	$\pm$	0.22	&	9.93	$\pm$	0.04	&	8.48	$\pm$	0.17	&	8.01	$\pm$	0.12	&	0.82	$\pm$	0.17	\\
117	&	G	&	0.02662	(0.8)	&	0.70	$\pm$	0.19	&	0.10	&	0.32	$\pm$	0.09	&	1.441	$\pm$	0.036	&	1.332	$\pm$	0.026	&	40.28	$\pm$	0.11	&	8.20	$\pm$	0.17	&	1.10	$\pm$	0.13	&	8.57	$\pm$	0.06	&	7.20	$\pm$	0.14	&	5.91	$\pm$	0.11	&	-0.46	$\pm$	0.14	\\
118	&	NG	&	0.10880	(1.0)	&	0.32	$\pm$	0.16	&	0.02	&	0.14	$\pm$	0.06	&	1.559	$\pm$	0.046	&	1.707	$\pm$	0.025	&	41.25	$\pm$	0.08	&	7.96	$\pm$	0.13	&	1.35	$\pm$	0.14	&	8.27	$\pm$	0.05	&	7.93	$\pm$	0.11	&	6.90	$\pm$	0.08	&	0.27	$\pm$	0.11	\\
119	&	NG	&	0.11506	(0.7)	&	0.80	$\pm$	0.27	&	0.00	&	0.36	$\pm$	0.08	&	1.757	$\pm$	0.033	&	1.785	$\pm$	0.023	&	41.64	$\pm$	0.13	&	7.82	$\pm$	0.20	&	1.59	$\pm$	0.33	&	9.72	$\pm$	0.04	&	8.62	$\pm$	0.14	&	7.69	$\pm$	0.09	&	0.96	$\pm$	0.14	\\
120	&	G	&	0.10726	(0.5)	&	1.11	$\pm$	0.29	&	0.02	&	0.50	$\pm$	0.11	&	1.707	$\pm$	0.025	&	1.726	$\pm$	0.008	&	41.44	$\pm$	0.14	&	7.98	$\pm$	0.23	&	1.38	$\pm$	0.31	&	9.46	$\pm$	0.05	&	8.17	$\pm$	0.18	&	7.62	$\pm$	0.12	&	0.51	$\pm$	0.18	\\
121	&	G	&	0.06551	(0.5)	&	0.41	$\pm$	0.12	&	0.03	&	0.18	$\pm$	0.05	&	1.627	$\pm$	0.031	&	1.603	$\pm$	0.006	&	41.27	$\pm$	0.08	&	7.99	$\pm$	0.10	&	1.38	$\pm$	0.10	&	8.94	$\pm$	0.03	&	8.19	$\pm$	0.10	&	6.96	$\pm$	0.07	&	0.53	$\pm$	0.10	\\
122	&	G	&	0.07928	(0.8)	&	0.74	$\pm$	0.17	&	0.01	&	0.34	$\pm$	0.07	&	1.662	$\pm$	0.033	&	1.626	$\pm$	0.023	&	41.59	$\pm$	0.10	&	8.16	$\pm$	0.13	&	1.08	$\pm$	0.11	&	9.42	$\pm$	0.03	&	8.55	$\pm$	0.13	&	7.29	$\pm$	0.09	&	0.89	$\pm$	0.13	\\
123	&	G	&	0.06094	(0.6)	&	0.70	$\pm$	0.16	&	0.04	&	0.31	$\pm$	0.07	&	1.660	$\pm$	0.033	&	1.696	$\pm$	0.023	&	41.74	$\pm$	0.09	&	8.09	$\pm$	0.11	&	1.22	$\pm$	0.11	&	9.46	$\pm$	0.03	&	8.68	$\pm$	0.13	&	7.61	$\pm$	0.08	&	1.02	$\pm$	0.13	\\
124	&	G	&	0.02283	(0.5)	&	0.79	$\pm$	0.19	&	0.01	&	0.36	$\pm$	0.08	&	1.318	$\pm$	0.046	&	1.395	$\pm$	0.024	&	40.48	$\pm$	0.11	&	8.09	$\pm$	0.14	&	1.23	$\pm$	0.14	&	8.62	$\pm$	0.03	&	7.42	$\pm$	0.14	&	6.77	$\pm$	0.08	&	-0.25	$\pm$	0.14	\\
125	&	G	&	0.02873	(89.4)	&	0.81	$\pm$	0.18	&	0.05	&	0.37	$\pm$	0.08	&	1.568	$\pm$	0.033	&	1.571	$\pm$	0.023	&	41.06	$\pm$	0.11	&	8.00	$\pm$	0.14	&	1.34	$\pm$	0.14	&	9.17	$\pm$	0.03	&	7.99	$\pm$	0.14	&	7.25	$\pm$	0.09	&	0.33	$\pm$	0.14	\\
126	&	NG	&	0.12456	(1.0)	&	0.40	$\pm$	0.11	&	0.10	&	0.18	$\pm$	0.05	&	1.805	$\pm$	0.032	&	1.758	$\pm$	0.022	&	41.71	$\pm$	0.08	&	7.98	$\pm$	0.11	&	1.20	$\pm$	0.13	&	9.55	$\pm$	0.03	&	8.69	$\pm$	0.11	&	7.04	$\pm$	0.10	&	1.03	$\pm$	0.11	\\
127	&	G	&	0.03278	(0.5)	&	0.31	$\pm$	0.18	&	0.07	&	0.14	$\pm$	0.08	&	1.393	$\pm$	0.041	&	1.438	$\pm$	0.024	&	40.23	$\pm$	0.10	&	7.96	$\pm$	0.17	&	1.31	$\pm$	0.21	&	8.75	$\pm$	0.09	&	7.12	$\pm$	0.12	&	6.38	$\pm$	0.09	&	-0.54	$\pm$	0.12	\\
128	&	G	&	0.06479	(0.6)	&	0.69	$\pm$	0.21	&	0.00	&	0.31	$\pm$	0.06	&	1.573	$\pm$	0.033	&	1.575	$\pm$	0.023	&	41.19	$\pm$	0.11	&	8.13	$\pm$	0.16	&	1.25	$\pm$	0.16	&	9.28	$\pm$	0.05	&	8.12	$\pm$	0.13	&	7.51	$\pm$	0.07	&	0.46	$\pm$	0.13	\\

\end{longtable}
%\end{ThreePartTable}
\end{center}
\normalsize 
\end{landscape}
\twocolumn


==> ch04/tab/tab06.tex <==
%Table --- Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the second parameter. }
  \label{tab:tab06}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	33.94	&	3.04	&	0.81	&	0.259	&	87	\\
$R_g$	&	34.20	&	3.15	&	0.66	&	0.267	&	89	\\
$R_r$	&	33.95	&	3.26	&	0.67	&	0.273	&	88	\\
$R_i$	&	33.83	&	3.42	&	0.62	&	0.284	&	88	\\
$R_z$	&	33.97	&	3.39	&	0.58	&	0.284	&	88	\\
$O/H + 12$	&	32.06	&	3.77	&	0.38	&	0.298	&	86	\\
$W(H\beta)$	&	34.70	&	3.81	&	0.18	&	0.309	&	92	\\
$(u-i)$	&	34.88	&	3.89	&	0.03	&	0.305	&	86	\\
Ex	&	34.83	&	3.90	&	0.35	&	0.308	&	86	\\




\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab061018B.tex <==
%Table --- Bayesian Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Bayesian Regression coefficients for S4}%. Profiles $< 10\%$ - Log$\sigma < $1.80}
  \label{tab:tab061018B}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	33.81	$\pm$	0.38	&	3.24	$\pm$	0.29	&	0.75	$\pm$	0.16	&	0.262	&	88	\\
$R_g$	&	33.89	$\pm$	0.38	&	3.30	$\pm$	0.28	&	0.68	$\pm$	0.14	&	0.271	&	90	\\
$R_r$	&	33.76	$\pm$	0.42	&	3.45	$\pm$	0.29	&	0.63	$\pm$	0.16	&	0.276	&	89	\\
$R_i$	&	33.53	$\pm$	0.49	&	3.56	$\pm$	0.28	&	0.65	$\pm$	0.19	&	0.287	&	89	\\
$R_z$	&	33.16	$\pm$	0.49	&	3.33	$\pm$	0.28	&	0.88	$\pm$	0.20	&	0.294	&	89	\\
$O/H$	&	30.80	$\pm$	3.96	&	3.92	$\pm$	0.32	&	0.51	$\pm$	0.52	&	0.301	&	87	\\
$N2$	&	34.84	$\pm$	0.63	&	4.02	$\pm$	0.31	&	0.10	$\pm$	0.15	&	0.303	&	89	\\
$R23$	&	33.87	$\pm$	0.75	&	4.17	$\pm$	0.28	&	0.70	$\pm$	0.52	&	0.307	&	89	\\
$W(H\beta)$	&	34.27	$\pm$	0.61	&	4.05	$\pm$	0.26	&	0.21	$\pm$	0.20	&	0.311	&	93	\\
$(u-i)$	&	34.65	$\pm$	0.41	&	4.06	$\pm$	0.27	&	0.01	$\pm$	0.09	&	0.308	&	90	\\









\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab061019.tex <==
%Table --- Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {REMOVE-Regression coefficients. Profiles $< 10\%$ - Log$\sigma < $1.90}

  \label{tab:tab061019}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	34.35	&	2.73	&	0.84	&	0.273	&	92	\\
$R_g$	&	34.56	&	2.83	&	0.70	&	0.278	&	94	\\
$R_r$	&	34.32	&	2.91	&	0.72	&	0.285	&	93	\\
$R_i$	&	34.19	&	3.06	&	0.68	&	0.296	&	93	\\
$R_z$	&	34.34	&	3.03	&	0.64	&	0.295	&	93	\\
$O/H$	&	31.89	&	3.39	&	0.47	&	0.312	&	91	\\
$N2$	&	35.78	&	3.42	&	0.08	&	0.311	&	91	\\
$W(H\beta)$	&	35.22	&	3.46	&	0.18	&	0.322	&	97	\\
$(u-i)$	&	35.48	&	3.50	&	0.03	&	0.321	&	91	\\







\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab06A19.tex <==
%Table --- Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Regression coefficients. All Profiles  - Log$\sigma < $1.90}
  \label{tab:tab06A19}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	34.46	$\pm$	0.34	&	2.83	$\pm$	0.20	&	0.74	$\pm$	0.13	&	0.274	&	106	\\
$R_g$	&	34.67	$\pm$	0.33	&	2.95	$\pm$	0.20	&	0.60	$\pm$	0.12	&	0.281	&	110	\\
$R_r$	&	34.48	$\pm$	0.37	&	3.02	$\pm$	0.20	&	0.61	$\pm$	0.13	&	0.286	&	108	\\
$R_i$	&	34.52	$\pm$	0.44	&	3.20	$\pm$	0.20	&	0.50	$\pm$	0.14	&	0.298	&	109	\\
$R_z$	&	34.47	$\pm$	0.45	&	3.08	$\pm$	0.20	&	0.57	$\pm$	0.14	&	0.291	&	108	\\
$O/H$	&	31.77	$\pm$	0.54	&	3.38	$\pm$	0.20	&	0.49	$\pm$	0.21	&	0.305	&	106	\\
$N2$	&	36.00	$\pm$	0.52	&	3.32	$\pm$	0.24	&	0.17	$\pm$	0.12	&	0.308	&	109	\\
$R23$	&		$\pm$		&		$\pm$		&		$\pm$		&		&		\\
$W(H\beta)$	&	35.22	$\pm$	0.47	&	3.40	$\pm$	0.20	&	0.22	$\pm$	0.15	&	0.312	&	114	\\
$(u-i)$	&	35.57	$\pm$	0.32	&	3.43	$\pm$	0.20	&	0.05	$\pm$	0.07	&	0.313	&	110	\\









\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab06A19B.tex <==
%Table --- Bayesian Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Bayesian Regression coefficients. All Profiles  - Log$\sigma < $1.90}
  \label{tab:tab06A19B}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	34.21	$\pm$	0.36	&	3.03	$\pm$	0.23	&	0.72	$\pm$	0.14	&	0.276	&	106	\\
$R_g$	&	34.29	$\pm$	0.35	&	3.13	$\pm$	0.22	&	0.63	$\pm$	0.12	&	0.283	&	110	\\
$R_r$	&	34.19	$\pm$	0.39	&	3.22	$\pm$	0.22	&	0.60	$\pm$	0.14	&	0.287	&	108	\\
$R_i$	&	34.12	$\pm$	0.46	&	3.39	$\pm$	0.22	&	0.53	$\pm$	0.16	&	0.299	&	109	\\
$R_z$	&	33.63	$\pm$	0.45	&	3.16	$\pm$	0.22	&	0.81	$\pm$	0.16	&	0.298	&	108	\\
$O/H$	&	29.23	$\pm$	4.02	&	3.53	$\pm$	0.26	&	0.77	$\pm$	0.52	&	0.311	&	106	\\
$N2$	&	35.43	$\pm$	0.54	&	3.62	$\pm$	0.27	&	0.10	$\pm$	0.13	&	0.311	&	109	\\
$R23$	&		$\pm$		&		$\pm$		&		$\pm$		&		&		\\
$W(H\beta)$	&	34.87	$\pm$	0.49	&	3.62	$\pm$	0.21	&	0.22	$\pm$	0.17	&	0.314	&	114	\\
$(u-i)$	&	35.24	$\pm$	0.34	&	3.64	$\pm$	0.22	&	0.04	$\pm$	0.08	&	0.314	&	110	\\










\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab06All.tex <==
%Table --- Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the second parameter. }
  \label{tab:tab06All}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	33.90	&	3.16	&	0.77	&	0.260	&	98	\\
$R_g$	&	34.16	&	3.30	&	0.59	&	0.269	&	102	\\
$R_r$	&	33.94	&	3.37	&	0.62	&	0.273	&	100	\\
$R_i$	&	33.92	&	3.58	&	0.51	&	0.285	&	101	\\
$R_z$	&	33.93	&	3.44	&	0.57	&	0.280	&	100	\\
$O/H + 12$	&	31.77	&	3.77	&	0.41	&	0.294	&	99	\\
$W(H\beta)$	&	34.67	&	3.78	&	0.21	&	0.303	&	106	\\
$(u-i)$	&	34.86	&	3.89	&	0.07	&	0.301	&	99	\\
Ex	&	34.86	&	3.87	&	0.41	&	0.304	&	99	\\


\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab06old.tex <==
%Table --- Linear regressions 3 
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the second parameter. }
  \label{tab:tab06old}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) \\ 
Parameter & $\alpha$ & $\beta$ & $\gamma$ & rms & N \\
\hline
$R_u$	&	33.30	&	4.26	&	0.40	&	0.206	&	66	\\
$R_g$	&	33.67	&	4.36	&	0.22	&	0.216	&	68	\\
$R_r$	&	33.58	&	4.41	&	0.22	&	0.216	&	68	\\
$R_i$	&	33.72	&	4.51	&	0.11	&	0.219	&	68	\\
$R_z$	&	33.63	&	4.45	&	0.17	&	0.218	&	68	\\
$12 + \log \mathrm{O/H}$	&	32.12	&	4.53	&	0.24	&	0.218	&	68	\\
$W(H\beta)$	&	33.62	&	4.59	&	0.16	&	0.219	&	68	\\
$(u-i)$	&	33.99	&	4.62	&	-0.11	&	0.216	&	68	\\


\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab07.tex <==
%Table --- Linear regressions Multi
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the fourth and fifth parameters. }
  \label{tab:tab07}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_r$, $(u Ð i)$	&	33.57	&	3.11	&	0.95	&	-0.26	&	---	&	0.260	&	88	\\
$R_r$, $O/H + 12$	&	32.58	&	3.26	&	0.63	&	0.19	&	---	&	0.270	&	85	\\
$R_r$, $W(H\beta)$	&	32.82	&	3.17	&	0.81	&	0.44	&	---	&	0.264	&	88	\\
$R_r$, $(u Ð i)$, $O/H + 12$	&	28.65	&	3.01	&	1.10	&	-0.29	&	0.58	&	0.237	&	82	\\
$R_r$, $W(H\beta)$, $O/H + 12$	&	30.00	&	3.12	&	0.77	&	0.49	&	0.36	&	0.259	&	85	\\
$W(H\beta)$, $O/H + 12$	&	31.36	&	3.77	&	0.13	&	0.43	&	---	&	0.297	&	86	\\
$W(H\beta)$, $O/H + 12$, $(u Ð i)$	&	31.45	&	3.82	&	0.07	&	0.43	&	0.01	&	0.297	&	83	\\
$W(H\beta)$, Ex, $(u Ð i)$	&	34.84	&	3.93	&	-0.03	&	0.28	&	0.03	&	0.308	&	83	\\


\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab071018.tex <==
%Table --- Linear regressions Multi
\begin{table*}
 \centering
% \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Regression coefficients for S4.}
    \label{tab:tab071018}
 \resizebox{0.7 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_u$, $(u Ð i)$	&	33.98	$\pm$	0.20	&	2.88	$\pm$	0.25	&	0.94	$\pm$	0.15	&	-0.15	$\pm$	0.08	&	---			&	0.255	&	88	\\
$R_u$, $O/H$	&	32.42	$\pm$	0.25	&	2.97	$\pm$	0.25	&	0.77	$\pm$	0.14	&	0.22	$\pm$	0.21	&	---			&	0.259	&	85	\\
$R_u$, $N2$	&	33.64	$\pm$	0.21	&	2.95	$\pm$	0.25	&	0.97	$\pm$	0.14	&	-0.02	$\pm$	0.12	&	---			&	0.243	&	86	\\
$R_u$, $R23$	&	33.08	$\pm$	0.24	&	3.08	$\pm$	0.25	&	0.84	$\pm$	0.14	&	0.84	$\pm$	0.43	&	---			&	0.256	&	87	\\
$R_u$, $W(H\beta)$	&	32.94	$\pm$	0.23	&	2.88	$\pm$	0.24	&	0.95	$\pm$	0.14	&	0.45	$\pm$	0.17	&	---			&	0.250	&	88	\\
$W(H\beta)$, $O/H$	&	31.43	$\pm$	0.36	&	3.71	$\pm$	0.24	&	0.16	$\pm$	0.20	&	0.43	$\pm$	0.25	&	---			&	0.297	&	87	\\
$W(H\beta)$, $N2$	&	35.38	$\pm$	0.20	&	3.47	$\pm$	0.29	&	0.37	$\pm$	0.27	&	0.38	$\pm$	0.19	&	---			&	0.296	&	89	\\
$W(H\beta)$, $R23$	&	34.57	$\pm$	0.25	&	3.85	$\pm$	0.25	&	-0.02	$\pm$	0.22	&	0.51	$\pm$	0.57	&	---			&	0.304	&	89	\\
$R_u$, $(u Ð i)$, $O/H$	&	30.28	$\pm$	0.32	&	2.79	$\pm$	0.25	&	0.93	$\pm$	0.15	&	-0.23	$\pm$	0.09	&	0.49	$\pm$	0.23	&	0.248	&	85	\\
$R_u$, $(u Ð i)$, $N2$	&	34.02	$\pm$	0.20	&	2.77	$\pm$	0.27	&	1.03	$\pm$	0.15	&	-0.15	$\pm$	0.10	&	0.11	$\pm$	0.14	&	0.239	&	86	\\
$R_u$, $(u Ð i)$, $R23$	&	33.17	$\pm$	0.23	&	3.00	$\pm$	0.25	&	0.94	$\pm$	0.15	&	-0.13	$\pm$	0.08	&	0.70	$\pm$	0.43	&	0.252	&	87	\\
$R_u$, $W(H\beta)$, $O/H$	&	29.36	$\pm$	0.34	&	2.82	$\pm$	0.24	&	0.92	$\pm$	0.14	&	0.55	$\pm$	0.18	&	0.44	$\pm$	0.21	&	0.244	&	85	\\
$R_u$, $W(H\beta)$, $N2$	&	33.17	$\pm$	0.21	&	2.60	$\pm$	0.27	&	1.04	$\pm$	0.14	&	0.65	$\pm$	0.22	&	0.30	$\pm$	0.16	&	0.231	&	86	\\
$R_u$, $W(H\beta)$, $R23$	&	32.66	$\pm$	0.25	&	2.95	$\pm$	0.25	&	0.94	$\pm$	0.15	&	0.37	$\pm$	0.19	&	0.41	$\pm$	0.48	&	0.250	&	87	\\





\hline 
\end{tabular}
}
%\end{minipage}
\end{table*}

==> ch04/tab/tab071018B.tex <==
%Table --- Bayesian Linear regressions Multi
\begin{table*}
 \centering
% \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Bayesian Regression coefficients for S4.}
    \label{tab:tab071018B}
 \resizebox{0.7 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_u$, $(u Ð i)$	&	33.68	$\pm$	0.37	&	3.13	$\pm$	0.29	&	0.91	$\pm$	0.17	&	-0.18	$\pm$	0.09	&	---			&	0.257	&	88	\\
$R_u$, $O/H$	&	32.56	$\pm$	1.97	&	3.25	$\pm$	0.30	&	0.70	$\pm$	0.16	&	0.17	$\pm$	0.26	&	---			&	0.261	&	85	\\
$R_u$, $N2$	&	33.04	$\pm$	0.60	&	3.29	$\pm$	0.29	&	0.93	$\pm$	0.16	&	-0.12	$\pm$	0.13	&	---			&	0.246	&	86	\\
$R_u$, $R23$	&	32.59	$\pm$	0.67	&	3.37	$\pm$	0.30	&	0.80	$\pm$	0.16	&	1.03	$\pm$	0.45	&	---			&	0.258	&	87	\\
$R_u$, $W(H\beta)$	&	32.51	$\pm$	0.60	&	3.11	$\pm$	0.28	&	0.93	$\pm$	0.16	&	0.52	$\pm$	0.19	&	---			&	0.251	&	88	\\
$W(H\beta)$, $O/H$	&	30.95	$\pm$	2.65	&	3.97	$\pm$	0.27	&	0.20	$\pm$	0.22	&	0.43	$\pm$	0.31	&	---			&	0.299	&	87	\\
$W(H\beta)$, $N2$	&	34.78	$\pm$	0.63	&	3.89	$\pm$	0.35	&	0.21	$\pm$	0.32	&	0.21	$\pm$	0.23	&	---			&	0.299	&	89	\\
$W(H\beta)$, $R23$	&	33.91	$\pm$	0.75	&	4.17	$\pm$	0.28	&	-0.01	$\pm$	0.24	&	0.68	$\pm$	0.60	&	---			&	0.307	&	89	\\
$R_u$, $(u Ð i)$, $O/H$	&	29.16	$\pm$	2.41	&	3.00	$\pm$	0.31	&	0.91	$\pm$	0.18	&	-0.29	$\pm$	0.11	&	0.60	$\pm$	0.31	&	0.251	&	85	\\
$R_u$, $(u Ð i)$, $N2$	&	33.35	$\pm$	0.66	&	3.15	$\pm$	0.32	&	0.99	$\pm$	0.17	&	-0.11	$\pm$	0.11	&	-0.01	$\pm$	0.16	&	0.242	&	86	\\
$R_u$, $(u Ð i)$, $R23$	&	32.65	$\pm$	0.66	&	3.27	$\pm$	0.30	&	0.91	$\pm$	0.17	&	-0.14	$\pm$	0.09	&	0.90	$\pm$	0.45	&	0.254	&	87	\\
$R_u$, $W(H\beta)$, $O/H$	&	28.86	$\pm$	2.37	&	3.01	$\pm$	0.30	&	0.90	$\pm$	0.17	&	0.61	$\pm$	0.21	&	0.46	$\pm$	0.28	&	0.246	&	85	\\
$R_u$, $W(H\beta)$, $N2$	&	32.70	$\pm$	0.59	&	2.94	$\pm$	0.34	&	1.01	$\pm$	0.16	&	0.56	$\pm$	0.27	&	0.17	$\pm$	0.19	&	0.234	&	86	\\
$R_u$, $W(H\beta)$, $R23$	&	32.11	$\pm$	0.71	&	3.20	$\pm$	0.30	&	0.92	$\pm$	0.17	&	0.40	$\pm$	0.22	&	0.58	$\pm$	0.51	&	0.252	&	87	\\






\hline 
\end{tabular}
}
%\end{minipage}
\end{table*}

==> ch04/tab/tab071019.tex <==
%Table --- Linear regressions Multi
\begin{table*}
 \centering 
% \begin{minipage}{140mm}
  \caption[Radii Linear regressions]  {Regression coefficients. Profiles $< 10\%$ - Log$\sigma < $1.90}
  \label{tab:tab071019}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_u$, $(u Ð i)$	&	34.24	&	2.69	&	0.94	&	-0.14	&	---	&	0.268	&	92	\\
$R_u$, $O/H + 12$	&	31.27	&	2.67	&	0.80	&	0.41	&	---	&	0.268	&	89	\\
$R_u$, $N2$	&	33.74	&	2.75	&	0.98	&	-0.08	&	---	&	0.250	&	89	\\
$R_u$, $W(H\beta)$	&	33.17	&	2.66	&	0.97	&	0.47	&	---	&	0.262	&	92	\\
$R_u$, $(u Ð i)$, $O/H + 12$	&	27.71	&	2.50	&	1.13	&	-0.19	&	0.79	&	0.239	&	86	\\
$R_u$, $(u Ð i)$, $N2$	&	33.94	&	2.64	&	1.06	&	-0.11	&	0.00	&	0.249	&	87	\\
$R_u$, $W(H\beta)$, $O/H +12$	&	28.13	&	2.53	&	0.98	&	0.59	&	0.62	&	0.251	&	89	\\
$R_u$, $W(H\beta)$, $N2$	&	33.28	&	2.51	&	1.06	&	0.51	&	0.11	&	0.240	&	89	\\
$W(H\beta)$, $O/H + 12$	&	31.09	&	3.39	&	0.16	&	0.53	&	---	&	0.310	&	91	\\
$W(H\beta)$, $N2$	&	35.63	&	3.34	&	0.22	&	0.17	&	---	&	0.309	&	91	\\
$W(H\beta)$, $O/H + 12$, $(u Ð i)$	&	31.17	&	3.42	&	0.14	&	0.52	&	0.02	&	0.312	&	88	\\
$W(H\beta)$, $N2$, $(u Ð i)$	&	35.46	&	3.30	&	0.33	&	0.16	&	0.03	&	0.310	&	89	\\
$W(H\beta)$, Ex, $(u Ð i)$	&	35.27	&	3.65	&	-0.06	&	0.40	&	0.04	&	0.317	&	87	\\



\hline 
\end{tabular}
}
%\end{minipage}
\end{table*}

==> ch04/tab/tab07A19.tex <==
%Table --- Linear regressions Multi
\begin{table*}
 \centering
% \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {REMOVE-Regression coefficients. All Profiles  - Log$\sigma < $1.90}
  \label{tab:tab07A19}
 \resizebox{0.7 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_u$, $(u Ð i)$	&	34.31	&	2.75	&	0.90	&	-0.17	&	---	&	0.268	&	106	\\
$R_u$, $O/H + 12$	&	31.75	&	2.79	&	0.71	&	0.36	&	---	&	0.271	&	102	\\
$R_u$, $N2$	&	34.14	&	2.81	&	0.86	&	-0.01	&	---	&	0.264	&	103	\\
$R_u$, $W(H\beta)$	&	33.20	&	2.74	&	0.90	&	0.50	&	---	&	0.262	&	106	\\
$W(H\beta)$, $O/H$	&	30.21	&	3.38	&	0.30	&	0.61	&	---	&	0.301	&	106	\\
$W(H\beta)$, $N2$	&	35.75	&	3.10	&	0.47	&	0.40	&	---	&	0.301	&	109	\\
$W(H\beta)$, $O/H $, $(u Ð i)$	&	30.41	&	3.39	&	0.30	&	0.58	&	0.04	&	0.302	&	103	\\
$W(H\beta)$, $N2$, $(u Ð i)$	&	35.59	&	3.11	&	0.50	&	0.36	&	0.05	&	0.305	&	105	\\
$R_u$, $(u Ð i)$, $O/H$	&	28.31	&	2.64	&	1.02	&	-0.25	&	0.73	&	0.246	&	99	\\
$R_u$, $(u Ð i)$, $N2$	&	34.68	&	2.55	&	0.98	&	-0.20	&	0.21	&	0.260	&	101	\\
$R_u$, $W(H\beta)$, $O/H$	&	28.45	&	2.67	&	0.87	&	0.62	&	0.58	&	0.253	&	102	\\
$R_u$, $W(H\beta)$, $N2$	&	33.51	&	2.49	&	0.95	&	0.68	&	0.29	&	0.250	&	103	\\




\hline 
\end{tabular}
}
%\end{minipage}
\end{table*}

==> ch04/tab/tab07All.tex <==
%Table --- Linear regressions Multi
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the fourth and fifth parameters. }
  \label{tab:tab07all}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_r$, $(u Ð i)$	&	33.58	&	3.21	&	0.89	&	-0.24	&	---	&	0.263	&	100	\\
$R_r$, $O/H + 12$	&	32.89	&	3.38	&	0.57	&	0.14	&	---	&	0.270	&	97	\\
$R_r$, $W(H\beta)$	&	32.71	&	3.25	&	0.78	&	0.48	&	---	&	0.261	&	100	\\
$R_r$, $(u Ð i)$, $O/H + 12$	&	29.78	&	3.21	&	0.97	&	-0.27	&	0.45	&	0.246	&	94	\\
$R_r$, $W(H\beta)$, $O/H + 12$	&	30.07	&	3.23	&	0.72	&	0.53	&	0.34	&	0.257	&	97	\\
$W(H\beta)$, $O/H + 12$	&	30.42	&	3.74	&	0.24	&	0.53	&	---	&	0.290	&	99	\\
$W(H\beta)$, $O/H + 12$, $(u Ð i)$	&	30.61	&	3.79	&	0.23	&	0.49	&	0.05	&	0.290	&	96	\\
$W(H\beta)$, Ex, $(u Ð i)$	&	34.54	&	3.88	&	0.14	&	0.18	&	0.10	&	0.303	&	96	\\


\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab07old.tex <==
%Table --- Linear regressions Multi
\begin{table}
 \centering
 \begin{minipage}{140mm}
  \caption[Radii Linear regressions] {Correlation coefficients for the fourth and fifth parameters. }
  \label{tab:tab07old}
 \resizebox{0.6 \textwidth}{!}{
\begin{tabular} { c c c c c c c c }
\hline
\hline
(1) & (2) & (3) & (4) & (5) & (6) & (7) & (8)\\ 
Parameters & $\alpha$ & $\beta$ & $\gamma$ &  $\delta$ & $\epsilon$ &  rms & N \\
\hline
$R_r$, $(u - i)$	&	33.20	&	4.25	&	0.51	&	-0.26	&	---	&	0.201	&	68	\\
$R_r$, $12 + \log \mathrm{O/H}$	&	31.91	&	4.37	&	0.21	&	0.22	&	---	&	0.215	&	68	\\
$R_r$, $W(H\beta)$	&	32.97	&	4.37	&	0.28	&	0.24	&	---	&	0.212	&	68	\\
$R_r$, $(u - i)$, $12 +\log \mathrm{O/H} $	&	30.46	&	4.17	&	0.52	&	-0.29	&	0.35	&	0.196	&	68	\\
$R_r$, $W(H\beta)$, $12 + \log \mathrm{O/H}$	&	30.41	&	4.30	&	0.28	&	0.30	&	0.31	&	0.209	&	68	\\



\hline 
\end{tabular}
}
\end{minipage}
\end{table}

==> ch04/tab/tab08.tex <==
%Table  8 --- Zero Point Sample Distance Moduli

\onecolumn
%\begin{landscape}
\scriptsize
\begin{center}
\begin{longtable}{ l l l l  l  }
 
\caption{ Distance Moduli for the host galaxies of the GEHR sample. } 
\label{tab:tab08} \\


%This is the header for the first page of the table...
\hline \hline \\[-2ex]
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} \\ 

\multicolumn{1}{c}{\bf{Galaxy}} &
\multicolumn{1}{c}{$\mu$} &
\multicolumn{1}{c}{$D$} &
\multicolumn{1}{c}{\bf{Method}} &
\multicolumn{1}{c}{\bf{Reference}} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{(mag)} &
\multicolumn{1}{c}{(kpc)} &
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{ }  \\[0.5ex] \hline \\[-1.8ex]


\endfirsthead

%This is the header for the remaining page(s) of the table...
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} \\ 

\multicolumn{1}{c}{\bf{Galaxy}} &
\multicolumn{1}{c}{$\mu$} &
\multicolumn{1}{c}{$D$} &
\multicolumn{1}{c}{\bf{Method}} &
\multicolumn{1}{c}{\bf{Reference}} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{(mag)} &
\multicolumn{1}{c}{(kpc)} &
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{ }  \\[0.5ex] \hline \\[-1.8ex]

\endhead

\multicolumn{4}{l}{{Continued on Next Page\ldots}} \\
\endfoot


\\[-1.8ex] \hline 
%Notes 

\endlastfoot
LMC	&	18.64	$\pm$	0.02	&	53.46	$\pm$	2.46	&	Cepheids 	&	\citet{1995ApJ...452..195D}	\\
	&	18.42	$\pm$	0.11	&	48.31	$\pm$	12.24	&	Cepheids 	&	\citet{1997AJ....113...13B}	\\
	&	18.57	$\pm$	0.19	&	51.76	$\pm$	22.64	&	RR Lyrae 	&	\citet{1997ApJ...482...89A}	\\
	&	18.58	$\pm$	0.02	&	52.00	$\pm$	2.39	&	Cepheids 	&	\citet{1997ApJ...486...60D}	\\
	&	18.53	$\pm$	0.04	&	50.82	$\pm$	4.68	&	RR Lyrae 	&	\citet{1997MNRAS.284..761F}	\\
	&	18.26	$\pm$	0.15	&	44.87	$\pm$	15.50	&	RR Lyrae 	&	\citet{1998AyA...330..515F}	\\
	&	18.29	$\pm$	0.17	&	45.50	$\pm$	17.81	&	Cepheids 	&	\citet{1998AyA...335L..81L}	\\
	&	18.37	$\pm$	0.23	&	47.21	$\pm$	25.00	&	RR Lyrae 	&	\citet{1998AyA...335L..81L}	\\
	&	18.44	$\pm$	0.35	&	48.75	$\pm$	39.29	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.50	$\pm$	0.13	&	50.12	$\pm$	15.00	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.53	$\pm$	0.14	&	50.82	$\pm$	16.38	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.57	$\pm$	0.11	&	51.76	$\pm$	13.11	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.59	$\pm$	0.15	&	52.24	$\pm$	18.04	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.60	$\pm$	0.15	&	52.48	$\pm$	18.13	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.62	$\pm$	0.18	&	52.97	$\pm$	21.95	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.74	$\pm$	0.24	&	55.98	$\pm$	30.93	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.77	$\pm$	0.24	&	56.75	$\pm$	31.36	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.86	$\pm$	0.36	&	59.16	$\pm$	49.04	&	Cepheids 	&	\citet{1998ApJ...492..110M}	\\
	&	18.46	$\pm$	0.02	&	49.20	$\pm$	2.27	&	Cepheids 	&	\citet{1998ApJ...496...17G}	\\
	&	18.30	$\pm$	0.07	&	45.71	$\pm$	7.37	&	Eclipsing Binary 	&	\citet{1998ApJ...509L..21G}	\\
	&	18.35	$\pm$	0.07	&	46.77	$\pm$	7.54	&	Eclipsing Binary 	&	\citet{1998ApJ...509L..21G}	\\
	&	18.22	$\pm$	0.13	&	44.06	$\pm$	13.19	&	Eclipsing Binary 	&	\citet{1998ApJ...509L..25U}	\\
	&	18.61	$\pm$	0.28	&	52.72	$\pm$	33.99	&	RR Lyrae 	&	\citet{1999AyA...348L..33G}	\\
	&	18.42	$\pm$	0.30	&	48.31	$\pm$	33.37	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	18.62	$\pm$	0.12	&	52.97	$\pm$	14.64	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	18.62	$\pm$	0.17	&	52.97	$\pm$	20.73	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	18.74	$\pm$	0.13	&	55.98	$\pm$	16.76	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	18.57	$\pm$	0.05	&	51.76	$\pm$	5.96	&	Cepheids 	&	\citet{1999ApJ...522..250S}	\\
	&	18.72	$\pm$	0.09	&	55.46	$\pm$	11.49	&	Cepheids 	&	\citet{1999PASP..111..775F}	\\
	&	18.52	$\pm$	0.18	&	50.58	$\pm$	20.96	&	Cepheids 	&	\citet{2000AyA...356..849G}	\\
	&	18.54	$\pm$	0.19	&	51.05	$\pm$	22.33	&	Cepheids 	&	\citet{2000AyA...356..849G}	\\
	&	18.60	$\pm$	0.11	&	52.48	$\pm$	13.29	&	Cepheids 	&	\citet{2000AyA...356..849G}	\\
	&	18.66	$\pm$	0.15	&	53.95	$\pm$	18.63	&	Cepheids 	&	\citet{2000AyA...356..849G}	\\
	&	18.52	$\pm$	0.02	&	50.58	$\pm$	2.33	&	RR Lyrae 	&	\citet{2000AyA...363L...1K}	\\
	&	18.40	$\pm$	0.07	&	47.86	$\pm$	7.71	&	Eclipsing Binary 	&	\citet{2000AJ....119.1205N}	\\
	&	18.42	$\pm$	0.10	&	48.31	$\pm$	11.12	&	Cepheids 	&	\citet{2000ApJ...533L.107G}	\\
	&	18.50	$\pm$	0.13	&	50.12	$\pm$	15.00	&	Cepheids 	&	\citet{2000ApJS..128..431F}	\\
	&	18.42	$\pm$	0.08	&	48.31	$\pm$	8.90	&	Eclipsing Binary 	&	\citet{2001AyA...366..752G}	\\
	&	18.46	$\pm$	0.06	&	49.20	$\pm$	6.80	&	Eclipsing Binary 	&	\citet{2001AyA...366..752G}	\\
	&	18.42	$\pm$	0.24	&	48.31	$\pm$	26.69	&	Eclipsing Binary 	&	\citet{2002AyA...381..440S}	\\
	&	18.43	$\pm$	0.24	&	48.53	$\pm$	26.82	&	Eclipsing Binary 	&	\citet{2002AyA...381..440S}	\\
	&	18.35	$\pm$	0.03	&	46.77	$\pm$	3.23	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	18.37	$\pm$	0.14	&	47.21	$\pm$	15.22	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	18.38	$\pm$	0.10	&	47.42	$\pm$	10.92	&	RR Lyrae 	&	\citet{2002AJ....123..473B}	\\
	&	18.53	$\pm$	0.10	&	50.82	$\pm$	11.70	&	RR Lyrae 	&	\citet{2002AJ....123..473B}	\\
	&	18.50	$\pm$	0.13	&	50.12	$\pm$	15.00	&	Cepheids 	&	\citet{2002AJ....124.1695B}	\\
	&	18.58	$\pm$	0.15	&	52.00	$\pm$	17.96	&	Cepheids 	&	\citet{2002AJ....124.1695B}	\\
	&	18.31	$\pm$	0.10	&	45.92	$\pm$	10.57	&	Eclipsing Binary 	&	\citet{2002ApJ...564..260F}	\\
	&	18.36	$\pm$	0.10	&	46.99	$\pm$	10.82	&	Eclipsing Binary 	&	\citet{2002ApJ...564..260F}	\\
	&	18.50	$\pm$	0.06	&	50.12	$\pm$	6.92	&	Eclipsing Binary 	&	\citet{2002ApJ...564..260F}	\\
	&	18.52	$\pm$	0.06	&	50.58	$\pm$	6.99	&	Eclipsing Binary 	&	\citet{2002ApJ...564..260F}	\\
	&	18.53	$\pm$	0.05	&	50.82	$\pm$	5.85	&	Cepheids 	&	\citet{2002ApJ...565L..83B}	\\
	&	18.37	$\pm$	0.08	&	47.21	$\pm$	8.70	&	Eclipsing Binary 	&	\citet{2002ApJ...574..771R}	\\
	&	18.38	$\pm$	0.08	&	47.42	$\pm$	8.74	&	Eclipsing Binary 	&	\citet{2002ApJ...574..771R}	\\
	&	18.48	$\pm$	0.13	&	49.66	$\pm$	14.86	&	Cepheids 	&	\citet{2002ApJ...574L..33B}	\\
	&	18.53	$\pm$	0.08	&	50.82	$\pm$	9.36	&	Cepheids 	&	\citet{2002ApJ...574L..33B}	\\
	&	18.55	$\pm$	0.02	&	51.29	$\pm$	2.36	&	Cepheids 	&	\citet{2002ApJ...578..144K}	\\
	&	18.63	$\pm$	0.08	&	53.21	$\pm$	9.80	&	Eclipsing Binary 	&	\citet{2003AyA...402..509C}	\\
	&	18.65	$\pm$	0.10	&	53.70	$\pm$	12.37	&	Cepheids 	&	\citet{2003AyA...410..887G}	\\
	&	18.30	$\pm$	0.04	&	45.71	$\pm$	4.21	&	Cepheids 	&	\citet{2003AJ....125.1261D}	\\
	&	18.32	$\pm$	0.01	&	46.13	$\pm$	1.06	&	Cepheids 	&	\citet{2003AJ....125.1261D}	\\
	&	18.47	$\pm$	0.07	&	49.43	$\pm$	7.97	&	RR Lyrae 	&	\citet{2003AJ....125.1261D}	\\
	&	18.30	$\pm$	0.14	&	45.71	$\pm$	14.73	&	RR Lyrae 	&	\citet{2003AJ....125.1309C}	\\
	&	18.38	$\pm$	0.16	&	47.42	$\pm$	17.47	&	RR Lyrae 	&	\citet{2003AJ....125.1309C}	\\
	&	18.45	$\pm$	0.09	&	48.98	$\pm$	10.15	&	RR Lyrae 	&	\citet{2003AJ....125.1309C}	\\
	&	18.52	$\pm$	0.09	&	50.58	$\pm$	10.48	&	RR Lyrae 	&	\citet{2003AJ....125.1309C}	\\
	&	18.18	$\pm$	0.09	&	43.25	$\pm$	8.96	&	Eclipsing Binary 	&	\citet{2003ApJ...587..685F}	\\
	&	18.23	$\pm$	0.09	&	44.26	$\pm$	9.17	&	Eclipsing Binary 	&	\citet{2003ApJ...587..685F}	\\
	&	18.56	$\pm$	0.03	&	51.52	$\pm$	3.56	&	Cepheids 	&	\citet{2003MNRAS.342L..58K}	\\
	&	18.55	$\pm$	0.03	&	51.29	$\pm$	3.54	&	RR Lyrae 	&	\citet{2003MNRAS.342L..58K}	\\
	&	18.48	$\pm$	0.10	&	49.66	$\pm$	11.43	&	Cepheids 	&	\citet{2003MNRAS.345..269H}	\\
	&	18.51	$\pm$	0.10	&	50.35	$\pm$	11.59	&	Cepheids 	&	\citet{2003MNRAS.345..269H}	\\
	&	18.54	$\pm$	0.10	&	51.05	$\pm$	11.75	&	Cepheids 	&	\citet{2003MNRAS.345..269H}	\\
	&	18.45	$\pm$	0.07	&	48.98	$\pm$	7.89	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.46	$\pm$	0.07	&	49.20	$\pm$	7.93	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.47	$\pm$	0.07	&	49.43	$\pm$	7.97	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.48	$\pm$	0.07	&	49.66	$\pm$	8.00	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.50	$\pm$	0.07	&	50.12	$\pm$	8.08	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.48	$\pm$	0.08	&	49.66	$\pm$	9.15	&	RR Lyrae 	&	\citet{2004AyA...423...97B}	\\
	&	18.43	$\pm$	0.06	&	48.53	$\pm$	6.70	&	RR Lyrae 	&	\citet{2004AJ....127..334A}	\\
	&	18.50	$\pm$	0.05	&	50.12	$\pm$	5.77	&	Cepheids 	&	\citet{2004AJ....128.2239P}	\\
	&	18.50	$\pm$	0.10	&	50.12	$\pm$	11.54	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	18.52	$\pm$	0.01	&	50.58	$\pm$	1.16	&	RR Lyrae 	&	\citet{2004ApJ...610..269D}	\\
	&	18.39	$\pm$	0.05	&	47.64	$\pm$	5.49	&	Cepheids 	&	\citet{2005AyA...434.1077M}	\\
	&	18.51	$\pm$	0.02	&	50.35	$\pm$	2.32	&	Cepheids 	&	\citet{2005AyA...434.1077M}	\\
	&	18.54	$\pm$	0.02	&	51.05	$\pm$	2.35	&	RR Lyrae 	&	\citet{2005AJ....129.2257M}	\\
	&	18.56	$\pm$	0.04	&	51.52	$\pm$	4.75	&	Cepheids 	&	\citet{2005ApJ...627..224G}	\\
	&	18.54	$\pm$	0.02	&	51.05	$\pm$	2.35	&	Cepheids 	&	\citet{2006ApJ...642..834K}	\\
	&	18.41	$\pm$	0.10	&	48.08	$\pm$	11.07	&	Cepheids 	&	\citet{2006ApJ...652.1133M}	\\
	&	18.54	$\pm$	0.15	&	51.05	$\pm$	17.63	&	RR Lyrae 	&	\citet{2006MNRAS.372.1675S}	\\
	&	18.42	$\pm$	0.10	&	48.31	$\pm$	11.12	&	Cepheids 	&	\citet{2007AyA...462..599T}	\\
	&	18.45	$\pm$	0.11	&	48.98	$\pm$	12.41	&	Cepheids 	&	\citet{2007AyA...462..599T}	\\
	&	18.42	$\pm$	0.06	&	48.31	$\pm$	6.67	&	Eclipsing Binary 	&	\citet{2007AyA...473..847V}	\\
	&	18.40	$\pm$	0.10	&	47.86	$\pm$	11.02	&	Cepheids 	&	\citet{2007AyA...476...73F}	\\
	&	18.40	$\pm$	0.05	&	47.86	$\pm$	5.51	&	Cepheids 	&	\citet{2007AJ....133.1810B}	\\
	&	18.50	$\pm$	0.03	&	50.12	$\pm$	3.46	&	Cepheids 	&	\citet{2007AJ....133.1810B}	\\
	&	18.34	$\pm$	0.06	&	46.56	$\pm$	6.43	&	Cepheids 	&	\citet{2007ApJ...671.1640A}	\\
	&	18.39	$\pm$	0.05	&	47.64	$\pm$	5.49	&	Cepheids 	&	\citet{2007MNRAS.379..723V}	\\
	&	18.45	$\pm$	0.04	&	48.98	$\pm$	4.51	&	Cepheids 	&	\citet{2007MNRAS.379..723V}	\\
	&	18.47	$\pm$	0.03	&	49.43	$\pm$	3.41	&	Cepheids 	&	\citet{2007MNRAS.379..723V}	\\
	&	18.52	$\pm$	0.03	&	50.58	$\pm$	3.49	&	Cepheids 	&	\citet{2007MNRAS.379..723V}	\\
	&	18.49	$\pm$	0.11	&	49.89	$\pm$	12.64	&	RR Lyrae 	&	\citet{2008AJ....135...83C}	\\
	&	18.58	$\pm$	0.03	&	52.00	$\pm$	3.59	&	RR Lyrae 	&	\citet{2008AJ....136..272S}	\\
	&	18.44	$\pm$	0.11	&	48.75	$\pm$	12.35	&	RR Lyrae 	&	\citet{2008ApJ...676L.135C}	\\
	&	18.45	$\pm$	0.09	&	48.98	$\pm$	10.15	&	Cepheids 	&	\citet{2008ApJ...684..102B}	\\
	&	18.56	$\pm$	0.09	&	51.52	$\pm$	10.68	&	Cepheids 	&	\citet{2008ApJ...684..102B}	\\
	&	18.53	$\pm$	0.13	&	50.82	$\pm$	15.21	&	RR Lyrae 	&	\citet{2009AyA...502..505B}	\\
	&	18.50	$\pm$	0.06	&	50.12	$\pm$	6.92	&	Eclipsing Binary 	&	\citet{2009ApJ...697..862P}	\\
	&	18.48	$\pm$	0.03	&	49.59	$\pm$	3.77	&	Cepheids 	&	\citet{Freedman2012}	\\
	&	18.49	$\pm$	0.05	&	49.97	$\pm$	1.13	&	Cepheids 	&	\citet{2013Natur.495...76P}	\\
\hline													
LMC Final	&	18.482	$\pm$	0.004	&	49.697	$\pm$	0.458	&	---	&	---	\\
\hline													
SMC	&	19.09	$\pm$	0.02	&	65.77	$\pm$	3.03	&	Cepheids 	&	\citet{1995ApJ...452..195D}	\\
	&	18.84	$\pm$	0.10	&	58.61	$\pm$	13.50	&	Cepheids 	&	\citet{1997AJ....113...13B}	\\
	&	19.00	$\pm$	0.03	&	63.10	$\pm$	4.36	&	Cepheids 	&	\citet{1997ApJ...486...60D}	\\
	&	18.83	$\pm$	0.05	&	58.34	$\pm$	6.72	&	Cepheids 	&	\citet{1997ApJ...491...13K}	\\
	&	18.98	$\pm$	0.02	&	62.52	$\pm$	2.88	&	Cepheids 	&	\citet{1997ApJ...491...13K}	\\
	&	18.98	$\pm$	0.28	&	62.52	$\pm$	40.31	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	19.14	$\pm$	0.15	&	67.30	$\pm$	23.24	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	19.19	$\pm$	0.17	&	68.87	$\pm$	26.96	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	19.28	$\pm$	0.17	&	71.78	$\pm$	28.10	&	Cepheids 	&	\citet{1999ApJ...512..711B}	\\
	&	19.05	$\pm$	0.13	&	64.57	$\pm$	19.33	&	Cepheids 	&	\citet{2000AyA...360L...1K}	\\
	&	19.04	$\pm$	0.17	&	64.27	$\pm$	25.16	&	Cepheids 	&	\citet{2000AyA...363..901G}	\\
	&	19.11	$\pm$	0.11	&	66.37	$\pm$	16.81	&	Cepheids 	&	\citet{2000AyA...363..901G}	\\
	&	18.99	$\pm$	0.05	&	62.81	$\pm$	7.23	&	Cepheids 	&	\citet{2000ApJS..128..431F}	\\
	&	19.01	$\pm$	0.13	&	63.39	$\pm$	18.97	&	Cepheids 	&	\citet{2002ApJ...574L..33B}	\\
	&	19.04	$\pm$	0.11	&	64.27	$\pm$	16.28	&	Cepheids 	&	\citet{2002ApJ...574L..33B}	\\
	&	18.88	$\pm$	0.01	&	59.70	$\pm$	1.37	&	Cepheids 	&	\citet{2003AJ....125.1261D}	\\
	&	18.91	$\pm$	0.04	&	60.53	$\pm$	5.58	&	Cepheids 	&	\citet{2003AJ....125.1261D}	\\
	&	18.86	$\pm$	0.07	&	59.16	$\pm$	9.53	&	RR Lyrae 	&	\citet{2003AJ....125.1261D}	\\
	&	18.89	$\pm$	0.04	&	59.98	$\pm$	5.52	&	Eclipsing Binary 	&	\citet{2003MNRAS.339..157H}	\\
	&	18.88	$\pm$	0.12	&	59.70	$\pm$	16.50	&	Cepheids 	&	\citet{2004AyA...415..531S}	\\
	&	18.93	$\pm$	0.24	&	61.09	$\pm$	33.76	&	RR Lyrae 	&	\citet{2004AJ....128..736W}	\\
	&	18.99	$\pm$	0.05	&	62.81	$\pm$	7.23	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	18.91	$\pm$	0.03	&	60.53	$\pm$	4.18	&	Eclipsing Binary 	&	\citet{2005MNRAS.357..304H}	\\
	&	18.93	$\pm$	0.02	&	61.09	$\pm$	2.81	&	Cepheids 	&	\citet{2006ApJ...642..834K}	\\
	&	18.97	$\pm$	0.03	&	62.23	$\pm$	4.30	&	RR Lyrae 	&	\citet{2009AJ....138.1661S}	\\
	&	18.83	$\pm$	0.01	&	58.34	$\pm$	1.34	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.84	$\pm$	0.01	&	58.61	$\pm$	1.35	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.86	$\pm$	0.01	&	59.16	$\pm$	1.36	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.87	$\pm$	0.03	&	59.43	$\pm$	4.11	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.87	$\pm$	0.02	&	59.43	$\pm$	2.74	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.89	$\pm$	0.01	&	59.98	$\pm$	1.38	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.89	$\pm$	0.04	&	59.98	$\pm$	5.52	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
	&	18.92	$\pm$	0.04	&	60.81	$\pm$	5.60	&	RR Lyrae 	&	\citet{2010MNRAS.402..691D}	\\
\hline													
SMC Final	&	18.885	$\pm$	0.004	&	59.839	$\pm$	0.487	&	---	&	---	\\
\hline													
IC 2574	&	27.89	$\pm$	0.03	&	3784.43	$\pm$	261.42	&	TRGB 	&	\citet{2009ApJS..183...67D}	\\
	&	27.93	$\pm$	0.03	&	3854.78	$\pm$	266.28	&	TRGB 	&	\citet{2009ApJS..183...67D}	\\
	&	28.02	$\pm$	0.22	&	4017.91	$\pm$	2035.35	&	TRGB 	&	\citet{2003AyA...398..479K}	\\
\hline													
IC 2574 Final	&	27.911	$\pm$	0.021	&	3821.23	$\pm$	185.79	&	---	&	---	\\
\hline													
M 101	&	29.34	$\pm$	0.10	&	7379.04	$\pm$	1699.09	&	Cepheids 	&	\citet{1996ApJ...463...26K}	\\
	&	29.05	$\pm$	0.14	&	6456.54	$\pm$	2081.34	&	Cepheids 	&	\citet{1998ApJ...508..491S}	\\
	&	29.21	$\pm$	0.17	&	6950.24	$\pm$	2720.60	&	Cepheids 	&	\citet{1998ApJ...508..491S}	\\
	&	29.20	$\pm$	0.08	&	6918.31	$\pm$	1274.40	&	Cepheids 	&	\citet{2001ApJ...548..564W}	\\
	&	29.04	$\pm$	0.08	&	6426.88	$\pm$	1183.87	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.37	$\pm$	0.01	&	7481.70	$\pm$	172.27	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.45	$\pm$	0.08	&	7762.47	$\pm$	1429.90	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.58	$\pm$	0.09	&	8241.38	$\pm$	1707.88	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.71	$\pm$	0.18	&	8749.84	$\pm$	3626.50	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.77	$\pm$	0.09	&	8994.98	$\pm$	1864.05	&	Cepheids 	&	\citet{2001ApJ...549..721M}	\\
	&	29.13	$\pm$	0.11	&	6698.85	$\pm$	1696.71	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	29.13	$\pm$	0.11	&	6698.85	$\pm$	1696.71	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	29.06	$\pm$	0.11	&	6486.34	$\pm$	1642.89	&	Cepheids 	&	\citet{2001ApJ...553..562N}	\\
	&	29.16	$\pm$	0.09	&	6792.04	$\pm$	1407.53	&	Cepheids 	&	\citet{2001ApJ...553..562N}	\\
	&	29.23	$\pm$	0.07	&	7014.55	$\pm$	1130.61	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	29.26	$\pm$	0.15	&	7112.14	$\pm$	2456.44	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	29.30	$\pm$	0.07	&	7244.36	$\pm$	1167.65	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	29.14	$\pm$	0.09	&	6729.77	$\pm$	1394.63	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	29.24	$\pm$	0.08	&	7046.93	$\pm$	1298.09	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	29.18	$\pm$	0.08	&	6854.88	$\pm$	1262.72	&	Cepheids 	&	\citet{2006ApJS..165..108S}	\\
	&	29.30	$\pm$	0.12	&	7244.36	$\pm$	2008.63	&	TRGB	&	\citet{2012ApJ...760L..14L}	\\
\hline													
M 101 Final	&	29.353	$\pm$	0.009	&	7423.351	$\pm$	154.889	&	---	&	---	\\
\hline													
NGC 6822	&	23.49	$\pm$	0.08	&	498.88	$\pm$	91.90	&	Cepheids 	&	\citet{1996AJ....112.1928G}	\\
	&	23.27	$\pm$	0.18	&	450.82	$\pm$	186.85	&	Cepheids 	&	\citet{2001ApJ...548..564W}	\\
	&	23.22	$\pm$	0.52	&	440.55	$\pm$	527.50	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	23.30	$\pm$	0.40	&	457.09	$\pm$	420.99	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	23.38	$\pm$	0.52	&	474.24	$\pm$	567.83	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	23.36	$\pm$	0.17	&	469.89	$\pm$	183.94	&	RR Lyrae 	&	\citet{2003ApJ...588L..85C}	\\
	&	23.34	$\pm$	0.04	&	465.59	$\pm$	42.88	&	Cepheids 	&	\citet{2004AJ....128.2815P}	\\
	&	23.39	$\pm$	0.08	&	476.43	$\pm$	87.76	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	23.31	$\pm$	0.02	&	459.20	$\pm$	21.15	&	Cepheids 	&	\citet{2006ApJ...647.1056G}	\\
	&	23.31	$\pm$	0.03	&	459.20	$\pm$	31.72	&	Cepheids 	&	\citet{2006ApJS..165..108S}	\\
	&	23.49	$\pm$	0.03	&	498.88	$\pm$	34.46	&	Cepheids 	&	\citet{2009ApJ...693..936M}	\\
	&	23.40	$\pm$	0.05	&	478.63	$\pm$	55.10	&	Cepheids 	&	\citet{2012MNRAS.421.2998F}	\\
\hline													
NGC 6822 Final	&	23.358	$\pm$	0.013	&	469.499	$\pm$	13.798	&	---	&	---	\\
\hline													
M33	&	24.85	$\pm$	0.09	&	933.25	$\pm$	193.40	&	Cepheids 	&	\citet{1997ApJ...491...13K}	\\
	&	24.84	$\pm$	0.16	&	928.97	$\pm$	342.24	&	RR Lyrae 	&	\citet{2000AJ....120.2437S}	\\
	&	24.85	$\pm$	0.13	&	933.25	$\pm$	279.36	&	Miras 	&	\citet{2000MNRAS.313..271P}	\\
	&	24.47	$\pm$	0.13	&	783.43	$\pm$	234.51	&	Cepheids 	&	\citet{2001ApJ...548..564W}	\\
	&	24.56	$\pm$	0.08	&	816.58	$\pm$	150.42	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	24.62	$\pm$	0.08	&	839.46	$\pm$	154.63	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	24.70	$\pm$	0.13	&	870.96	$\pm$	260.71	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	24.77	$\pm$	0.39	&	899.50	$\pm$	807.76	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	24.83	$\pm$	0.12	&	924.70	$\pm$	255.50	&	Cepheids 	&	\citet{2002AyA...389...19P}	\\
	&	24.52	$\pm$	0.14	&	801.68	$\pm$	258.43	&	Cepheids 	&	\citet{2002ApJ...565..959L}	\\
	&	24.52	$\pm$	0.15	&	801.68	$\pm$	276.89	&	Cepheids 	&	\citet{2002ApJ...565..959L}	\\
	&	24.47	$\pm$	0.11	&	783.43	$\pm$	198.43	&	Cepheids 	&	\citet{2004ApJ...608...42S}	\\
	&	24.52	$\pm$	0.14	&	801.68	$\pm$	258.43	&	TRGB	&	\citet{2004MNRAS.350..243M}	\\
	&	24.67	$\pm$	0.08	&	859.01	$\pm$	158.24	&	RR Lyrae 	&	\citet{2006AJ....132.1361S}	\\
	&	24.92	$\pm$	0.12	&	963.83	$\pm$	266.32	&	Eclipsing Binary 	&	\citet{2006ApJ...652..313B}	\\
	&	24.64	$\pm$	0.06	&	847.23	$\pm$	117.05	&	Cepheids 	&	\citet{2006ApJS..165..108S}	\\
	&	24.55	$\pm$	0.28	&	812.83	$\pm$	524.05	&	Cepheids 	&	\citet{2007ApJ...671.1640A}	\\
	&	24.37	$\pm$	0.02	&	748.17	$\pm$	34.45	&	Cepheids 	&	\citet{2009MNRAS.396.1287S}	\\
	&	24.53	$\pm$	0.11	&	805.38	$\pm$	203.99	&	Cepheids 	&	\citet{2009MNRAS.396.1287S}	\\
	&	24.54	$\pm$	0.03	&	809.10	$\pm$	55.89	&	Cepheids 	&	\citet{2009MNRAS.396.1287S}	\\
\hline													
M33 Final	&	24.492	$\pm$	0.013	&	791.554	$\pm$	24.426	&	---	&	---	\\
\hline													
NGC 2366 Final	&	27.680	$\pm$	0.200	&	3435.579	$\pm$	1582.14	&	Cepheids 	&	\citet{1995AJ....110.1640T}	\\
\hline													
NGC 2403	&	27.48	$\pm$	0.24	&	3133.29	$\pm$	1731.52	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	27.54	$\pm$	0.24	&	3221.07	$\pm$	1780.03	&	Cepheids 	&	\citet{Freedman2001}	\\
	&	27.43	$\pm$	0.15	&	3061.96	$\pm$	1057.56	&	Cepheids 	&	\citet{2006ApJS..165..108S}	\\
\hline													
NGC 2403 Final	&	27.465	$\pm$	0.112	&	3111.842	$\pm$	805.308	&	---	&	---	\\
\hline													
NGC 4236 Final	&	28.240	$\pm$	0.220	&	4446.313	$\pm$	2252.363	&	TRGB 	&	\citet{2002AyA...383..125K}	\\
\hline


\end{longtable}
%\end{ThreePartTable}
\end{center}
\normalsize 
%\end{landscape}
\twocolumn

==> ch04/tab/tbl2.tex <==
\onecolumn
%\begin{landscape}
\scriptsize
\begin{center}
\begin{longtable}{@{} l l r r c c c @{}}
 
\caption{ FWHM of $\hb$ and $[\Oiii]\ \lambda \lambda 5007$ lines from the high resolution spectra. } 
\label{tab:tbl2} \\


%This is the header for the first page of the table...
\hline \hline \\[-2ex]
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} \\ 

\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{$\mathbf{\alpha}$(J2000) } &
\multicolumn{1}{c}{$\mathbf{\delta }$ (J2000) } &
\multicolumn{1}{c}{$\mathbf{z_{hel}}$} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{FWHM}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 5007}$ \textbf{FWHM}} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{(deg) } &
\multicolumn{1}{c}{ (deg)} &
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{(\AA)} & 
\multicolumn{1}{c}{(\AA)}  \\[0.5ex] \hline \\[-1.8ex]

\endfirsthead

%This is the header for the remaining page(s) of the table...
\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} \\ 

\multicolumn{1}{c}{(1)} &
\multicolumn{1}{c}{(2)} &
\multicolumn{1}{c}{(3)} &
\multicolumn{1}{c}{(4)} &
\multicolumn{1}{c}{(5)} &
\multicolumn{1}{c}{(6)} & 
\multicolumn{1}{c}{(7)} \\ 

\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{$\mathbf{\alpha}$(J2000) } &
\multicolumn{1}{c}{$\mathbf{\delta }$ (J2000) } &
\multicolumn{1}{c}{$\mathbf{z_{hel}}$} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{FWHM}} &
%\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 4959}$ \textbf{FWHM}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 5007}$ \textbf{FWHM}} \\


\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{(deg) } &
\multicolumn{1}{c}{ (deg)} &
\multicolumn{1}{c}{ } &
\multicolumn{1}{c}{(\AA)} & 
%\multicolumn{1}{c}{(\AA)} & 
\multicolumn{1}{c}{(\AA)}  \\[0.5ex] \hline \\[-1.8ex]

\endhead

\multicolumn{2}{l}{{Continued on Next Page\ldots}} \\
\endfoot


\\[-1.8ex] \hline 
%\insertTableNotes
\endlastfoot
001	&	J000657+005125	&	1.74	&	0.86	&	0.074	$\pm$	0.000006	&	1.98	$\pm$	0.133	&	1.69	$\pm$	0.095	\\
002	&	J001647-104742	&	4.20	&	-10.80	&	0.023	$\pm$	0.000005	&	0.94	$\pm$	0.080	&	0.91	$\pm$	0.050	\\
003	&	J002339-094848	&	5.92	&	-9.81	&	0.053	$\pm$	0.000035	&	0.55	$\pm$	0.236	&	1.43	$\pm$	0.077	\\
004	&	J002425+140410	&	6.11	&	14.07	&	0.014	$\pm$	0.000006	&	1.59	$\pm$	0.123	&	1.30	$\pm$	0.073	\\
005	&	J003218+150014	&	8.08	&	15.00	&	0.018	$\pm$	0.000979	&	1.65	$\pm$	0.118	&	1.69	$\pm$	0.089	\\
006	&	J005147+000940	&	12.95	&	0.16	&	0.038	$\pm$	0.000879	&	1.20	$\pm$	0.093	&	0.91	$\pm$	0.050	\\
007	&	J005602-101009	&	14.01	&	-10.17	&	0.058	$\pm$	0.000006	&	1.46	$\pm$	0.108	&	1.30	$\pm$	0.071	\\
008	&	J013258-085337	&	23.24	&	-8.89	&	0.095	$\pm$	0.000691	&	1.72	$\pm$	0.120	&	1.43	$\pm$	0.077	\\
009	&	J013344+005711	&	23.44	&	0.95	&	0.019	$\pm$	0.000006	&	0.94	$\pm$	0.081	&	0.65	$\pm$	0.037	\\
010	&	J014137-091435	&	25.41	&	-9.24	&	0.018	$\pm$	0.000004	&	1.07	$\pm$	0.087	&	0.91	$\pm$	0.050	\\
011	&	J014707+135629	&	26.78	&	13.94	&	0.057	$\pm$	0.000835	&	1.85	$\pm$	0.127	&	1.69	$\pm$	0.088	\\
012	&	J021852-091218	&	34.72	&	-9.21	&	0.013	$\pm$	0.000004	&	0.81	$\pm$	0.074	&	0.65	$\pm$	0.037	\\
013	&	J022037-092907	&	35.16	&	-9.49	&	0.113	$\pm$	0.000007	&	2.24	$\pm$	0.150	&	1.95	$\pm$	0.102	\\
014	&	J024052-082827	&	40.22	&	-8.47	&	0.082	$\pm$	0.000908	&	1.72	$\pm$	0.121	&	1.82	$\pm$	0.096	\\
015	&	J024453-082137	&	41.22	&	-8.36	&	0.078	$\pm$	0.000005	&	1.85	$\pm$	0.128	&	1.69	$\pm$	0.088	\\
016	&	J025426-004122	&	43.61	&	-0.69	&	0.015	$\pm$	0.000005	&	1.07	$\pm$	0.088	&	1.04	$\pm$	0.056	\\
017	&	J030321-075923	&	45.84	&	-7.99	&	0.165	$\pm$	0.000012	&	2.89	$\pm$	0.184	&	2.73	$\pm$	0.144	\\
018	&	J031023-083432	&	47.60	&	-8.58	&	0.052	$\pm$	0.000006	&	1.46	$\pm$	0.110	&	1.30	$\pm$	0.070	\\
019	&	J033526-003811	&	53.86	&	-0.64	&	0.023	$\pm$	0.000004	&	1.07	$\pm$	0.088	&	0.78	$\pm$	0.050	\\
020	&	J040937-051805	&	62.41	&	-5.30	&	0.075	$\pm$	0.000740	&	1.72	$\pm$	0.125	&	1.43	$\pm$	0.075	\\
021	&	J051519-391741	&	78.83	&	-39.29	&	0.050	$\pm$	0.000335	&	1.22	$\pm$	0.042	&	1.11	$\pm$	0.013	\\
022	&	J064650-374322	&	101.71	&	-37.72	&	0.026	$\pm$	0.000174	&	---	&	---	\\
023	&	J074806+193146	&	117.03	&	19.53	&	0.063	$\pm$	0.000844	&	1.67	$\pm$	0.059	&	1.51	$\pm$	0.027	\\
024	&	J074947+154013	&	117.45	&	15.67	&	0.074	$\pm$	0.000006	&	1.69	$\pm$	0.055	&	1.55	$\pm$	0.015	\\
025	&	J080000+274642	&	120.00	&	27.78	&	0.039	$\pm$	0.000008	&	1.33	$\pm$	0.049	&	1.10	$\pm$	0.017	\\
026	&	J080619+194927	&	121.58	&	19.82	&	0.070	$\pm$	0.000775	&	2.37	$\pm$	0.155	&	2.34	$\pm$	0.124	\\
027	&	J081334+313252	&	123.39	&	31.55	&	0.020	$\pm$	0.000005	&	1.20	$\pm$	0.094	&	1.30	$\pm$	0.071	\\
028	&	J081403+235328	&	123.52	&	23.89	&	0.020	$\pm$	0.000005	&	1.31	$\pm$	0.047	&	1.29	$\pm$	0.014	\\
029	&	J081420+575008	&	123.59	&	57.84	&	0.055	$\pm$	0.000005	&	1.72	$\pm$	0.128	&	1.56	$\pm$	0.084	\\
030	&	J081737+520236	&	124.41	&	52.04	&	0.024	$\pm$	0.000033	&	1.59	$\pm$	0.113	&	1.69	$\pm$	0.090	\\
031	&	J082520+082723	&	126.33	&	8.46	&	0.087	$\pm$	0.000008	&	1.68	$\pm$	0.068	&	1.66	$\pm$	0.006	\\
032	&	J082530+504804	&	126.38	&	50.80	&	0.097	$\pm$	0.000008	&	2.11	$\pm$	0.143	&	2.08	$\pm$	0.110	\\
033	&	J082722+202612	&	126.84	&	20.44	&	0.109	$\pm$	0.000006	&	2.46	$\pm$	0.079	&	2.47	$\pm$	0.032	\\
034	&	J083946+140033	&	129.94	&	14.01	&	0.112	$\pm$	0.000007	&	2.45	$\pm$	0.056	&	2.45	$\pm$	0.026	\\
035	&	J084000+180531	&	130.00	&	18.09	&	0.072	$\pm$	0.000007	&	2.06	$\pm$	0.095	&	1.94	$\pm$	0.039	\\
036	&	J084029+470710	&	130.12	&	47.12	&	0.042	$\pm$	0.001019	&	1.59	$\pm$	0.115	&	1.30	$\pm$	0.069	\\
037	&	J084056+022030	&	130.23	&	2.34	&	0.050	$\pm$	0.000796	&	---	&	---	\\
038	&	J084219+300703	&	130.58	&	30.12	&	0.084	$\pm$	0.000009	&	2.07	$\pm$	0.071	&	1.89	$\pm$	0.031	\\
039	&	J084220+115000	&	130.59	&	11.83	&	0.029	$\pm$	0.000030	&	1.33	$\pm$	0.099	&	1.17	$\pm$	0.062	\\
040	&	J084414+022621	&	131.06	&	2.44	&	0.091	$\pm$	0.000741	&	2.49	$\pm$	0.037	&	2.41	$\pm$	0.026	\\
041	&	J084527+530852	&	131.37	&	53.15	&	0.031	$\pm$	0.000031	&	1.20	$\pm$	0.093	&	1.17	$\pm$	0.064	\\
042	&	J084634+362620	&	131.64	&	36.44	&	0.011	$\pm$	0.000010	&	0.68	$\pm$	0.148	&	1.04	$\pm$	0.057	\\
043	&	J085221+121651	&	133.09	&	12.28	&	0.076	$\pm$	0.000796	&	2.76	$\pm$	0.171	&	1.69	$\pm$	0.104	\\
044	&	J090418+260106	&	136.08	&	26.02	&	0.098	$\pm$	0.000006	&	2.79	$\pm$	0.092	&	2.66	$\pm$	0.040	\\
045	&	J090506+223833	&	136.28	&	22.64	&	0.126	$\pm$	0.000009	&	2.23	$\pm$	0.068	&	2.15	$\pm$	0.019	\\
046	&	J090531+033530	&	136.38	&	3.59	&	0.039	$\pm$	0.000918	&	1.58	$\pm$	0.049	&	1.53	$\pm$	0.015	\\
047	&	J091434+470207	&	138.65	&	47.04	&	0.027	$\pm$	0.000030	&	1.46	$\pm$	0.106	&	1.30	$\pm$	0.069	\\
048	&	J091640+182807	&	139.17	&	18.47	&	0.022	$\pm$	0.000006	&	1.33	$\pm$	0.108	&	1.17	$\pm$	0.063	\\
049	&	J091652+003113	&	139.22	&	0.52	&	0.057	$\pm$	0.000004	&	1.78	$\pm$	0.034	&	1.71	$\pm$	0.016	\\
050	&	J092540+063116	&	141.42	&	6.52	&	0.075	$\pm$	0.000005	&	2.09	$\pm$	0.080	&	1.98	$\pm$	0.056	\\
051	&	J092749+084037	&	141.95	&	8.68	&	0.107	$\pm$	0.000007	&	2.60	$\pm$	0.090	&	2.41	$\pm$	0.035	\\
052	&	J092918+002813	&	142.33	&	0.47	&	0.094	$\pm$	0.000005	&	1.75	$\pm$	0.046	&	1.71	$\pm$	0.013	\\
053	&	J093006+602653	&	142.53	&	60.45	&	0.014	$\pm$	0.000009	&	1.20	$\pm$	0.094	&	1.04	$\pm$	0.056	\\
054	&	J093424+222522	&	143.60	&	22.42	&	0.084	$\pm$	0.000753	&	2.30	$\pm$	0.066	&	2.24	$\pm$	0.023	\\
055	&	J093813+542825	&	144.56	&	54.47	&	0.102	$\pm$	0.000712	&	2.89	$\pm$	0.178	&	2.73	$\pm$	0.141	\\
056	&	J094000+203122	&	145.00	&	20.52	&	0.045	$\pm$	0.000007	&	1.73	$\pm$	0.072	&	1.66	$\pm$	0.025	\\
057	&	J094252+354725	&	145.72	&	35.79	&	0.015	$\pm$	0.000010	&	1.33	$\pm$	0.100	&	1.30	$\pm$	0.072	\\
058	&	J094254+340411	&	145.73	&	34.07	&	0.022	$\pm$	0.000004	&	1.98	$\pm$	0.487	&	0.91	$\pm$	0.052	\\
059	&	J094809+425713	&	147.04	&	42.95	&	0.017	$\pm$	0.000006	&	1.20	$\pm$	0.094	&	1.04	$\pm$	0.056	\\
060	&	J095000+300341	&	147.50	&	30.06	&	0.017	$\pm$	0.000004	&	1.20	$\pm$	0.094	&	1.17	$\pm$	0.062	\\
061	&	J095023+004229	&	147.60	&	0.71	&	0.098	$\pm$	0.000719	&	2.67	$\pm$	0.093	&	2.42	$\pm$	0.032	\\
062	&	J095131+525936	&	147.88	&	52.99	&	0.046	$\pm$	0.000817	&	2.24	$\pm$	0.156	&	2.08	$\pm$	0.112	\\
063	&	J095226+021759	&	148.11	&	2.30	&	0.119	$\pm$	0.000685	&	2.57	$\pm$	0.098	&	2.44	$\pm$	0.044	\\
064	&	J095227+322809	&	148.11	&	32.47	&	0.015	$\pm$	0.000004	&	0.94	$\pm$	0.080	&	0.78	$\pm$	0.043	\\
065	&	J095545+413429	&	148.94	&	41.57	&	0.016	$\pm$	0.000005	&	1.20	$\pm$	0.095	&	1.04	$\pm$	0.056	\\
066	&	J100720+193349	&	151.84	&	19.56	&	0.031	$\pm$	0.000005	&	0.98	$\pm$	0.053	&	0.82	$\pm$	0.000	\\
067	&	J100746+025228	&	151.94	&	2.87	&	0.024	$\pm$	0.000926	&	1.46	$\pm$	0.106	&	1.17	$\pm$	0.063	\\
068	&	J101036+641242	&	152.65	&	64.21	&	0.040	$\pm$	0.000810	&	2.76	$\pm$	0.173	&	2.73	$\pm$	0.144	\\
069	&	J101042+125516	&	152.68	&	12.92	&	0.061	$\pm$	0.000933	&	1.94	$\pm$	0.101	&	1.70	$\pm$	0.046	\\
070	&	J101136+263027	&	152.90	&	26.51	&	0.055	$\pm$	0.000775	&	1.82	$\pm$	0.066	&	1.66	$\pm$	0.028	\\
071	&	J101157+130822	&	152.99	&	13.14	&	0.144	$\pm$	0.000005	&	0.68	$\pm$	0.077	&	2.34	$\pm$	0.123	\\
072	&	J101430+004755	&	153.63	&	0.80	&	0.147	$\pm$	0.000003	&	3.15	$\pm$	0.068	&	3.01	$\pm$	0.006	\\
073	&	J101458+193219	&	153.74	&	19.54	&	0.013	$\pm$	0.000004	&	0.94	$\pm$	0.084	&	0.65	$\pm$	0.037	\\
074	&	J102429+052451	&	156.12	&	5.41	&	0.033	$\pm$	0.000889	&	1.59	$\pm$	0.114	&	1.30	$\pm$	0.069	\\
075	&	J102732-284201	&	156.88	&	-28.70	&	0.032	$\pm$	0.000215	&	1.46	$\pm$	0.043	&	1.48	$\pm$	0.018	\\
076	&	J103226+271755	&	158.11	&	27.30	&	0.192	$\pm$	0.000009	&	---	&	---	\\
077	&	J103328+070801	&	158.37	&	7.13	&	0.045	$\pm$	0.000879	&	2.37	$\pm$	0.152	&	2.47	$\pm$	0.129	\\
078	&	J103412+014249	&	158.55	&	1.71	&	0.069	$\pm$	0.000004	&	1.88	$\pm$	0.052	&	1.71	$\pm$	0.004	\\
079	&	J103509+094516	&	158.79	&	9.75	&	0.049	$\pm$	0.000006	&	1.85	$\pm$	0.135	&	1.56	$\pm$	0.086	\\
080	&	J103726+270759	&	159.36	&	27.13	&	0.077	$\pm$	0.000005	&	1.84	$\pm$	0.062	&	1.84	$\pm$	0.029	\\
081	&	J104457+035313	&	161.24	&	3.89	&	0.013	$\pm$	0.000027	&	1.07	$\pm$	0.087	&	1.04	$\pm$	0.056	\\
082	&	J104554+010405	&	161.48	&	1.07	&	0.026	$\pm$	0.000030	&	1.33	$\pm$	0.104	&	1.56	$\pm$	0.083	\\
083	&	J104653+134645	&	161.72	&	13.78	&	0.011	$\pm$	0.000988	&	0.55	$\pm$	0.124	&	0.91	$\pm$	0.050	\\
084	&	J104723+302144	&	161.85	&	30.36	&	0.029	$\pm$	0.000033	&	1.72	$\pm$	0.119	&	1.69	$\pm$	0.092	\\
085	&	J104755+073951	&	161.98	&	7.66	&	0.168	$\pm$	0.000019	&	---	&	---	\\
086	&	J104829+111520	&	162.12	&	11.26	&	0.093	$\pm$	0.000006	&	1.63	$\pm$	0.059	&	1.43	$\pm$	0.012	\\
087	&	J105032+153806	&	162.64	&	15.64	&	0.085	$\pm$	0.000825	&	1.85	$\pm$	0.126	&	1.69	$\pm$	0.088	\\
088	&	J105040+342947	&	162.67	&	34.50	&	0.052	$\pm$	0.000855	&	1.58	$\pm$	0.060	&	1.47	$\pm$	0.017	\\
089	&	J105108+131927	&	162.79	&	13.32	&	0.045	$\pm$	0.000036	&	1.20	$\pm$	0.105	&	1.04	$\pm$	0.058	\\
090	&	J105210+032713	&	163.04	&	3.45	&	0.150	$\pm$	0.000008	&	2.06	$\pm$	0.128	&	2.01	$\pm$	0.001	\\
091	&	J105326+043014	&	163.36	&	4.50	&	0.019	$\pm$	0.000005	&	0.94	$\pm$	0.089	&	0.91	$\pm$	0.050	\\
092	&	J105331+011740	&	163.38	&	1.29	&	0.124	$\pm$	0.000006	&	2.23	$\pm$	0.069	&	2.14	$\pm$	0.040	\\
093	&	J105741+653539	&	164.42	&	65.59	&	0.011	$\pm$	0.000010	&	1.07	$\pm$	0.089	&	1.04	$\pm$	0.058	\\
094	&	J105940+080056	&	164.92	&	8.02	&	0.028	$\pm$	0.000004	&	2.11	$\pm$	0.143	&	2.21	$\pm$	0.121	\\
095	&	J110838+223809	&	167.16	&	22.64	&	0.024	$\pm$	0.000005	&	1.16	$\pm$	0.042	&	1.06	$\pm$	0.010	\\
096	&	J114212+002003	&	175.55	&	0.33	&	0.020	$\pm$	0.002160	&	3.24	$\pm$	0.066	&	3.20	$\pm$	0.057	\\
097	&	J115023-003141	&	177.60	&	-0.53	&	0.012	$\pm$	0.000081	&	0.87	$\pm$	0.032	&	0.68	$\pm$	0.005	\\
098	&	J121329+114056	&	183.37	&	11.68	&	0.021	$\pm$	0.000007	&	1.27	$\pm$	0.032	&	1.14	$\pm$	0.011	\\
099	&	J121717-280233	&	184.32	&	-28.04	&	0.026	$\pm$	0.000174	&	1.11	$\pm$	0.046	&	0.99	$\pm$	0.002	\\
100	&	J125305-031258	&	193.27	&	-3.22	&	0.023	$\pm$	0.001478	&	2.45	$\pm$	0.056	&	2.48	$\pm$	0.030	\\
101	&	J130119+123959	&	195.33	&	12.67	&	0.069	$\pm$	0.000766	&	3.18	$\pm$	0.060	&	3.14	$\pm$	0.021	\\
102	&	J131235+125743	&	198.15	&	12.96	&	0.026	$\pm$	0.000005	&	1.20	$\pm$	0.038	&	1.06	$\pm$	0.001	\\
103	&	J132347-013252	&	200.95	&	-1.55	&	0.022	$\pm$	0.000031	&	0.99	$\pm$	0.036	&	0.86	$\pm$	0.005	\\
104	&	J132549+330354	&	201.46	&	33.07	&	0.015	$\pm$	0.000113	&	1.14	$\pm$	0.038	&	1.05	$\pm$	0.007	\\
105	&	J133708-325528	&	204.28	&	-32.92	&	0.012	$\pm$	0.000081	&	0.80	$\pm$	0.032	&	0.63	$\pm$	0.002	\\
106	&	J134531+044232	&	206.38	&	4.71	&	0.030	$\pm$	0.000824	&	1.54	$\pm$	0.060	&	1.28	$\pm$	0.025	\\
107	&	J142342+225728	&	215.93	&	22.96	&	0.033	$\pm$	0.000018	&	2.06	$\pm$	0.064	&	2.16	$\pm$	0.059	\\
108	&	J144805-011057	&	222.02	&	-1.18	&	0.027	$\pm$	0.000047	&	2.05	$\pm$	0.061	&	2.05	$\pm$	0.038	\\
109	&	J162152+151855	&	245.47	&	15.32	&	0.034	$\pm$	0.000032	&	2.28	$\pm$	0.056	&	2.26	$\pm$	0.027	\\
110	&	J171236+321633	&	258.15	&	32.28	&	0.012	$\pm$	0.000004	&	1.03	$\pm$	0.032	&	0.96	$\pm$	0.005	\\
111	&	J192758-413432	&	291.99	&	-41.58	&	0.009	$\pm$	0.000060	&	1.06	$\pm$	0.040	&	0.92	$\pm$	0.015	\\
112	&	J210114-055510	&	315.31	&	-5.92	&	0.196	$\pm$	0.000006	&	---	&	---	\\
113	&	J210501-062238	&	316.26	&	-6.38	&	0.143	$\pm$	0.000010	&	2.24	$\pm$	0.184	&	2.34	$\pm$	0.128	\\
114	&	J211527-075951	&	318.86	&	-8.00	&	0.028	$\pm$	0.000007	&	1.12	$\pm$	0.037	&	0.89	$\pm$	0.004	\\
115	&	J211902-074226	&	319.76	&	-7.71	&	0.090	$\pm$	0.000008	&	1.33	$\pm$	0.263	&	1.43	$\pm$	0.077	\\
116	&	J212043+010006	&	320.18	&	1.00	&	0.114	$\pm$	0.000790	&	3.43	$\pm$	0.153	&	3.24	$\pm$	0.219	\\
117	&	J212332-074831	&	320.89	&	-7.81	&	0.028	$\pm$	0.000008	&	1.07	$\pm$	0.106	&	0.91	$\pm$	0.052	\\
118	&	J214350-072003	&	325.96	&	-7.33	&	0.110	$\pm$	0.000010	&	0.81	$\pm$	0.419	&	2.47	$\pm$	0.139	\\
119	&	J220802+131334	&	332.01	&	13.23	&	0.116	$\pm$	0.000007	&	3.02	$\pm$	0.205	&	2.99	$\pm$	0.158	\\
120	&	J221823+003918	&	334.60	&	0.66	&	0.108	$\pm$	0.000005	&	2.65	$\pm$	0.155	&	2.58	$\pm$	0.046	\\
121	&	J222510-001152	&	336.29	&	-0.20	&	0.067	$\pm$	0.000005	&	1.87	$\pm$	0.076	&	1.81	$\pm$	0.023	\\
122	&	J224556+125022	&	341.49	&	12.84	&	0.080	$\pm$	0.000008	&	2.24	$\pm$	0.149	&	1.95	$\pm$	0.102	\\
123	&	J225140+132713	&	342.92	&	13.45	&	0.062	$\pm$	0.000006	&	2.11	$\pm$	0.139	&	2.21	$\pm$	0.115	\\
124	&	J230117+135230	&	345.32	&	13.88	&	0.025	$\pm$	0.000005	&	1.07	$\pm$	0.087	&	1.04	$\pm$	0.056	\\
125	&	J230123+133314	&	345.35	&	13.55	&	0.030	$\pm$	0.000894	&	1.59	$\pm$	0.112	&	1.56	$\pm$	0.083	\\
126	&	J230703+011311	&	346.77	&	1.22	&	0.126	$\pm$	0.000010	&	3.02	$\pm$	0.186	&	2.86	$\pm$	0.147	\\
127	&	J231442+010621	&	348.68	&	1.11	&	0.034	$\pm$	0.000005	&	1.33	$\pm$	0.112	&	1.17	$\pm$	0.063	\\
128	&	J232936-011056	&	352.40	&	-1.18	&	0.066	$\pm$	0.000006	&	1.72	$\pm$	0.120	&	1.69	$\pm$	0.088	\\

\end{longtable}
%\end{ThreePartTable}
\end{center}
\normalsize 
%\end{landscape}
\twocolumn


==> ch04/tab/tbl3.tex <==
\onecolumn
\scriptsize
\begin{center}
\begin{longtable}{@{} l l c c c c @{}}
 
\caption{ Total fluxes for $\hb$ and $[\Oiii]\ \lambda \lambda 4959, 5007$ lines as measured from the low resolution spectra (LS) and the  $\hb$ flux measured from SDSS DR7. } 
\label{tab:tbl3} \\


%This is the header for the first page of the table...
\hline \hline \\[-2ex]
\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{Flux (SDSS DR7)}} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{Flux (LS)}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 4959}$ \textbf{Flux}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 5007}$ \textbf{Flux}} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} \\[0.5ex] \hline \\[-1.8ex]

\endfirsthead

%This is the header for the remaining page(s) of the table...
\multicolumn{1}{c}{\bf{Index}} &
\multicolumn{1}{c}{\bf{Name}} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{Flux (SDSS DR7)}} &
\multicolumn{1}{c}{$\mathbf{\hb}$ \textbf{Flux (LS)}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 4959}$ \textbf{Flux}} &
\multicolumn{1}{c}{$\mathbf{[\Oiii]\ \lambda \lambda 5007}$ \textbf{Flux}} \\

\multicolumn{1}{c}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} &
\multicolumn{1}{c}{ ($10^{-16}\ \mathrm{erg\ s^{-1} cm^{-2}}$)} \\[0.5ex] \hline \\[-1.8ex]

\endhead



\multicolumn{2}{l}{{Continued on Next Page\ldots}} \\
\endfoot


\\[-1.8ex] \hline 
%\insertTableNotes
\endlastfoot

001	&	J000657+005125	&	88.73	$\pm$	1.353	&	67.74	$\pm$	4.295	&	126.90	$\pm$	8.132	&	381.70	$\pm$	22.569	\\
002	&	J001647-104742	&	171.76	$\pm$	1.832	&	233.70	$\pm$	14.817	&	298.10	$\pm$	19.102	&	882.50	$\pm$	52.181	\\
003	&	J002339-094848	&	128.14	$\pm$	1.030	&	155.30	$\pm$	9.846	&	315.30	$\pm$	20.205	&	955.50	$\pm$	56.497	\\
004	&	J002425+140410	&	275.68	$\pm$	1.903	&	419.20	$\pm$	29.311	&	603.15	$\pm$	48.039	&	1804.75	$\pm$	146.982	\\
005	&	J003218+150014	&	253.01	$\pm$	1.361	&	410.20	$\pm$	26.007	&	671.90	$\pm$	43.056	&	2060.00	$\pm$	121.805	\\
006	&	J005147+000940	&	96.48	$\pm$	0.580	&	120.40	$\pm$	7.634	&	192.10	$\pm$	12.310	&	581.10	$\pm$	34.360	\\
007	&	J005602-101009	&	66.57	$\pm$	0.846	&	70.10	$\pm$	4.444	&	88.78	$\pm$	5.689	&	252.00	$\pm$	14.900	\\
008	&	J013258-085337	&	79.77	$\pm$	0.994	&	80.08	$\pm$	5.077	&	113.50	$\pm$	7.273	&	307.10	$\pm$	18.158	\\
009	&	J013344+005711	&	71.07	$\pm$	1.046	&	30.95	$\pm$	1.962	&	64.69	$\pm$	4.145	&	166.60	$\pm$	9.851	\\
010	&	J014137-091435	&	91.01	$\pm$	1.156	&	---	&	---	&	---	\\
011	&	J014707+135629	&	114.37	$\pm$	0.963	&	160.60	$\pm$	10.182	&	288.30	$\pm$	18.474	&	867.70	$\pm$	51.306	\\
012	&	J021852-091218	&	71.59	$\pm$	1.183	&	95.20	$\pm$	6.036	&	204.20	$\pm$	13.085	&	603.90	$\pm$	35.708	\\
013	&	J022037-092907	&	87.07	$\pm$	1.448	&	170.20	$\pm$	10.791	&	293.80	$\pm$	18.827	&	879.00	$\pm$	51.974	\\
014	&	J024052-082827	&	173.25	$\pm$	7.354	&	196.00	$\pm$	12.427	&	474.30	$\pm$	30.393	&	1397.00	$\pm$	82.603	\\
015	&	J024453-082137	&	69.82	$\pm$	0.761	&	112.40	$\pm$	7.126	&	149.70	$\pm$	9.593	&	440.00	$\pm$	26.017	\\
016	&	J025426-004122	&	133.24	$\pm$	1.269	&	207.80	$\pm$	13.175	&	305.10	$\pm$	19.551	&	898.90	$\pm$	53.151	\\
017	&	J030321-075923	&	65.21	$\pm$	1.458	&	45.52	$\pm$	2.886	&	80.35	$\pm$	5.149	&	248.30	$\pm$	14.682	\\
018	&	J031023-083432	&	60.86	$\pm$	0.820	&	---	&	---	&	---	\\
019	&	J033526-003811	&	69.06	$\pm$	1.059	&	115.50	$\pm$	7.323	&	188.90	$\pm$	12.105	&	541.60	$\pm$	32.024	\\
020	&	J040937-051805	&	61.40	$\pm$	0.798	&	---	&	---	&	---	\\
021	&	J051519-391741	&	173.78	$\pm$	5.213	&	---	&	---	&	---	\\
022	&	J064650-374322	&	181.97	$\pm$	5.459	&	---	&	---	&	---	\\
023	&	J074806+193146	&	87.31	$\pm$	1.283	&	74.98	$\pm$	4.754	&	96.12	$\pm$	6.159	&	289.00	$\pm$	17.088	\\
024	&	J074947+154013	&	44.73	$\pm$	0.683	&	60.32	$\pm$	3.824	&	94.18	$\pm$	6.035	&	282.50	$\pm$	16.704	\\
025	&	J080000+274642	&	98.89	$\pm$	1.175	&	60.63	$\pm$	3.844	&	116.40	$\pm$	7.459	&	315.90	$\pm$	18.679	\\
026	&	J080619+194927	&	293.37	$\pm$	2.494	&	400.30	$\pm$	25.380	&	526.20	$\pm$	33.719	&	1610.00	$\pm$	95.197	\\
027	&	J081334+313252	&	226.56	$\pm$	1.618	&	360.10	$\pm$	22.831	&	791.20	$\pm$	50.701	&	2348.50	$\pm$	138.864	\\
028	&	J081403+235328	&	120.58	$\pm$	2.010	&	122.60	$\pm$	7.773	&	205.40	$\pm$	13.162	&	599.30	$\pm$	35.436	\\
029	&	J081420+575008	&	73.86	$\pm$	0.781	&	112.60	$\pm$	7.139	&	155.60	$\pm$	9.971	&	459.70	$\pm$	27.181	\\
030	&	J081737+520236	&	250.40	$\pm$	2.011	&	338.30	$\pm$	21.449	&	456.40	$\pm$	29.246	&	1303.00	$\pm$	77.045	\\
031	&	J082520+082723	&	43.61	$\pm$	0.786	&	45.09	$\pm$	2.859	&	105.50	$\pm$	6.760	&	292.50	$\pm$	17.295	\\
032	&	J082530+504804	&	105.40	$\pm$	1.190	&	135.00	$\pm$	8.559	&	229.30	$\pm$	14.694	&	654.20	$\pm$	38.682	\\
033	&	J082722+202612	&	89.16	$\pm$	1.237	&	129.10	$\pm$	8.185	&	208.60	$\pm$	13.367	&	628.80	$\pm$	37.180	\\
034	&	J083946+140033	&	70.39	$\pm$	0.844	&	83.71	$\pm$	5.307	&	106.90	$\pm$	6.850	&	309.40	$\pm$	18.294	\\
035	&	J084000+180531	&	109.27	$\pm$	1.311	&	124.90	$\pm$	7.919	&	252.10	$\pm$	16.155	&	733.40	$\pm$	43.365	\\
036	&	J084029+470710	&	249.99	$\pm$	4.364	&	354.10	$\pm$	22.450	&	651.10	$\pm$	41.723	&	1952.00	$\pm$	115.419	\\
037	&	J084056+022030	&	73.72	$\pm$	0.762	&	44.54	$\pm$	2.824	&	36.62	$\pm$	2.347	&	107.70	$\pm$	6.368	\\
038	&	J084219+300703	&	96.21	$\pm$	0.916	&	128.80	$\pm$	8.166	&	175.00	$\pm$	11.214	&	507.40	$\pm$	30.002	\\
039	&	J084220+115000	&	220.44	$\pm$	1.430	&	---	&	---	&	---	\\
040	&	J084414+022621	&	167.65	$\pm$	1.584	&	211.80	$\pm$	13.428	&	393.15	$\pm$	25.193	&	1165.00	$\pm$	68.885	\\
041	&	J084527+530852	&	198.32	$\pm$	1.395	&	212.50	$\pm$	13.473	&	382.00	$\pm$	24.479	&	1096.00	$\pm$	64.805	\\
042	&	J084634+362620	&	324.74	$\pm$	1.964	&	---	&	---	&	---	\\
043	&	J085221+121651	&	370.73	$\pm$	3.199	&	448.00	$\pm$	28.404	&	868.60	$\pm$	55.660	&	2594.00	$\pm$	153.380	\\
044	&	J090418+260106	&	113.73	$\pm$	1.034	&	---	&	---	&	---	\\
045	&	J090506+223833	&	79.73	$\pm$	0.686	&	---	&	---	&	---	\\
046	&	J090531+033530	&	110.18	$\pm$	0.909	&	178.30	$\pm$	11.304	&	273.30	$\pm$	17.513	&	879.20	$\pm$	51.986	\\
047	&	J091434+470207	&	394.81	$\pm$	1.471	&	526.60	$\pm$	28.081	&	927.38	$\pm$	52.650	&	2702.50	$\pm$	134.910	\\
048	&	J091640+182807	&	112.27	$\pm$	1.189	&	---	&	---	&	---	\\
049	&	J091652+003113	&	65.51	$\pm$	0.758	&	81.43	$\pm$	5.163	&	112.40	$\pm$	7.203	&	339.60	$\pm$	20.080	\\
050	&	J092540+063116	&	68.24	$\pm$	1.169	&	98.43	$\pm$	6.241	&	147.10	$\pm$	9.426	&	437.50	$\pm$	25.869	\\
051	&	J092749+084037	&	83.03	$\pm$	1.319	&	99.69	$\pm$	6.320	&	84.03	$\pm$	5.385	&	268.10	$\pm$	15.852	\\
052	&	J092918+002813	&	70.06	$\pm$	1.141	&	115.70	$\pm$	7.336	&	185.50	$\pm$	11.887	&	530.80	$\pm$	31.385	\\
053	&	J093006+602653	&	321.23	$\pm$	1.538	&	509.80	$\pm$	32.322	&	878.00	$\pm$	56.263	&	2540.00	$\pm$	150.187	\\
054	&	J093424+222522	&	99.16	$\pm$	1.176	&	---	&	---	&	---	\\
055	&	J093813+542825	&	151.26	$\pm$	2.877	&	293.70	$\pm$	18.621	&	410.90	$\pm$	26.331	&	1202.00	$\pm$	71.073	\\
056	&	J094000+203122	&	103.86	$\pm$	0.904	&	101.00	$\pm$	6.404	&	123.90	$\pm$	7.940	&	377.20	$\pm$	22.303	\\
057	&	J094252+354725	&	191.97	$\pm$	1.002	&	---	&	---	&	---	\\
058	&	J094254+340411	&	64.37	$\pm$	0.915	&	83.35	$\pm$	5.285	&	142.80	$\pm$	9.151	&	414.10	$\pm$	24.485	\\
059	&	J094809+425713	&	160.17	$\pm$	1.238	&	---	&	---	&	---	\\
060	&	J095000+300341	&	148.45	$\pm$	1.367	&	198.20	$\pm$	12.566	&	304.60	$\pm$	19.519	&	933.60	$\pm$	55.202	\\
061	&	J095023+004229	&	123.16	$\pm$	2.039	&	139.90	$\pm$	8.870	&	240.20	$\pm$	15.392	&	768.20	$\pm$	45.423	\\
062	&	J095131+525936	&	186.09	$\pm$	1.957	&	312.20	$\pm$	19.794	&	605.70	$\pm$	38.814	&	1792.00	$\pm$	105.958	\\
063	&	J095226+021759	&	100.26	$\pm$	1.919	&	---	&	---	&	---	\\
064	&	J095227+322809	&	148.42	$\pm$	1.674	&	219.60	$\pm$	13.923	&	449.10	$\pm$	28.779	&	1304.00	$\pm$	77.104	\\
065	&	J095545+413429	&	195.13	$\pm$	1.972	&	---	&	---	&	---	\\
066	&	J100720+193349	&	59.28	$\pm$	0.934	&	48.95	$\pm$	3.104	&	82.61	$\pm$	5.294	&	246.90	$\pm$	14.599	\\
067	&	J100746+025228	&	180.69	$\pm$	0.895	&	245.60	$\pm$	15.571	&	395.50	$\pm$	25.344	&	1137.00	$\pm$	67.229	\\
068	&	J101036+641242	&	234.88	$\pm$	3.374	&	316.20	$\pm$	20.048	&	414.60	$\pm$	26.568	&	1220.00	$\pm$	72.137	\\
069	&	J101042+125516	&	318.65	$\pm$	7.967	&	460.30	$\pm$	29.184	&	813.60	$\pm$	52.136	&	2409.00	$\pm$	142.441	\\
070	&	J101136+263027	&	90.69	$\pm$	0.720	&	125.40	$\pm$	7.951	&	181.00	$\pm$	11.599	&	552.20	$\pm$	32.651	\\
071	&	J101157+130822	&	86.39	$\pm$	4.602	&	---	&	---	&	---	\\
072	&	J101430+004755	&	73.70	$\pm$	1.056	&	---	&	---	&	---	\\
073	&	J101458+193219	&	49.30	$\pm$	0.674	&	---	&	---	&	---	\\
074	&	J102429+052451	&	274.01	$\pm$	1.448	&	564.10	$\pm$	35.765	&	889.40	$\pm$	56.993	&	2553.00	$\pm$	150.955	\\
075	&	J102732-284201	&	158.49	$\pm$	3.170	&	---	&	---	&	---	\\
076	&	J103226+271755	&	53.18	$\pm$	1.190	&	54.80	$\pm$	3.474	&	100.70	$\pm$	6.453	&	308.60	$\pm$	18.247	\\
077	&	J103328+070801	&	388.92	$\pm$	2.212	&	555.00	$\pm$	35.188	&	493.60	$\pm$	31.630	&	1435.00	$\pm$	84.850	\\
078	&	J103412+014249	&	48.16	$\pm$	0.881	&	---	&	---	&	---	\\
079	&	J103509+094516	&	76.84	$\pm$	0.805	&	85.30	$\pm$	5.408	&	130.30	$\pm$	8.350	&	379.70	$\pm$	22.451	\\
080	&	J103726+270759	&	63.61	$\pm$	1.033	&	---	&	---	&	---	\\
081	&	J104457+035313	&	420.94	$\pm$	4.519	&	467.60	$\pm$	29.647	&	688.70	$\pm$	44.132	&	2038.00	$\pm$	120.504	\\
082	&	J104554+010405	&	388.87	$\pm$	2.225	&	630.40	$\pm$	39.968	&	982.00	$\pm$	62.927	&	2736.00	$\pm$	161.776	\\
083	&	J104653+134645	&	184.55	$\pm$	1.186	&	430.40	$\pm$	27.288	&	712.40	$\pm$	45.651	&	2092.00	$\pm$	123.697	\\
084	&	J104723+302144	&	488.90	$\pm$	2.757	&	922.40	$\pm$	58.482	&	1319.00	$\pm$	84.522	&	3892.00	$\pm$	230.129	\\
085	&	J104755+073951	&	66.50	$\pm$	3.595	&	---	&	---	&	---	\\
086	&	J104829+111520	&	70.42	$\pm$	0.836	&	77.49	$\pm$	4.913	&	148.50	$\pm$	9.516	&	406.90	$\pm$	24.059	\\
087	&	J105032+153806	&	244.45	$\pm$	5.990	&	329.00	$\pm$	20.859	&	688.30	$\pm$	44.107	&	1980.00	$\pm$	117.075	\\
088	&	J105040+342947	&	143.34	$\pm$	1.035	&	211.60	$\pm$	13.416	&	334.30	$\pm$	21.422	&	980.00	$\pm$	57.946	\\
089	&	J105108+131927	&	62.93	$\pm$	0.709	&	101.70	$\pm$	6.448	&	123.50	$\pm$	7.914	&	357.50	$\pm$	21.138	\\
090	&	J105210+032713	&	41.76	$\pm$	4.663	&	---	&	---	&	---	\\
091	&	J105326+043014	&	109.70	$\pm$	1.187	&	---	&	---	&	---	\\
092	&	J105331+011740	&	76.17	$\pm$	1.217	&	---	&	---	&	---	\\
093	&	J105741+653539	&	166.45	$\pm$	1.246	&	---	&	---	&	---	\\
094	&	J105940+080056	&	135.22	$\pm$	1.408	&	178.50	$\pm$	11.317	&	275.60	$\pm$	17.661	&	789.80	$\pm$	46.700	\\
095	&	J110838+223809	&	172.79	$\pm$	1.432	&	121.80	$\pm$	7.722	&	238.90	$\pm$	15.309	&	717.40	$\pm$	42.419	\\
096	&	J114212+002003	&	689.72	$\pm$	3.283	&	2985.00	$\pm$	189.254	&	2773.00	$\pm$	177.695	&	8456.00	$\pm$	499.991	\\
097	&	J115023-003141	&	95.50	$\pm$	2.865	&	---	&	---	&	---	\\
098	&	J121329+114056	&	215.44	$\pm$	1.786	&	243.80	$\pm$	15.457	&	505.30	$\pm$	32.380	&	1530.00	$\pm$	90.467	\\
099	&	J121717-280233	&	223.87	$\pm$	4.477	&	---	&	---	&	---	\\
100	&	J125305-031258	&	1909.74	$\pm$	11.319	&	3484.33	$\pm$	275.115	&	7357.00	$\pm$	464.634	&	22180.00	$\pm$	1038.436	\\
101	&	J130119+123959	&	225.69	$\pm$	4.080	&	331.70	$\pm$	21.030	&	364.60	$\pm$	23.364	&	1076.00	$\pm$	63.622	\\
102	&	J131235+125743	&	146.31	$\pm$	1.333	&	220.25	$\pm$	13.964	&	343.85	$\pm$	22.034	&	1007.90	$\pm$	59.596	\\
103	&	J132347-013252	&	156.22	$\pm$	1.542	&	196.20	$\pm$	9.400	&	471.85	$\pm$	10.250	&	1411.50	$\pm$	45.500	\\
104	&	J132549+330354	&	383.32	$\pm$	1.647	&	309.90	$\pm$	19.648	&	605.50	$\pm$	38.801	&	1826.00	$\pm$	107.969	\\
105	&	J133708-325528	&	257.04	$\pm$	5.141	&	---	&	---	&	---	\\
106	&	J134531+044232	&	166.90	$\pm$	1.063	&	371.53	$\pm$	5.668	&	575.37	$\pm$	14.134	&	1722.67	$\pm$	54.618	\\
107	&	J142342+225728	&	178.23	$\pm$	1.019	&	268.40	$\pm$	17.017	&	436.70	$\pm$	27.984	&	1255.00	$\pm$	74.206	\\
108	&	J144805-011057	&	485.02	$\pm$	2.017	&	736.04	$\pm$	22.399	&	1599.60	$\pm$	75.978	&	4788.40	$\pm$	123.951	\\
109	&	J162152+151855	&	318.48	$\pm$	2.529	&	507.33	$\pm$	35.661	&	712.70	$\pm$	45.630	&	2107.67	$\pm$	173.509	\\
110	&	J171236+321633	&	151.27	$\pm$	1.193	&	207.86	$\pm$	32.385	&	365.72	$\pm$	54.693	&	1079.50	$\pm$	155.155	\\
111	&	J192758-413432	&	2630.27	$\pm$	5.261	&	---	&	---	&	---	\\
112	&	J210114-055510	&	52.91	$\pm$	0.924	&	62.85	$\pm$	3.985	&	102.90	$\pm$	6.594	&	304.10	$\pm$	17.981	\\
113	&	J210501-062238	&	46.64	$\pm$	0.697	&	36.72	$\pm$	2.328	&	40.32	$\pm$	2.584	&	119.80	$\pm$	7.084	\\
114	&	J211527-075951	&	126.76	$\pm$	1.186	&	---	&	---	&	---	\\
115	&	J211902-074226	&	52.20	$\pm$	0.928	&	84.76	$\pm$	5.374	&	132.70	$\pm$	8.503	&	395.90	$\pm$	23.409	\\
116	&	J212043+010006	&	69.84	$\pm$	1.001	&	---	&	---	&	---	\\
117	&	J212332-074831	&	51.01	$\pm$	0.913	&	69.95	$\pm$	4.435	&	103.70	$\pm$	6.645	&	302.40	$\pm$	17.880	\\
118	&	J214350-072003	&	47.54	$\pm$	0.887	&	---	&	---	&	---	\\
119	&	J220802+131334	&	60.88	$\pm$	1.136	&	85.33	$\pm$	5.410	&	138.10	$\pm$	8.850	&	377.00	$\pm$	22.291	\\
120	&	J221823+003918	&	38.77	$\pm$	0.792	&	---	&	---	&	---	\\
121	&	J222510-001152	&	146.12	$\pm$	1.479	&	150.80	$\pm$	9.561	&	297.90	$\pm$	19.090	&	896.50	$\pm$	53.009	\\
122	&	J224556+125022	&	129.95	$\pm$	1.310	&	161.90	$\pm$	10.265	&	177.50	$\pm$	11.374	&	532.90	$\pm$	31.510	\\
123	&	J225140+132713	&	210.10	$\pm$	1.280	&	404.40	$\pm$	25.640	&	548.70	$\pm$	35.161	&	1612.00	$\pm$	95.315	\\
124	&	J230117+135230	&	103.47	$\pm$	1.238	&	152.80	$\pm$	9.688	&	209.50	$\pm$	13.425	&	644.40	$\pm$	38.102	\\
125	&	J230123+133314	&	185.45	$\pm$	1.274	&	340.80	$\pm$	21.607	&	547.90	$\pm$	35.110	&	1662.00	$\pm$	98.272	\\
126	&	J230703+011311	&	99.65	$\pm$	2.527	&	113.70	$\pm$	7.209	&	131.10	$\pm$	8.401	&	385.10	$\pm$	22.770	\\
127	&	J231442+010621	&	51.90	$\pm$	0.845	&	58.58	$\pm$	3.714	&	78.24	$\pm$	5.014	&	226.00	$\pm$	13.363	\\
128	&	J232936-011056	&	84.60	$\pm$	0.870	&	104.00	$\pm$	6.594	&	210.30	$\pm$	13.476	&	591.10	$\pm$	34.951	\\


\end{longtable}
%\end{ThreePartTable}
\end{center}
\normalsize 
\twocolumn

